Estimating Egocentric 3D Human Pose in the Wild with External Weak Supervision

Egocentric 3D human pose estimation with a single fisheye camera has drawn a significant amount of attention recently. However, existing methods struggle with pose estimation from in-the-wild images, because they can only be trained on synthetic data due to the unavailability of large-scale in-the-wild egocentric datasets. Furthermore, these methods easily fail when the body parts are occluded by or interacting with the surrounding scene. To address the shortage of in-the-wild data, we collect a large-scale in-the-wild egocentric dataset called Egocentric Poses in the Wild (EgoPW). This dataset is captured by a head-mounted fisheye camera and an auxiliary external camera, which provides an additional observation of the human body from a third-person perspective during training. We present a new egocentric pose estimation method, which can be trained on the new dataset with weak external supervision. Specifically, we first generate pseudo labels for the EgoPW dataset with a spatio-temporal optimization method by incorporating the external-view supervision. The pseudo labels are then used to train an egocentric pose estimation network. To facilitate the network training, we propose a novel learning strategy to supervise the egocentric features with the high-quality features extracted by a pretrained external-view pose estimation model. The experiments show that our method predicts accurate 3D poses from a single in-the-wild egocentric image and outperforms the state-of-the-art methods both quantitatively and qualitatively.

==> Estimating Egocentric 3D Human Pose in the Wild-CVPR2022/sections/abstract.tex <==
\begin{abstract}
Egocentric 3D human pose estimation with a single fisheye camera has drawn a significant amount of attention recently. However, existing methods struggle with pose estimation from in-the-wild images, because they can only be trained on synthetic data due to the unavailability of large-scale in-the-wild egocentric datasets. Furthermore, these methods easily fail when the body parts are occluded by or interacting with the surrounding scene. To address the shortage of in-the-wild data, we collect a large-scale in-the-wild egocentric dataset called \emph{Egocentric Poses in the Wild (EgoPW)}. This dataset is captured by a head-mounted fisheye camera and an auxiliary external camera, which provides an additional observation of the human body from a third-person perspective during training.
We present a new egocentric pose estimation method, which can be trained on the new dataset with weak external supervision. 
Specifically, we first generate pseudo labels for the EgoPW dataset with a spatio-temporal optimization method by incorporating the external-view supervision.
The pseudo labels are then used to train an egocentric pose estimation network. To facilitate the network training, we propose a novel learning strategy to supervise the egocentric features with the high-quality features extracted by a pretrained external-view pose estimation model. 
The experiments show that our method predicts accurate 3D poses from a single in-the-wild egocentric image and outperforms the state-of-the-art methods both quantitatively and qualitatively. 
% Egocentric 3D human pose estimation with a single fisheye camera has drawn a significant amount of attention recently. However, existing methods are usually trained only on synthetic datasets due to the limited accessible real data, which causes performance drop on real images as the domain gap between the synthetic and real images exists. Furthermore, these methods often fail when the body parts are occluded by or interacting with the surrounding scene. To tackle these issues, we present a new approach to egocentric 3D human pose estimation from an egocentric image. Our method can be trained in a weakly supervised manner based on 2D supervision from an egocentric view and an auxiliary external view. 

% on a new in-the-wild egocentric dataset, called \emph{Egocentric Poses in the Wild (EgoPW)}, captured by a head-mounted fisheye camera and an auxiliary external camera, which provides additional observation of the body from a third-person perspective for training. Note that this external camera view is only used for training, while during the test we only rely on the egocentric fisheye camera. Our training method combines the information from both the egocentric view and external view to generate pseudo labels for the EgoPW dataset as optimization in the training loop. We also present an adversarial training strategy to align the semantic representation between the egocentric images and external images.
% The experiments show that our method predicts accurate 3D poses from a single in-the-wild egocentric image and significantly outperforms the state-of-the-arts both quantitatively and qualitatively. 
% Note that this external camera view is only used for training, while during the test we only rely on the egocentric fisheye camera. 
% The pseudo labels are then used to train an egocentric pose estimation network. To facilitate the learning of the features extracted from the egocentric view for pose estimation, we propose a novel learning strategy by supervising the egocentric features with the high-quality features extracted from external view by a pretrained external-view feature extraction model. 
% facilitate the learning of egocentric with the features from the external view. 
%  since the egocentric and external images share the same identity and pose
% Then, we exploit an observation that the extracted features from the external view can facilitate the learning of egocentric pose estimation network, since the egocentric and external view share the same identity and pose. In light of this observation, we enforce the feature distribution extracted from these two views to be consistent with an adversarial discriminator. 
% In light of this observation, we propose a new training strategy to enforce the features extracted from these two views to be consistent with an adversarial discriminator. 
% We then  propose an adversarial training strategy to enforce the  egocentric semantic features with supervision from an external pose estimation network. 
\end{abstract}

==> Estimating Egocentric 3D Human Pose in the Wild-CVPR2022/sections/conclusions.tex <==
\section{Conclusions}
In this paper, we have proposed a new approach to egocentric human pose estimation with a single head-mounted fisheye camera. We collected a new in-the-wild egocentric dataset (EgoPW) and designed a new optimization method to generate accurate egocentric poses as pseudo labels. Next, we supervise the egocentric pose estimation network with the pseudo labels and the features from the external network.
The experiments show that our method outperforms all of the state-of-the-art methods both qualitatively and quantitatively and our method also works well under severe occlusion. 
% The performance of each individual component is also evaluated in the ablation study. 
As future work, we would like to develop a video-based method for estimating temporally-consistent egocentric poses from an in-the-wild video. 
% Another interesting direction is to integrate the physics constraints into the egocentric pose estimation problem for more accurate body pose estimation.

\noindent\textbf{Limitations.} The accuracy of pseudo labels in our method is constrained by our in-the-wild capture system, which only contains one egocentric view and one external view, and further constrains the performance of our method. To solve this, we can fuse different sensors, including IMUs and depth cameras, for capturing the in-the-wild dataset, which can be explored in our follow-up work.



==> Estimating Egocentric 3D Human Pose in the Wild-CVPR2022/sections/experiments.tex <==
\section{Experiments}

\subsection{Datasets}

% Our network is trained on the synthetic dataset from Mo$^2$Cap$^2$ \cite{DBLP:journals/tvcg/XuCZRFST19} and the training split of EgoPW dataset. The Mo$^2$Cap$^2$ training dataset contains 530k images under 700 body textures.
We quantitatively evaluate our finetuned network on the real-world dataset from Mo$^2$Cap$^2$ \cite{DBLP:journals/tvcg/XuCZRFST19} and Wang \etal~\cite{wang2021estimating}. The real-world dataset in Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} contains 2.7k frames of two people captured in indoor and outdoor scenes, and that in Wang \etal~\cite{wang2021estimating} contains 12k frames of two people captured in the studio. To measure the accuracy of our pseudo labels, we evaluate our optimization method (Sec.~\ref{subsec:optimizer}) only on the dataset from Wang \etal~\cite{wang2021estimating} since the Mo$^2$Cap$^2$ dataset does not include the external view.

% These datasets have the ground truth 3D poses from a multi-view motion capture system while they are mostly captured in the studio. \LJ{suggest removing the above sentence} 
To evaluate our method on the in-the-wild data, we also conduct a qualitative evaluation on the test set of the EgoPW dataset. The EgoPW dataset will be made publicly available, and more details and comparisons to other datasets are included in the supplementary materials.

\subsection{Evaluation Metrics}
We measure the results of our method as well as other baseline methods with two metrics, PA-MPJPE and BA-MPJPE, which estimate the accuracy of a single body pose. For \textbf{PA-MPJPE}, we rigidly align the estimated pose $\mathcal{\hat{P}}$ of each frame to the ground truth pose $\mathcal{P}$ using Procrustes analysis \cite{kendall1989survey}. In order to eliminate the influence of the body scale, we also report the \textbf{BA-MPJPE} scores. In this metric,  we first resize the bone length of each predicted body pose $\mathcal{\hat{P}}$ and ground truth body pose $\mathcal{P}$ to the bone length of a standard skeleton. Then, we calculate the PA-MPJPE between the two resulting poses. 

\begin{figure*}
\centering
\includegraphics[width=0.975\linewidth]{figures/results/results_new_crop.pdf}
\caption{Qualitative comparison between our method and the state-of-the-art methods. From left to right: input image, Mo$^2$Cap$^2$ result, $x$R-egopose result, our result, and external image. The ground truth pose is shown in red. Note that the external images are not used during inference.}
\label{fig:results}
\end{figure*}

\subsection{Pseudo Label Generation}\label{subsec:pseudo_labels}

\begin{table}[h]
\begin{center}
\small
\begin{tabular}{p{0.19\textwidth}
>{\centering}p{0.1\textwidth}
>{\centering\arraybackslash}p{0.1\textwidth}}
\hlineB{2.5}
Method & PA-MPJPE & BA-MPJPE \\ \hline
Mo$^2$Cap$^2$ & 102.3 & 74.46 \\
$x$R-egopose & 112.0 & 87.20 \\
Wang \etal~\cite{wang2021estimating} & 83.40 & 63.88 \\
VIBE~\cite{DBLP:conf/cvpr/KocabasAB20} & 68.13 & 52.99 \\
\hline
Our Optimizer & \textbf{57.19} & \textbf{46.14}\\
\hlineB{2.5}
\end{tabular}
\end{center}
\caption{The performance of our optimization framework on  Wang \etal's dataset. Our optimization method outperforms all previous egocentric pose estimation methods and the state-of-the-art pose estimation method of the external view.}
\label{table:pseudo_labels}
% \vspace{-1em}
\end{table}

In this paper, we first generate the pseudo labels with the optimization framework (Sec.~\ref{subsec:optimizer}) and use them to train our network. Thus, pseudo labels with higher accuracy generally lead to better network performance.
% Thus, the accuracy of pseudo labels is critical \DL{if we say that it is critical, one could say that 60mm after PA is not precise enough}. 
In this experiment, we evaluate the accuracy of pseudo labels on Wang~\etal's dataset and show the results in Table~\ref{table:pseudo_labels}. 
This table shows that our method outperforms all the baseline methods by leveraging both the egocentric view and external view during optimization. Note that though compared in Table~\ref{table:pseudo_labels}, we cannot use any external-view based pose estimation method, \eg VIBE~\cite{DBLP:conf/cvpr/KocabasAB20} and 3DPW~\cite{von2018recovering}, for training the egocentric pose estimation network. This is because the relative pose between the external and egocentric camera is unknown, making it impossible to obtain the egocentric body pose only from the external view. Compared with our optimization approach, the method in~\cite{wang2021estimating} performs worse due to the lack of external-view supervision. 
% It is still possible to use this method to generate 3D poses under egocentric perspective, which can also be used as pseudo labels for training the network. However, this results in worse performance, which is demonstrated in the ablation study (Sec.~\ref{subsec:ablation}).
% \ME{
% L680: "w. Comparing with our optimization approach, the method in [40] performs worse due to the lack of external-view supervision. It is still possible to use this method to generate pseudo label ". If there are no external view supervision, how is trained then ? Just synthetic data ? 
% }



\subsection{Comparisons on 3D Pose Estimation}

\begin{table}[h]
\begin{center}
\small
\begin{tabularx}{0.47\textwidth} { 
   >{\raggedright\arraybackslash}X 
   >{\centering\arraybackslash}X 
   >{\centering\arraybackslash}X  }
\hlineB{2.5}
Method & PA-MPJPE & BA-MPJPE \\
\hline
\multicolumn{2}{l}{\textbf{Wang \etal's test dataset}} \\
\hline
Rhodin \etal~\cite{rhodin2018learning} & 89.67 & 73.56 \\
Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} & 102.3 & 74.46 \\
$x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19} & 112.0 & 87.20 \\
Ours &\textbf{81.71} & \textbf{64.87} \\
\hlineB{2.5}
\multicolumn{2}{l}{\textbf{Mo$^2$Cap$^2$ test dataset}} \\
\hline
Rhodin \etal~\cite{rhodin2018learning} & 97.69 & 76.92 \\
Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} & 91.16 & 70.75 \\
$x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19} & 86.85 & 66.54 \\
Ours & \textbf{83.17} & \textbf{64.33} \\
\hlineB{2.5}
\end{tabularx}
\end{center}
\caption{The experimental results on Wang~\etal's test dataset and Mo$^2$Cap$^2$ test dataset \cite{DBLP:journals/tvcg/XuCZRFST19}. Our method outperforms the state-of-the-art methods, i.e. Mo$^2$Cap$^2$ \cite{DBLP:journals/tvcg/XuCZRFST19} and $x$R-egopose \cite{DBLP:conf/iccv/TomePAB19} on both of the metrics. Our method also outperforms a video-based method~\cite{wang2021estimating} in terms of  PA-MPJPE.
% \vspace{-0.5em}
}
\label{table:main}
\end{table}


We compare our approach with previous single-frame-based methods on the test dataset from~\cite{wang2021estimating} under the ``Wang~\etal's test dataset'' in Table~\ref{table:main}. Since the code or the predictions of $x$R-egopose are not publicly available, we use our reimplementation of $x$R-egopose instead. On this dataset, our method outperforms Mo$^2$Cap$^2$ by 20.1\% and $x$R-egopose by 27.0\% respectively. 
We also compared with previous methods on the Mo$^2$Cap$^2$ test dataset and show the results under the ``Mo$^2$Cap$^2$ test dataset'' in Table~\ref{table:main}. On the Mo$^2$Cap$^2$ test dataset, our method performs better than Mo$^2$Cap$^2$ and $x$R-egopose by 8.8\% and 4.2\%, respectively.

% We also compared with previous methods on the Mo$^2$Cap$^2$ test dataset in Table~\ref{table:main}. Since the camera parameters used in Mo$^2$Cap$^2$ are different from those used in this work, we train our network on the unlabeled dataset from the Mo$^2$Cap$^2$ work. Since the external view is not available for the Mo$^2$Cap$^2$ test dataset, we generate the pseudo labels with the optimize equation~\ref{eq:optim} without $E_{R}^{ext}$, $E_{J}^{ext}$, $E_{C}$, and $E_{M}$. Next, we follow Sec.~\ref{subsec:train} to train the pose estimation network on the Mo$^2$Cap$^2$ test dataset and show the results under the ``Mo$^2$Cap$^2$ test dataset'' in Table~\ref{table:main}. Our method performs better than Mo$^2$Cap$^2$ and $x$R-egopose by 10.4\% and 6.0\% respectively on Mo$^2$Cap$^2$ test dataset.

From the results in Table~\ref{table:main}, we can see that our approach outperforms all previous methods on the single-frame egocentric pose estimation task. More quantitative results on each type of motion are available in the supplementary material. For the qualitative comparison, we show the results of our method on the studio dataset and in-the-wild dataset in Fig.~\ref{fig:results}. Our method performs much better compared with Mo$^2$Cap$^2$ and $x$R-egopose, especially for the in-the-wild cases where the body parts are occluded. Please refer to the supplementary materials for more qualitative results.

We also compared our method with Rhodin~\etal's method~\cite{rhodin2018learning}, which leverages the weak supervision from multiple views to supervise the training of a single view pose estimation network. In our EgoPW dataset, we only have one egocentric and one external view. Thus, we fix the 3D pose estimation network for the external view and only train the egocentric pose estimation network. Following Rhodin~\etal~\cite{rhodin2018learning}, we align the prediction from the egocentric and external view with Procrustes analysis and calculate the loss proposed by Rhodin~\etal. Our result in Table~\ref{table:main} shows that the performance of our method is better. This is mainly because our spatio-temporal optimization method predicts accurate and temporally stable 3D poses as pseudo labels, while other methods suffer seriously from inaccurate egocentric pose estimations.


\subsection{Ablation Study}\label{subsec:ablation}

\begin{table}[h]
\begin{center}
\small
\begin{tabular}{p{0.2\textwidth}
>{\centering}p{0.1\textwidth}
>{\centering\arraybackslash}p{0.1\textwidth}}
\hlineB{2.5}
Method & PA-MPJPE & BA-MPJPE \\ 
\hline
% Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} & 102.3 & 74.46 \\
% $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19} & 112.0 & 87.20 \\
% \hline
w/o external view  & 90.05 & 68.99 \\
w/o learning representation  & 85.46 & 67.01 \\
w/o domain adaptation  & 84.22 & 66.48 \\
Unsupervised DA  & 91.56 & 69.17 \\
\hline
Ours & \textbf{81.71} & \textbf{64.87}\\
\hlineB{2.5}
\end{tabular}
\end{center}
\caption{The quantitative results of ablation study.}
\label{table:ablation}
% \vspace{-1em}
\end{table}

% In this section, we conduct experiments to further evaluate the effects of individual components in our approach. 
\paragraph{Supervision from the external view.}
In our work, we introduce the external view as supervision for training the network on the real EgoPW dataset. The external view enables generating accurate pseudo labels, especially when the human body parts are occluded in the egocentric view but can be observed in the external view. Without the external view, the obtained pseudo labels are less accurate and will further affect the network performance. In order to demonstrate this, 
% we compare the pseudo labels generated with our method and the egocentric 3D poses generated with Wang~\etal's method~\cite{wang2021estimating}, which can also be used for training pose estimation network. 
we firstly generate the 3D poses as pseudo labels with Wang~\etal's method, \ie without any external supervision, and then train the pose estimation network on these new pseudo labels.
% we first generate the pseudo labels without any external supervision, \ie run our optimizer without $E_{R}^{ext}$, $E_{J}^{ext}$, $E_{C}$, and $E_{M}$, and then train the pose estimation network on this new pseudo labels. 
The result is shown in the ``w/o external view'' row of Table~\ref{table:ablation}. We also show the qualitative results with and without external-view supervision in Fig.~\ref{fig:wo_external}. Both the qualitative and quantitative results demonstrate that with the external supervision, the performance of our pose estimation network is significantly better especially on occluded cases.
% \ME{
% In L790 it states: "e. In order to demonstrate this, we first generate the pseudo labels without any external supervision, i.e. run our optimizer without Eext R , EJext, EC, and EM , and then train the pose estimation network on this new pseudo labels." --> how is it even possible to train the proposed method on real data without external views ? You must have external supervision, either in-the-wild settings or in the studio. Right ? Please clarify this. 
% }

\begin{figure}
\centering
\includegraphics[width=0.98\linewidth]{figures/wo_external/wo_external_crop.pdf}
\caption{The results of our method with (c) and without external view (b). The network cannot predict accurate poses for the occluded cases without the external view supervision. 
The external view is only for visualization and not used for predicting the pose.
}
\label{fig:wo_external}
\vspace{-0.2em}
\end{figure}



% \paragraph{Learning semantic representation of egocentric human body images.}
% In our work, we train the egocentric pose estimation network by learning the semantic representation from egocentric human body images (Sec.~\ref{subsubsec:ext_adv}). In order to demonstrate the effectiveness of learning the semantic representation of human body, we removed the domain classifier $Gamma$ in our training process. We show the quantitative results in the row of ``w/o learning representation'' in Table~\ref{table:ablation}. After removing the domain classifier between egocentric and external view, our method suffers from performance drop, which demonstrates the necessity of this module.

% \paragraph{Adversarial domain adaptation strategy.}
% In our work, we train the pose estimation network on the synthetic images and in-the-wild images with the adversarial domain adaptation module (Sec.~\ref{subsubsec:da}). With a domain classifier, this module eliminates the domain gap and enables the full use of both the synthetic and real images.
% In order to investigate the efficacy of this strategy, we removed the domain classifier in our training framework and train the network without $L_{D}$. We evaluate this network on Wang~\etal's dataset and show the quantitative results in the row of ``w/o domain adaptation'' in Table~\ref{table:ablation}. After removing the domain classifier between synthetic and real images, our method suffers from performance drop, which demonstrates the effectiveness of domain adaptation module in our method.

% \JW{Maybe combine these two ablation studies?}

\paragraph{Learning egocentric feature representation and bridging the domain gap with adversarial training.} 
In our work, we train the pose estimation network with two adversarial components in order to learn the feature representation of the egocentric human body (Sec.~\ref{subsubsec:ext_adv}) and bridge the domain gap between synthetic and real images (Sec.~\ref{subsubsec:da}). In order to demonstrate the effectiveness of both modules, we removed the domain classifier $\Lambda$ in our training process and show the results in the row of ``w/o learning representation'' in Table~\ref{table:ablation}. We also removed the domain classifier $\Gamma$, train the network without $L_{D}$ and show the quantitative results in the row of ``w/o domain adaptation'' in Table~\ref{table:ablation}. After moving any of the two components, our method suffers from the performance drop, which demonstrates the effectiveness of both the feature representation learning module and the domain adaptation module.

\paragraph{Comparison with only using unsupervised domain adaptation.}
In this experiment, we compare our approach with the unsupervised adversarial domain adaptation method~\cite{tzeng2017adversarial} which is commonly used for transfer learning tasks. We train the network only with the $L_S$ and $L_D$ in the adversarial domain adaptation module (Sec.~\ref{subsubsec:da}) and show the results in the ``Unsupervised DA'' of the Table~\ref{table:ablation}. Our approach outperforms the unsupervised domain adaptation method due to our high-quality pseudo labels. 





==> Estimating Egocentric 3D Human Pose in the Wild-CVPR2022/sections/intro_new.tex <==
\section{Introduction}

% \ME{make sure that the '' semantic representation '' termonolgy is fixed during the paper. I think it is sometimes used interchangibly with '' features of extracted images ''. }

Egocentric motion capture using head- or body-mounted cameras has recently become popular, because traditional motion capture systems with outside-in cameras have limitations when the person is moving around in a large space and thus restrict the scope of applications. Different from traditional  systems, the egocentric motion capture system is mobile, flexible, and has no requirements on recording space, which enables capturing a wide range of human activities for many applications, such as wearable medical monitoring, sports analysis, and $x$R.  

\begin{figure}
\begin{center}
\includegraphics[width=0.97\linewidth]{figures/teaser/teaser_with_external_red_crop.pdf}
\end{center}
   \caption{Comparing with Mo$^2$Cap$^2$, our method gets a more accurate egocentric pose from a single in-the-wild image, especially when the body parts are occluded. Note that the external images are only used for visualization and the 3D poses in this figure are only generated from the egocentric images.}
\label{fig:teaser}
\end{figure}

In this work, we focus on estimating the full 3D body pose with a single head-mounted fisheye camera. The most related works to ours are Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} and $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19}. 
While these methods have produced compelling results they are only trained on the synthetic data as limited real data exists and therefore suffer from significant performance drop on real data due to the domain gap between synthetic and real images.
Furthermore, due to the similar reason, these methods often struggle with the cases when the human body is occluded by or interacting with the surrounding scene (See the Mo$^2$Cap$^2$ results in Fig.~\ref{fig:teaser}).
% mainly because the training supervision is only from a single egocentric view.

To address the limited data issue, we capture a large-scale in-the-wild egocentric dataset called \emph{Egocentric Poses in the Wild (EgoPW)}. This dataset is the largest egocentric in-the-wild dataset, containing more than 312k frames and covering 20 different daily activities in 8 everyday scenes. To improve the accuracy of the estimated poses from a single egocentric image, one possible way is to use a multi-view camera setup to capture training data to obtain a ground truth 3D body pose or apply multi-view weak supervision. However, this setup is impractical for recording in an environment with limited space (e.g. in the small kitchen shown in Fig.~\ref{fig:optimization_example}), which is a common recording scenario. Therefore, considering a balance between flexibility and data quality, we used a new device setup consisting of an egocentric camera and a single auxiliary external camera. The extra external view could provide additional supervision during training, especially on the occluded regions in the egocentric view (e.g. the lower body part). 

We then propose a new egocentric pose estimation method for training on the EgoPW dataset in a weakly supervised way. Specifically, we propose a spatio-temporal optimization method to generate accurate 3D poses for each frame in the EgoPW dataset. The generated poses are further used as pseudo labels for training an egocentric pose estimation network~\cite{DBLP:journals/tvcg/XuCZRFST19}. To improve the estimation accuracy, we propose an adversarial training strategy based on the observation that the feature representation of human body from the egocentric view and external view should contain similar parts. Specifically, we enforce the feature distribution extracted from these two views to be consistent by fooling a discriminator not being able to detect which views the features are from. 
To further improve the performance of pose estimation network, besides the EgoPW dataset, we also use a synthetic dataset~\cite{DBLP:journals/tvcg/XuCZRFST19} to train the egocentric pose estimation network and adopt a domain adaptation strategy to minimize the domain gap between synthetic and real data. 

% We then propose a new egocentric pose estimation method for training on the EgoPW dataset in a weakly supervised way. Specifically, we propose a spatio-temporal optimization method to generate accurate 3D poses for each frame in the EgoPW dataset. The generated poses are further used as pseudo labels for training an egocentric pose estimation network~\cite{DBLP:journals/tvcg/XuCZRFST19}. To improve the estimation accuracy, we propose an adversarial training strategy based on the observation that the feature representation of human body from the egocentric view and external view should be similar. Specifically, we enforce the features extracted from these two views to be consistent by fooling a discriminator not being able to detect which views the features are from. 
% To further improve the performance of pose estimation network, besides the EgoPW dataset, we also use a synthetic dataset~\cite{DBLP:journals/tvcg/XuCZRFST19} to train the egocentric pose estimation network and adopt a domain adaptation strategy to minimize the domain gap between synthetic and real data. 

% In order to leverage the supervision from both the external view and egocentric view, we generate pseudo labels by developing a new spatio-temporal optimization method that leverages the 2D and 3D keypoints detected from the two views. The pseudo labels are then used to train the pose estimation network. We note that the external view is only used for training, but not for testing. 
% \JW{To further improve the accuracy of the estimated poses, we introduce a new adversarial training strategy by aligning the semantic representation of egocentric and external images.
% We also use synthetic dataset to train our network and adopt a domain adaptation strategy that minimizes the domain gap. The network trained with our method gives accurate 3D pose even under serious occlusions (See our results in Figure~\ref{fig:teaser}).}

% \JW{Since the corresponding egocentric and external images share the same identity and body pose, the intermediate features of them should also share the same semantic representation. Aside from optimizing the pseudo labels, we introduce a new adversarial learning strategy to align the feature representation and supervise the training of egocentric pose estimation network.}

% \JW{To further improve the accuracy of the estimated poses, we also adopt a domain adaptation strategy that minimizes the domain gap between synthetic and real dataset, and a bootstrapping strategy that optimize pseudo labels and the pose estimation network in a loop. The network trained with our method gives accurate 3D pose even under serious occlusions (See our results in Figure~\ref{fig:teaser}). }

We evaluate our method on the test data provided by Wang~\etal~\cite{wang2021estimating} and Xu~\etal~\cite{DBLP:journals/tvcg/XuCZRFST19}. Our method significantly outperforms the state-of-the-art methods both quantitatively and qualitatively. We also show qualitative results on various in-the-wild images, demonstrating that our method can predict accurate 3D poses in the in-the-wild scenes, especially when the body joints are seriously occluded (See our results in Figure~\ref{fig:teaser}). To summarize, our contributions are:

\begin{itemize}
\itemsep -0.1em
    % \item A new approach to estimating accurate 3D human poses from a single in-the-wild egocentric image;
    \item A new learning approach for egocentric human pose estimation by leveraging supervision from an external view;
    % \item \DL{The first contribution is very important and it should be more specific. A new method that does X is a quite general statement. I believe we should state here that we propose a new learning method/framework for egocentric human pose estimation that leverages information from external views for improving the feature representation.}
    \item A large-scale in-the-wild egocentric dataset (EgoPW) captured with a head-mounted fisheye camera and an external normal camera. We will make this dataset publicly available;
    \item A new optimization method to generating the pseudo labels for the in-the-wild dataset by incorporating the supervision from the external view;
    \item  An adversarial method for training the network by learning the feature representation of egocentric images with external feature representation. 
    \LJ{A new efficient strategy for learning egocentric feature representation with the supervision from the high-quality features extracted by a pretrained model trained on a large amount of external-view data. }
    % \item  An adversarial learning method to enforcing the features of body parts from the egocentric view and external view to be consistent. \DL{this contribution is somehow in the first, so it could be emphasized there and removed from here. Instead, you could claim SotA results on two datasets}
\end{itemize}


==> Estimating Egocentric 3D Human Pose in the Wild-CVPR2022/sections/introduction.tex <==
\section{Introduction}

% \ME{make sure that the '' semantic representation '' termonolgy is fixed during the paper. I think it is sometimes used interchangibly with '' features of extracted images ''. }

Egocentric motion capture using head- or body-mounted cameras has recently become popular because traditional motion capture systems with outside-in cameras have limitations when the person is moving around in a large space and thus restrict the scope of applications. Different from traditional systems, the egocentric motion capture system is mobile, flexible, and has no requirements on recording space, which enables capturing a wide range of human activities for many applications, such as wearable medical monitoring, sports analysis, and $x$R.  

\begin{figure}
\begin{center}
\includegraphics[width=0.97\linewidth]{figures/teaser/teaser_with_external_red_crop.pdf}
\end{center}
   \caption{Compared with Mo$^2$Cap$^2$, our method gets a more accurate egocentric pose from a single in-the-wild image, especially when the body parts are occluded. Note that the external images are only used for visualization, not the inputs to our method.}
%   \caption{Comparing with Mo$^2$Cap$^2$, our method gets a more accurate egocentric pose from a single in-the-wild image, especially when the body parts are occluded. Note that the external images are only used for visualization and the 3D poses in this figure are only generated from the egocentric images.\LJ{-> ...for visualization and they are not the inputs to our method. }}
\label{fig:teaser}
\end{figure}

In this work, we focus on estimating the full 3D body pose from a single head-mounted fisheye camera. The most related works are Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} and $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19}. 
While these methods have produced compelling results, they are only trained on synthetic images as limited real data exists and, therefore, suffer from significant performance drop on real-world scenarios.
Furthermore, these methods often struggle with the cases when parts of the human body are occluded by or interacting with the surrounding scene (see the Mo$^2$Cap$^2$ results in Fig.~\ref{fig:teaser}).
% mainly because the training supervision is only from a single egocentric view.
This is due to the domain gap between synthetic and real data, but also due to their limited capability of handling occlusions.
% , which we propose to tackle with a weak external supervision \LJ{remove "which ...."}.

To address the issue of the limited real egocentric data, we capture a large-scale in-the-wild egocentric dataset called \emph{Egocentric Poses in the Wild (EgoPW)}. This is currently the largest egocentric in-the-wild dataset, containing more than 312k frames and covering 20 different daily activities in 8 everyday scenes. To obtain the supervision for the network training, one possibility is using a multi-view camera setup to capture training data with ground truth 3D body poses or apply multi-view weak supervision.
% To address the issue of limited real data, we capture a large-scale in-the-wild egocentric dataset called \emph{Egocentric Poses in the Wild (EgoPW)}. This dataset is the largest egocentric in-the-wild dataset, containing more than 312k frames and covering 20 different daily activities in 8 everyday scenes. To improve the accuracy of the \DL{estimated poses $\rightarrow$ reference poses ?} from a single egocentric image, one possible way is to use a multi-view camera setup to capture training data with ground truth 3D body poses or apply multi-view weak supervision.
%
% \DL{Here it is not clear if we are talking about the estimated poses from our final method or if we are talking about the pseudo labels generated for the dataset. If it is the first case, it is indeed confusing, because the paragraph is introducing the dataset and not the method}.
%
However, this setup is impractical for recording in an environment with limited space (e.g. in the small kitchen shown in Fig.~\ref{fig:optimization_example}), which is a common recording scenario. Therefore, considering a trade-off between flexibility and 3D accuracy, we use a new device setup consisting of an egocentric camera and a single auxiliary external camera. We demonstrate that the external view can provide additional supervision during training, especially for the highly occluded regions in the egocentric view (e.g. the lower body part). 

% Considering the limitations of existing methods and the new EgoPW dataset, \LJ{-> To handle occlusions and achieve accurate pose estimation, }we propose a new egocentric pose estimation method for training on the EgoPW dataset in a weakly supervised way.
To handle occlusions and estimate accurate poses, we propose a new egocentric pose estimation method for training on the EgoPW dataset in a weakly supervised way.
Specifically, we propose a spatio-temporal optimization method to generate accurate 3D poses for each frame in the EgoPW dataset. The generated poses are further used as pseudo labels for training an egocentric pose estimation network~\cite{DBLP:journals/tvcg/XuCZRFST19}. To improve the network performance, we facilitate the training of the egocentric pose estimation network with the extracted features from the external pose estimation network which has been trained on a large in-the-wild body pose dataset. 
% To improve the estimation accuracy, we facilitate the training of egocentric pose estimation network with the extracted features from the external view based on the observation that the egocentric and external view share the same identity and pose. 
% we propose an adversarial training strategy based on the observation that the feature representation of human body from the egocentric view and external view should contain similar parts. 
Specifically, we enforce the feature extracted from these two views to be similar by fooling a discriminator not being able to detect which view the features are from. 
To further improve the performance of the pose estimation network, besides the EgoPW dataset, we also use a synthetic dataset~\cite{DBLP:journals/tvcg/XuCZRFST19} to train the network and adopt a domain adaptation strategy to minimize the domain gap between synthetic and real data. 


% \DL{Considering the aforementioned limitations of existing methods and the newly collected EgoPW dataset, we propose...}
% \JW{We then propose a new egocentric pose estimation method for training on the EgoPW dataset in a weakly supervised way. Specifically, we propose a spatio-temporal optimization method to generate accurate 3D poses for each frame in the EgoPW dataset. The generated poses are further used as pseudo labels for training an egocentric pose estimation network~\cite{DBLP:journals/tvcg/XuCZRFST19}. To improve the estimation accuracy, we facilitate the training of egocentric pose estimation network with the extracted features from the external view based on the observation that the egocentric and external view share the same identity and pose. 
% % we propose an adversarial training strategy based on the observation that the feature representation of human body from the egocentric view and external view should contain similar parts. 
% Specifically, we enforce the feature extracted from these two views to be similar by fooling a discriminator not being able to detect which views the features are from. 
% To further improve the performance of pose estimation network, besides the EgoPW dataset, we also use a synthetic dataset~\cite{DBLP:journals/tvcg/XuCZRFST19} to train the network and adopt a domain adaptation strategy to minimize the domain gap between synthetic and real data. }

% We then propose a new egocentric pose estimation method for training on the EgoPW dataset in a weakly supervised way. Specifically, we propose a spatio-temporal optimization method to generate accurate 3D poses for each frame in the EgoPW dataset. The generated poses are further used as pseudo labels for training an egocentric pose estimation network~\cite{DBLP:journals/tvcg/XuCZRFST19}. To improve the estimation accuracy, we propose an adversarial training strategy based on the observation that the feature representation of human body from the egocentric view and external view should be similar. Specifically, we enforce the features extracted from these two views to be consistent by fooling a discriminator not being able to detect which views the features are from. 
% To further improve the performance of pose estimation network, besides the EgoPW dataset, we also use a synthetic dataset~\cite{DBLP:journals/tvcg/XuCZRFST19} to train the egocentric pose estimation network and adopt a domain adaptation strategy to minimize the domain gap between synthetic and real data. 

% In order to leverage the supervision from both the external view and egocentric view, we generate pseudo labels by developing a new spatio-temporal optimization method that leverages the 2D and 3D keypoints detected from the two views. The pseudo labels are then used to train the pose estimation network. We note that the external view is only used for training, but not for testing. 
% \JW{To further improve the accuracy of the estimated poses, we introduce a new adversarial training strategy by aligning the semantic representation of egocentric and external images.
% We also use synthetic dataset to train our network and adopt a domain adaptation strategy that minimizes the domain gap. The network trained with our method gives accurate 3D pose even under serious occlusions (See our results in Figure~\ref{fig:teaser}).}

% \JW{Since the corresponding egocentric and external images share the same identity and body pose, the intermediate features of them should also share the same semantic representation. Aside from optimizing the pseudo labels, we introduce a new adversarial learning strategy to align the feature representation and supervise the training of egocentric pose estimation network.}

% \JW{To further improve the accuracy of the estimated poses, we also adopt a domain adaptation strategy that minimizes the domain gap between synthetic and real dataset, and a bootstrapping strategy that optimize pseudo labels and the pose estimation network in a loop. The network trained with our method gives accurate 3D pose even under serious occlusions (See our results in Figure~\ref{fig:teaser}). }

We evaluate our method on the test data provided by Wang~\etal~\cite{wang2021estimating} and Xu~\etal~\cite{DBLP:journals/tvcg/XuCZRFST19}. Our method significantly outperforms the state-of-the-art methods both quantitatively and qualitatively. We also show qualitative results on various in-the-wild images, demonstrating that our method can predict accurate 3D poses on very challenging scenes, especially when the body joints are seriously occluded (see our results in Fig.~\ref{fig:teaser}). To summarize, our contributions are presented as follows:

\begin{itemize}
\itemsep -0.1em
    % \item A new approach to estimating accurate 3D human poses from a single in-the-wild egocentric image;
    % \item A new learning method for estimating egocentric human pose by leveraging weak supervision from an external view;
    \item A new method to estimate egocentric human pose with weak supervision from an external view, which significantly outperforms existing methods on in-the-wild data, especially when severe occlusions exist;
    % and significantly outperforms existing methods. 
    % \item \DL{The first contribution is very important and it should be more specific. A new method that does X is a quite general statement. I believe we should state here that we propose a new learning method/framework for egocentric human pose estimation that leverages information from external views for improving the feature representation.}
    \item A large in-the-wild egocentric dataset (EgoPW) captured with a head-mounted fisheye camera and an external camera. We will make it publicly available;
    \item A new optimization method to generating pseudo labels for the in-the-wild egocentric dataset by incorporating the supervision from an external view; 
    % \DL{make sure to refer to ''pseudo labels`` in the paragraph were that introduces EgoPW}
    \item  An adversarial method for training the network by learning the feature representation of egocentric images with external feature representation. 
    % \item  An adversarial learning method to enforcing the features of body parts from the egocentric view and external view to be consistent. \DL{this contribution is somehow in the first, so it could be emphasized there and removed from here. Instead, you could claim SotA results on two datasets}
\end{itemize}


==> Estimating Egocentric 3D Human Pose in the Wild-CVPR2022/sections/method.tex <==
\section{Method}
We propose a new approach to train a neural network on the in-the-wild dataset with weak supervision from egocentric and external views.
% We could skip this phrase if it was already stressed in the intro >>
% This network is able to estimate an accurate 3D body pose from a single egocentric in-the-wild image.
The overview of our approach is illustrated in Fig.~\ref{fig:framework}. We first capture a large-scale egocentric in-the-wild dataset, called \emph{EgoPW}, which contains synchronized egocentric and external image sequences (Sec.~\ref{subsec:dataset}). Next, we generate pseudo labels for the EgoPW dataset with an optimization-based framework. This framework takes as input a sequence in a time window with $B$ frames of egocentric images $\mathcal{I}^{ego}_{seq}=\{\mathcal{I}^{ego}_{1},\dots,\mathcal{I}^{ego}_{B}\}$ and external images $\mathcal{I}^{ext}_{seq}=\{\mathcal{I}^{ext}_{1},\dots,\mathcal{I}^{ext}_{B}\}$ and outputs egocentric 3D poses $\mathcal{P}^{ego}_{seq}=\{\mathcal{P}^{ego}_{1},\dots,\mathcal{P}^{ego}_{B}\}$ as the pseudo labels (Sec.~\ref{subsec:optimizer}). 
% \ME{
% L326-330: "rst large-scale in-the-wild human performance dataset captured by an egocentric camera and an external normal camera (Sony RX0) w"
% --> please clearly explain how the cameras are synchronized ? software sync ? hardware sync ? is there a drift ? how do you handle it? what is the impact of the sync ?
% }
% \JW{Comment: add the way to do synchronize in the supplementary material}
Next, we train the egocentric pose estimation network on the synthetic data from Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19}
% ~\DL{from where this synthetic data comes from?}
and on the EgoPW dataset with pseudo labels $\mathcal{P}^{ego}_{seq}$.
% \DL{Here synthetic+EgoPW are mentioned as training data, but in Fig. 1 it says Mo$^2$Cap$^2$+EgoPW. Check which is correct}. 
In the training process, we leverage the feature representation from an on-the-shelf external pose estimation network~\cite{xiao2018simple} to enforce our egocentric network to learn a better feature representation
%supervise the training of egocentric pose estimation network
in an adversarial way (Sec.~\ref{subsubsec:ext_adv}). We also use an adversarial domain adaptation strategy to mitigate the domain gap between synthetic and real datasets (Sec.~\ref{subsubsec:da}).


\subsection{EgoPW Dataset}\label{subsec:dataset}

We first describe the newly collected \emph{EgoPW} dataset, which is the first large-scale in-the-wild human performance dataset captured by an egocentric camera and an external camera (Sony RX0), both synchronized.
EgoPW contains a total of 318k frames, which are divided into 97 sequences of 10 actors in 20 clothing styles performing 20 different actions, including
%
\textit{reading magazine/newspaper},
\textit{playing board games},
\textit{doing a presentation},
\textit{walking},
\textit{sitting down},
\textit{using a computer},
\textit{calling on the phone},
\textit{drinking water},
\textit{writing on the paper},
\textit{writing on the whiteboard},
\textit{making tea},
\textit{cutting vegetables},
\textit{stretching},
\textit{running},
\textit{playing table tennis},
\textit{playing baseball},
\textit{climbing floors},
\textit{dancing},
\textit{opening the door}, and
\textit{waving hands}. All personal data is collected with an IRB approval.
We generate 3D poses as pseudo labels using the egocentric and external images, which will be elaborated later. 
In terms of size, our EgoPW dataset is larger than existing in-the-wild 3D pose estimation datasets, like 3DPW~\cite{von2018recovering}, and has similar scale to the existing synthetic egocentric datasets, including the  Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} and the $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19} datasets. 

\subsection{Optimization for Generating Pseudo Labels}\label{subsec:optimizer}

In this section, we present an optimization method based on \cite{wang2021estimating} to generate pseudo labels for EgoPW.
%
Given a sequence, we split it into segments containing $B$ consecutive frames. 
For the egocentric frames $I^{ego}_{seq}$, we estimate the 3D poses represented by 15 joint locations in the coordinate system of the egocentric camera (called ``egocentric poses")  $\widetilde{\mathcal{P}}^{ego}_{seq}=\{\widetilde{\mathcal{P}}^{ego}_1,\dots,\widetilde{\mathcal{P}}^{ego}_B \}$, $\widetilde{\mathcal{P}}^{ego}_i \in \mathbb{R}^{15{\times}3}$, and 2D heatmaps $H^{ego}_{seq}=\{H^{ego}_1,\dots,H^{ego}_B \}$ using the Mo$^2$Cap$^2$ method \cite{DBLP:journals/tvcg/XuCZRFST19}.
Aside from egocentric poses, we also estimate the transformation matrix between the egocentric camera poses of two adjacent frames $[R_{seq}^{SLAM} \mid t_{seq}^{SLAM}] = \{[R_1^2 \mid t_1^2], \dots, [R_{B-1}^{B} \mid t_{B-1}^B]\}$ using ORB-SLAM2~\cite{murTRO2015}.
For the external frames $I^{ext}_{seq}$, we estimate the 3D poses (called ``external poses") $\mathcal{P}^{ext}_{seq}=\{\mathcal{P}^{ext}_1,\dots,\mathcal{P}^{ext}_B \}$, $\mathcal{P}^{ext}_i \in \mathbb{R}^{15 \times 3}$ using VIBE~\cite{DBLP:conf/cvpr/KocabasAB20} and 2D joints $\mathcal{J}^{ext}_{seq}=\{\mathcal{J}^{ext}_1,\dots,\mathcal{J}^{ext}_B \}$, $\mathcal{J}^{ext}_i \in \mathbb{R}^{15 \times 2}$ using openpose~\cite{cao2017realtime}. 

Next, following \cite{wang2021estimating}, we learn a latent space to encode an egocentric motion prior with a sequential VAE which consists of a CNN-based encoder $f_{enc}$ and decoder $f_{dec}$. We then optimize the egocentric pose by finding a latent vector $z$ such that the corresponding pose sequence $P^{ego}_{seq} = f_{dec}(z)$ minimizes the objective function:

\begin{equation}
\begin{aligned}
	E (\mathcal{P}_{seq}^{ego}, R_{seq}, t_{seq}) &= \lambda_R^{ego} E_{R}^{ego} + \lambda_R^{ext} E_{R}^{ext} + \lambda_J^{ego} E_{J}^{ego} \\
	& +  \lambda_J^{ext} E_{J}^{ext} + \lambda_T E_{T} + \lambda_B E_{B}\\
	& + \lambda_C E_{C} + \lambda_M E_{M}.
	\label{eq:optim}
\end{aligned}
\end{equation}
In this objective function, $E_{R}^{ego}$, $E_{J}^{ego}$,$E_{T}$, and $E_{B}$ are egocentric reprojection term, egocentric pose regularization term, motion smoothness regularization term and bone length regularization term, which are the same as those defined in~\cite{wang2021estimating}.
%
$E_{R}^{ext}$, $E_{J}^{ext}$, $E_{C}$, and $E_{M}$ are the external reprojection term, external 3D body pose regularization term, camera pose consistency term, and camera matrix regularization term, which will be described later. 
%
Please see the supplemental material for a detailed definition of each term.

Note that since the relative pose between external camera and egocentric camera is unknown, we also need to optimize the relative egocentric camera pose with respect to the external camera pose for each frame, i.e. the rotations  $R_{seq} = {R_1,\dots,R_B}$ and translations $t_{seq} = {t_1,\dots,t_B}$.

\vspace{-0.2em}
\paragraph{External Reprojection Term.}
In order to supervise the optimization process with the external 2D pose, we designed the external reprojection term which minimizes the difference between the projected 3D pose with the external 2D joints.
% \DL{Need a to contextualize here. What are we doing here and why?}
% We use the external 2D detection as a supervision in the optimization framework. 
The energy term is defined as:
\begin{equation}
    E_{R}^{ext}(\mathcal{P}_{seq}^{ego}, R_{seq}, t_{seq}) = \sum_{i=1}^{B}\left\Vert \mathcal{J}_{i}^{ext} - K\left[R_i\mid t_i\right]\mathcal{P}_{i}^{ego} \right\Vert_2^2,
    \label{eq:ext_reproj}
\end{equation}
where $K$ is the intrinsic matrix of the external camera; $\left[R_{i} \mid t_{i} \right]$ is the pose of the egocentric camera in the $i$ th frame
w.r.t the external camera position.
% \DL{small change here (mine), is it correct?}.
% in the external camera space \DL{space -> positio}.
In Eq.~\ref{eq:ext_reproj}, we first project the egocentric body pose $\mathcal{P}_{i}^{ego}$ to the 2D body pose in the external view with the egocentric camera pose $\left[R_{i} \mid t_{i} \right]$ and the intrinsic matrix $K$, and then compare the projected body pose with the 2D joints estimated by the openpose~\cite{cao2017realtime}. Since the relative pose between the external camera and egocentric camera are unknown at the beginning of the optimization, we optimize the egocentric camera pose $\left[R_{i} \mid t_{i} \right]$ simultaneously while optimizing the egocentric body pose $\mathcal{P}_{seq}^{ego}$.
In order to make the optimization process converge faster, we initialize the egocentric camera pose $\left[R_{i} \mid t_{i} \right]$ with the Perspective-n-Point algorithm~\cite{Gao2003CompleteSC}.

\vspace{-0.2em}
\paragraph{Camera Pose Consistency.}
We cannot get the accurate 3D pose only with the external reprojection term because the egocentric camera pose and the optimized body pose can be arbitrarily changed without violating the external reprojection constraint.
% We cannot get the accurate 3D body pose only with the external reprojection term because the egocentric camera pose and the optimized body pose can be changed in a coordinated manner without violating the constraint, as long as their relative position remains unchanged. \DL{Could this previous sentence be explained in a different way?}
To alleviate this ambiguity, we introduce the camera consistency term $E_C$ as follows: 
\begin{equation}
\begin{aligned}
    E_{C}(R_{seq}, t_{seq}) & = \sum_{i=1}^{B-1}\left\Vert \begin{bmatrix} R_i  & t_i \\ 0 & 1 \end{bmatrix} \begin{bmatrix} R^{i+1}_i  & t^{i+1}_i \\ 0 & 1 \end{bmatrix} \right.\\
    & - \left. \begin{bmatrix} R_{i+1}  & t_{i+1} \\ 0 & 1 \end{bmatrix}\right\Vert_2,
    \label{eq:consistency}
\end{aligned}
\end{equation}
It enforces the egocentric camera pose at $(i + 1)$ th frame $[R_{i + 1} \mid t_{i + 1}]$ to be consistent with the pose obtained by transforming the egocentric camera pose at the $i$ th frame $[R_{i} \mid t_{i}]$ with the relative pose between the $i$ th and $(i + 1)$ th frame.

\vspace{-0.2em}
\paragraph{External 3D Body Pose Regularization.}
Besides the external reprojection term, we also use the external 3D body poses to supervise the optimization of the egocentric 3D body pose. 
We define the external 3D pose term which measures the difference between the external and the egocentric body poses after a rigid alignment:
% transformed from the egocentric camera space to the external camera space. 
% We make the optimized egocentric pose $\mathcal{P}_{i}^{ego}$ stay close to the external 3D pose estimation $\mathcal{P}_{i}^{ext}$ by defining the term as the difference between the 3D joint locations of egocentric and external view after the rigid alignment:
\begin{equation}
	E_{J}(\mathcal{P}_{seq}^{ego}, \mathcal{P}_{seq}^{ext}) = \sum_{i=1}^{B}\left\Vert \mathcal{P}_{i}^{ext} - \left[R_{i}^{pa}\mid t_{i}^{pa}\right]\mathcal{P}_{i}^{ego} \right\Vert_2^2,
	\label{eq:ext_3d_pose}
\end{equation}
where $\left[R_{i}^{pa} \mid t_{i}^{pa} \right]$ is the transformation matrix calculated with Procrustes analysis, which rigidly aligns the external 3D pose estimation $\mathcal{P}_{i}^{ext}$ and the egocentric 3D pose $\mathcal{P}_{i}^{ego}$.

% With the external reprojection term and external 3D pose regularization term, we are able to generate accurate pseudo labels even though the human body in the egocentric view is seriously occluded, as illustrated in Fig.~\ref{fig:optimization_example}. With the external view, we are able to train the network with the accurate pseudo labels for the in-the-wild images, especially in the occluded cases. 

% We note that only by combining the egocentric view and external view, we can reconstruct accurate pseudo labels since the body parts can be either occluded in the egocentric or external view. 
By combining the body poses estimated from the egocentric view and external view, we can reconstruct more accurate pseudo labels.  
As shown in Fig.~\ref{fig:optimization_example}, the hands of the person are occluded in the external view, resulting in the tracking of the hands failing in the external view (Fig.~\ref{fig:optimization_example}, b), however, the hands can be clearly seen and tracked in the egocentric view (Fig.~\ref{fig:optimization_example}, d); 
on the other hand, the feet cannot be observed in the egocentric view and thus fail to be tracked in this view (Fig.~\ref{fig:optimization_example}, b), but can be easily viewed and tracked in the external view (Fig.~\ref{fig:optimization_example}, d). 
%Thus, either the optimizer with only the egocentric view (second image) or the external pose estimation method like VIBE~\cite{DBLP:conf/cvpr/KocabasAB20} (fourth image) cannot predict accurate pseudo labels. 
By joining the information from both views, we can successfully predict accurate 3D poses as the pseudo labels (Fig.~\ref{fig:optimization_example}, c).  
% combining the egocentric and external view in our optimization framework, we can predict accurate 3D poses as the pseudo labels, which is illustrated in the third image.
We note that the external camera is only used for generating the pseudo labels but at test time, only the egocentric camera is used. 

\begin{figure}
\centering
\includegraphics[width=0.98\linewidth]{figures/optimization_example/optimization_example_crop.pdf}
\caption{Our pseudo label generation method combines the information from both the egocentric view and external view, therefore leading to more accurate pseudo labels (c). Only with the egocentric camera, the feet cannot be observed and well-tracked (b). Only with the external camera, the hands are occluded and result in the wrong result on the hand part (d).
% We note that the external camera is only used in the pseudo label generation for training, which is not used at test time.
}
% or external view is restrictive for predicting accurate 3D poses (the second and fourth image), while our optimization method gives reasonable result (the third image).
\label{fig:optimization_example}
\end{figure}



\paragraph{Camera Matrix Regularization.}
We constrain the camera rotation matrix $R_{i}$ to be orthogonal:

\begin{equation}
	E_{J}(R_{seq}) = \sum_{i=1}^{B}\left\Vert R_{i}^TR_{i} - I \right\Vert_2^2 \label{eq:matrix}.
\end{equation}
% where $det(.)$ is the determinant of the matrix.

Different from previous single-view pose estimation methods which leverages the weak supervision from multiple views~\cite{iqbal2020weakly,rhodin2018learning,wandt2021canonpose,kocabas2019self}, our spatio-temporal optimization method generates the pseudo labels under the guidance of learned motion prior, making it robust to noisy and inaccurate 2D pose estimations which is common for the 2D pose estimation results from the egocentric view.


\subsection{Training Egocentric Pose Estimation Network}\label{subsec:train}

Through the optimization framework in Sec.~\ref{subsec:optimizer}, we can get accurate 3D pose pseudo labels $\mathcal{P}_{seq}^{ego}$ for each egocentric frame in the EgoPW dataset, which is further processed into the 2D heatmap $H_E$ and the distance between joints and egocentric camera $D_E$ with the fisheye camera model \cite{scaramuzza2014omnidirectional} described in supplementary materials. 

Afterward, we train a single-image based egocentric pose estimation network on both the synthetic dataset from Mo$^2$Cap$^2$ and the EgoPW dataset, as shown in the right part of Fig.~\ref{fig:framework}. The pose estimation network contains a feature extractor $\Theta$ which encodes an image into a feature vector and a pose estimator $\Psi$ which decodes the feature vector to 2D heatmaps and a distance vector. The 3D pose can be reconstructed from them with the fisheye camera model. Here, we note the synthetic dataset $S = \{I_S, H_S, D_S\}$ including synthetic images $I_S$ along with their corresponding heatmaps $H_S$ and distance labels $D_S$ from Mo$^2$Cap$^2$ dataset, and the EgoPW dataset $E = \{I_E^{ego}, H_E, D_E, I_E^{ext} \}$ including egocentric in-the-wild images $I_E^{ego}$ along with pseudo heatmaps $H_E$, distance labels $D_E$ and corresponding external images $I_E^{ext}$. 
During the training process, we train the egocentric pose estimation network with two reconstruction loss terms and two adversarial loss terms. The reconstruction losses are defined as the mean squared error (MSE) between the predicted heatmaps/distances  and heatmaps/distances from labels:

% Afterwards, we train a single-image based egocentric pose estimation network on both the synthetic dataset from Mo$^2$Cap$^2$ and the EgoPW dataset, as shown on the right part of Fig.~\ref{fig:framework}. The pose estimation network contains a feature extractor $\Theta$ which encodes an image into a feature vector and a pose estimator $\Psi$ which decodes the feature vector to 2D heatmaps and a 3D pose. Here, we note the synthetic dataset $S = \{I_S, H_S, D_S\}$ which is composed of synthetic images $I_S$ along with their corresponding heatmaps $H_S$ and distance labels $D_S$ from Mo$^2$Cap$^2$ dataset, and the EgoPW dataset $E = \{I_E^{ego}, H_E, D_E, I_E^{ext} \}$ which is composed of egocentric in-the-wild images $I_E^{ego}$ along with pseudo heatmaps $H_E$, distance labels $D_E$ and corresponding external images $I_E^{ext}$. 
% During the training process, we train the egocentric pose estimation network with two reconstruction loss terms and two adversarial loss terms. The reconstruction losses are defined as the mean squared error (MSE) between the predicted heatmaps/distances  and heatmaps/distances from labels.

% After obtaining the pseudo labels for the EgoPW dataset, we train a single-image based egocentric pose estimation network on both the synthetic dataset from Mo$^2$Cap$^2$ and the EgoPW dataset. The pose estimation network contains a feature extractor $\Theta$ which encodes an image into a feature vector and a pose estimator $\Psi$ which decodes the feature vector to a heatmap and a 3D pose. Here, we note the synthetic dataset $S = \{\mathcal{I_S}, \mathcal{H_S}, \mathcal{D_S}\}$ which is composed of synthetic images $\mathcal{I_S}$ along with their corresponding heatmap $\mathcal{H_S}$ and distance labels $\mathcal{D_S}$ from Mo$^2$Cap$^2$ dataset, and the EgoPW dataset $\mathcal{E} = \{ \mathcal{I_E}^{ego}, \mathcal{H_E}, \mathcal{D_E}, \mathcal{I_E}^{ext} \}$ which is composed of egocentric in-the-wild images $\mathcal{I_E}^{ego}$ along with pseudo heatmaps $\mathcal{H_E}$, distance labels $\mathcal{D_E}$ and corresponding external images $\mathcal{I_E}^{ext}$. 
% During the training process, we train the egocentric pose estimation network with two reconstruction loss terms and two adversarial loss terms. The reconstruction loss is defined as the mean squared error (MSE) between the predicted heatmaps/distances and heatmaps/distances from labels.

\begin{equation}
    \begin{aligned}
        L_{S} &= \text{mse}(\hat{H}_{S}, H_{S}) + \text{mse}(\hat{D}_{S}, D_{S})\\
        L_{E} &= \text{mse}(\hat{H}_{E}, H_{E}) + \text{mse}(\hat{D}_{E}, D_{E}),
    \end{aligned}
\end{equation}
where 
\begin{equation}
    \begin{aligned}
        \hat{H}_{S}, \hat{D}_{S} = \Psi(F_{S}),& F_{S} = \Theta(I_{S});\\
        \hat{H}_{E}, \hat{D}_{E} = \Psi(F_{E}^{ego}),& F_{E}^{ego} = \Theta(I_{E}^{ego}).
    \end{aligned}
\end{equation}
% \begin{equation}
%     \begin{aligned}
%         \hat{H}_{S}, \hat{D}_{S} = \Psi(F_{S});& \hat{H}_{E}, \hat{D}_{E} = \Psi(F_{E}^{ego}),
%     \end{aligned}
% \end{equation}
% and
% \begin{equation}
%     \begin{aligned}
%         F_{S} = \Theta(I_{S});& F_{E}^{ego} = \Theta(I_{E}^{ego})
%     \end{aligned}
% \end{equation}
% \DL{I don't see the definition of $H$ and $D$. Also, try to reduce the lines for these equations. Essentially, all these equations are defining a standard L2 loss on the outputs of the network. This should be simpler to explain, or maybe don't need equations at all. Could also help to have the symbols $I_{(.)}$, $\hat{H}_{(.)}$, $\hat{D}_{(.)}$, $\Psi$, $\Theta$ in Fig. \ref{fig:framework}}

Two adversarial losses are separately designed for learning egocentric feature representation and bridging the domain gap between synthetic and real datasets. These two losses are described as follows. 


% \subsubsection{Learning Semantic Representation of Egocentric Human Body}\label{subsubsec:ext_adv}


\subsubsection{Adversarial Domain Adaptation}\label{subsubsec:da}
To bridge the domain gap between the synthetic and real data domains, following Tzeng~\etal~\cite{tzeng2017adversarial}, we introduce an adversarial discriminator $\Gamma$ which takes as input the feature vectors extracted from a synthetic image and an in-the-wild image, and determines if the feature is extracted from an in-the-wild image. 
The adversarial discriminator $\Gamma$ is trained with a cross-entropy loss:

\begin{equation}
    \mathcal{L}_{D} = -E[\log(\Gamma(\mathcal{F_S}))] - E[\log(1 - \Gamma(\mathcal{F_T}))].
\end{equation}

Once the discriminator $\Gamma$ has been trained, the feature extractor $\Theta$ maps the images from different domains to the same feature space such that the classifier $\Gamma$ cannot tell if the features are extracted from synthetic images or real images. Therefore, the pose estimator $\Psi$ can predict more accurate poses for the in-the-wild data. 

% Aside from training the network on the EgoPW dataset, we also train the pose estimation network simultaneously on the synthetic dataset considering that synthetic data has its advantages compared to real data, e.g. it is easily accessible and has large variations on poses and backgrounds. To address the domain gap between the synthetic data and real data, we introduce a new adversarial domain adaptation method. Specifically, we extract the features from the synthetic data and real data and use an adversarial discriminator to distinguish if the feature is from synthetic data or real data. Once trained, the feature extractor would learn to produce the features in the same feature space for synthetic data and real data. In this way, our method is able to make full use of the synthetic data and real data, thus achieving better results. 


\subsubsection{Supervising Egocentric Feature Representation with External View}\label{subsubsec:ext_adv}

% \DL{Following the comments from Mohamed, I would be careful with ''semantic representation``. I think this section could be renamed by something like ''Improving Features Representation with External View`` or something similar}
Although our new training dataset is large, the variation of identities in the dataset is still relatively limited (20 identities) compared with the existing large-scale external-view human datasets (thousands of identities). Generally speaking, the representations learned with these external-view datasets are of higher quality due to the large diversity of the datasets. To further improve the generalizability of our network and prevent overfitting to the training identities, we propose to supervise our egocentric representation by leveraging the high-quality third-person-view features.
From a transfer learning perspective, although following Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19}, our egocentric network is pretrained on the third-person-view datasets, it can easily ``forget'' the learned knowledge while being finetuned on the synthetic dataset. The supervision from third-person-view features can prevent the egocentric features from deviating too much from those learned from large-scale real human images.


% Note that the identity and body pose are exactly the same in a pair of egocentric-external images $\{ I_E^{ego}, I_E^{ext} \}$. Thus, the external view can bring a valuable additional information for supervising the pose and the \textit{features} from the egocentric view.
% Thus, the deep features from the egocentric pose estimation network $F_{E}^{ego}$ and the external pose estimation network $F_{E}^{ext}$ should contain the same semantic representation.
%
% \DL{We should also be very careful with this statement. The actual 3D poses from both views are the same (due to synchronization), but the semantic information on each image $\{ I_E^{ego}, I_E^{ext} \}$ can be very different. It think it would be much safer to say that the external view can bring a valuable additional information for supervising the pose \textit{and} the features from the egocentric view}
%
%Based on this observation, we use the features from external pose estimation network to supervise the egocentric pose estimation network. 
However, directly minimizing the distance between egocentric features $F_{E}^{ego}$ and external features $F_{E}^{ext}$ will not enhance the performance since the intermediate features of the egocentric and external view should be different from each other due to significant difference on the view direction and camera distortions.
%
% \DL{This is also contradicting the first statement. We should re-write this paragraph carefully}
%
To tackle this issue, we use the adversarial training strategy to align the feature representation from egocentric and external networks. Specifically, we use an adversarial discriminator $\Lambda$ which takes the feature vectors extracted from an egocentric image and the corresponding in-the-wild images and predicts if the feature is from egocentric or external images. The adversarial discriminator $\Lambda$ is trained with a cross-entropy loss:
\begin{equation}
    L_{V} = -E[\log(\Lambda(F_E^{ego}))] - E[\log(1 - \Lambda(F_E^{ext}))],
\end{equation}
where $F_{E}^{ext} = \Theta^{ext}(I_{E}^{ext})$ and $\Theta^{ext}$ is the feature extractor of external pose estimation network that shares exactly the same architecture as the egocentric pose estimation network. The parameters of the features extractor $\Theta^{ext}$ and the pose estimator $\Psi^{ext}$ of the external pose estimation network are obtained from the pretrained model in Xiao~\etal's work~\cite{xiao2018simple} and keep fixed during the training process.

Note that the deep layers of the pose estimation network usually represent the global semantic information of the human body~\cite{chu2017multi}, we use the output feature of the 4th res-block of ResNet-50 network~\cite{he2016deep} as the input to the discriminator $\Lambda$. Furthermore, the spatial position of the joints is quite different in the egocentric view and the external view, which will make the discriminator $\Lambda$ easily learn the difference between egocentric and external features. To solve this, we use an average pooling layer in the discriminator $\Lambda$ to spatially aggregate features, thus further eliminating the influence of spatial distribution between egocentric and external images. Please refer to the suppl. mat. for further details.

During the training process, the egocentric pose estimation network is trained to produce the features $F_E^{ego}$ to fool the domain classifier $\Lambda$ such that it cannot distinguish whether the feature is from an egocentric or external image.
%
% To achieve this, the egocentric pose estimation network need to produce features from the egocentric image with similar distribution as the features from corresponding external image, which will helps the network learn.
To achieve this, the egocentric network learns to pay more attention to the relevant parts of the input image,~\ie, the human body, which is demonstrated in Fig.~\ref{fig:feature}. 
% To achieve this, the egocentric pose estimation network need to generate features only with semantic representation of human body and without any other information specific to the egocentric view, since the semantic representation of corresponding egocentric and external images should be the same \DL{This is a strong statement. I would rather say the ego. network should produce features with the same distribution as the external network, which helps in the learning process, as demonstrated by our results...}. 
% This is demonstrated in Figure~\ref{fig:feature}, where the features from egocentric network focus on the representation of human body after the adversarial training process.


\begin{figure}
\centering
\includegraphics[width=0.98\linewidth]{figures/features/feature_crop.pdf}
\caption{The visualization of features with (b) or without (c) the adversarial supervision from external features. By supervising the training of the egocentric network with the feature representation from an external view, the egocentric network is able to focus on extracting the semantic features of the human body.
}
\label{fig:feature}
\end{figure}


==> Estimating Egocentric 3D Human Pose in the Wild-CVPR2022/sections/relatedwork.tex <==
\section{Related Work}


\paragraph{Egocentric 3D full body pose estimation.}
% Recently, more and more works aim at estimating the 3D human body pose from the egocentric camera perspective. \LJ{suggest removing the above sentence}
Rhodin \etal~\cite{DBLP:journals/tog/RhodinRCISSST16} developed the first method to estimate the full-body pose from a helmet-mounted stereo fisheye camera. Cha~\etal~\cite{cha2018fullycapture} presented an RNN-based method to estimate body pose with two pinhole cameras mounted on the head. Xu~\etal~\cite{DBLP:journals/tvcg/XuCZRFST19} introduced a single wide-view fisheye camera setup and proposed a single-frame based egocentric motion capture system. With the same setup, Tome \etal~\cite{DBLP:conf/iccv/TomePAB19} captured the egocentric pose with an auto-encoder network which captures the uncertainty in the predicted heatmaps. In order to further mitigate the effect of image distortions, Zhang~\etal~\cite{zhang2021automatic} proposed an automatic calibration module.  Hwang \etal \cite{Hwang2020} put an ultra-wide fisheye camera on the user's chest and estimate body pose, camera rotation and head pose simultaneously.
Jiang~\etal~\cite{jiang2021egocentric} mounted a front-looking fisheye camera on the user's head and estimated the body and head pose by leveraging the motion of the environment and extremity of the human body.
Wang~\etal~\cite{wang2021estimating} proposed an optimization algorithm to obtain temporally stable egocentric poses with motion prior learned from Mocap datasets.
However, these methods are all trained on synthetic datasets, thus suffering from the performance drop on the real images due to the domain gap and lack of external supervision. Our method, on the contrary, achieves better performance on the in-the-wild scenes. 

\begin{figure*}
\centering
\includegraphics[width=0.96\linewidth]{figures/framework/framework_parts_annot_crop.pdf}
\caption{Overview of our method.
We first collected the new EgoPW dataset (Sec.~\ref{subsec:dataset}), where pseudo labels are generated by a multi-view based optimization method (Sec.~\ref{subsec:optimizer}). We then train our model with the proposed framework (Sec.~\ref{subsec:train}), where the network is simultaneously trained with EgoPW datasets and synthetic data from Mo$^2$Cap$^2$. We enforce the egocentric network to learn a better feature representation from the external view (Sec.~\ref{subsubsec:ext_adv}) and bridge the gap between synthetic and real data with a domain classifier (Sec.~\ref{subsubsec:da}).
%
%We first train a pose estimation network on both the Mo$^2$Cap$^2$ dataset and the EgoPW dataset (Sec.~\ref{subsec:dataset}), where the pseudo labels are generated by a multi-view based optimization method (Sec.~\ref{subsec:optimizer}). Despite training with optimized pseudo labels, we use a discriminator between egocentric view and external view to train the egocentric pose estimation network with the semantic representation from the external pose estimation network (Sec.~\ref{subsubsec:ext_adv}).
%We also bridge the domain gap between the synthetic and real data with an adversarial domain adaptation network (Sec.~\ref{subsubsec:da}).
}
\label{fig:framework}
\end{figure*}


% \paragraph{Domain adaptation for 3D human pose estimation}

% In order to solve the issue of lacking labeled training data for 3D pose estimation, many works first synthesize images with ground truth pose annotation and then introduce a domain adaptation method to bridge the gap between the synthetic and real data.  Chen~\etal~\cite{chen2016synthesizing} proposed a  domain adaptation by introducing a domain mixer to minimize the discrepancy between the features from synthetic and real images. Zhang~\etal~\cite{zhang2019unsupervised} presented an unsupervised adversarial domain adaptation strategy that utilized the synthetic depth images as the source domain. Xu~\etal~\cite{xu2020alleviating} designed a new domain adaptation framework consisting of three different adaptation components for multi-person 3D pose estimation. Different from previous methods which focus on human pose estimation from an external view, our method is the first domain adaptation method for predicting egocentric human body poses. Our method incorporates an adversarial domain adaptation strategy and a bootstrapping strategy, which significantly improves the performance on real images.

%\vspace{-0.3cm}
\paragraph{Pseudo label generation.}
The task of pseudo-labeling~\cite{lee2013pseudo, shi2018transductive,yang2019pseudo} is a semi-supervised learning technique that generates pseudo labels for unlabeled data and uses the generated labels to train a new model. This has been applied in the areas of segmentation~\cite{li2020self,zou2020pseudoseg,zheng2021rectifying,chen2020digging}, pose estimation~\cite{cao2019cross,li2021synthetic,mu2020learning,ludwig2021self} and image classification~\cite{hu2021simple,pham2021meta,arazo2020pseudo}.
Since the pseudo labels may be inaccurate, some methods have been proposed to filter inaccurate labels to increase the labeling stability. Shi~\etal~\cite{shi2018transductive} set confidence levels on unlabeled samples by measuring the sample density. Chen~\etal~\cite{chen2019progressive} enforced the stability of pseudo labels by adopting an easy-to-hard transfer strategy. Wang and Wu~\cite{wang2020repetitive} introduced a repetitive re-prediction strategy to update the pseudo labels, while Rizve~\etal~\cite{rizve2021defense} proposed an uncertainty-aware pseudo-label selection framework that selects pseudo labels. Morerio~\etal~\cite{morerio2020generative} used a conditional GAN to filter the noise in the pseudo labels.
Different from previous pseudo-labeling works which generate the labels from network predictions or clustering, we design an optimization framework to generate labels with supervision from egocentric and external views simultaneously. 

%\vspace{-0.3cm}
\paragraph{Weakly Supervised 3D Human Pose Estimation.}
Recently, there is a growing interest in developing weakly-supervised 3D pose estimation methods. Weakly-supervised methods do not require datasets with paired images and 3D annotations. Some works~\cite{wang2019distill,novotny2019c3dpo} leverages the non-rigid SFM to get 3D joint positions from 2D keypoint annotations in unconstrained images. Some works~\cite{drover2018can,chen2019unsupervised,wandt2019repnet,pavllo20193d,chen2019weakly} present an unsupervised learning approach to train the 3D pose estimation network with the supervision from 2D reprojections. The closest to our work are the approaches of~\cite{iqbal2020weakly,rhodin2018learning,wandt2021canonpose,kocabas2019self} in that they leverage the weak supervision from multi-view images for training. 
Iqbal~\etal~\cite{iqbal2020weakly} and Rhodin~\etal~\cite{rhodin2018learning} supervise the network training process by calculating the differences between Procrustes-aligned 3D poses from different views. Wandt~\etal~\cite{wandt2021canonpose} predict the camera poses and 3D body poses in a canonical form, and then supervise the training with the multi-view consistency. Kocabas~\etal~\cite{kocabas2019self} obtain the pseudo labels with epipolar geometry between different views and use the pseudo labels to train the 3D pose lifting network.
Different from previous works~\cite{iqbal2020weakly,rhodin2018learning,wandt2021canonpose,kocabas2019self}, our method uses spatio-temporal optimization framework that takes egocentric and external view as input to obtain robust 3D pseudo labels for training the network. This optimization method ensures the stability of the network training process when the 2D pose estimations are inaccurate.
% \ME{Earlier on it was not clear what is '' multi-view based optimization from the external camera '' L267-270 . It is only one camera, where is the multiview coming from ? 
% Then later on it is clear it is not multiview but '' temporal optimization ''. Maybe you can modify the termonolgy ? } 
% \JW{Yes, it is not "multiview", we can say it is takes the egocentric and external view as input.}


==> Estimating Egocentric 3D Human Pose in the Wild-CVPR2022/sections_old/experiments.tex <==
\section{Experiments}

\subsection{Datasets}

% Our network is trained on the synthetic dataset from Mo$^2$Cap$^2$ \cite{DBLP:journals/tvcg/XuCZRFST19} and the training split of EgoPW dataset. The Mo$^2$Cap$^2$ training dataset contains 530k images under 700 body textures.
We quantitatively evaluate our finetuned network on the real-world dataset from Mo$^2$Cap$^2$ \cite{DBLP:journals/tvcg/XuCZRFST19} and Wang \etal~\cite{wang2021estimating}. The real-world dataset in Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} contains 2.7k frames of two people captured in indoor and outdoor scenes, and that in Wang \etal~\cite{wang2021estimating} contains 12k frames of two people captured in the studio. To measure the accuracy of our pseudo labels, we evaluate our optimization method (Sec~\ref{subsec:optimizer}) only on the dataset from Wang \etal~\cite{wang2021estimating} since the Mo$^2$Cap$^2$ dataset does not include the external view.

% These datasets have the ground truth 3D poses from a multi-view motion capture system while they are mostly captured in the studio. \LJ{suggest removing the above sentence} 
To evaluate our method on the in-the-wild data, we also conduct a qualitative evaluation on the test set of EgoPW dataset. The EgoPW dataset will be made publicly available, and more details and comparisons to other datasets are included in the supplementary materials.

\subsection{Evaluation Metrics}
We measure the results of our method as well as other baseline methods with two metrics, PA-MPJPE and BA-MPJPE, which estimate the accuracy of a single body pose. For \textbf{PA-MPJPE}, we rigidly align the estimated pose $\mathcal{\hat{P}}$ of each frame to the ground truth pose $\mathcal{P}$ using Procrustes analysis \cite{kendall1989survey}. In order to eliminate the influence of body scale, we also report the \textbf{BA-MPJPE} scores. We first resize the bone length of each predicted body pose $\mathcal{\hat{P}}$ and ground truth body pose $\mathcal{P}$ to the bone length of a standard skeleton. Then, we calculate the PA-MPJPE between the two resulting poses. 

\begin{figure*}
\centering
\includegraphics[width=0.975\linewidth]{figures/results/results_wide_crop.pdf}
\caption{Qualitative comparison between our method and the state-of-the-art methods. From left to right: input image, Mo$^2$Cap$^2$ result, $x$R-egopose result, our result and external image. The ground truth pose is shown in red. Note that the external images is only for visualization and they are not used for predicting the pose.}
\label{fig:results}
\end{figure*}

\subsection{Accuracy of Pseudo Labels}\label{subsec:pseudo_labels}

\begin{table}[h]
\begin{center}
\small
\begin{tabular}{p{0.19\textwidth}
>{\centering}p{0.1\textwidth}
>{\centering\arraybackslash}p{0.1\textwidth}}
\hlineB{2.5}
Method & PA-MPJPE & BA-MPJPE \\ \hline
Mo$^2$Cap$^2$ & 102.3 & 74.46 \\
$x$R-egopose & 112.0 & 87.20 \\
Wang \etal~\cite{wang2021estimating} & 83.40 & 63.88 \\
VIBE~\cite{DBLP:conf/cvpr/KocabasAB20} & 68.13 & 52.99 \\
\hline
Our Optimizer & \textbf{57.19} & \textbf{46.14}\\
\hlineB{2.5}
\end{tabular}
\end{center}
\caption{The performance of our optimization framework on  Wang \etal's dataset. Our optimization method outperforms all previous egocentric pose estimation methods and the state-of-the-art pose estimation method of the external view.}
\label{table:pseudo_labels}
% \vspace{-1em}
\end{table}

In this paper, we first generate the pseudo labels with the optimization framework (Sec.~\ref{subsec:optimizer}) and use them to train the network. Thus, the accuracy of pseudo labels are critical. In this experiment, we evaluate the accuracy of pseudo labels on the Wang~\etal's dataset and show the results in Table~\ref{table:pseudo_labels}. 
This table shows that our method outperforms all the baseline methods by leveraging both the egocentric view and external view during optimization. Note that though compared in Table~\ref{table:pseudo_labels}, we cannot use any external-view based pose estimation method, \eg VIBE~\cite{DBLP:conf/cvpr/KocabasAB20} and 3DPW~\cite{von2018recovering}, for training the egocentric pose estimation network. This is because the relative pose between the external and egocentric camera is unknown, making it impossible to obtain the egocentric body pose only from the external view. Comparing with our optimization approach, the method in~\cite{wang2021estimating} performs worse due to the lack of external-view supervision. It is still possible to use this method to generate pseudo labels for training the network yet resulting in worse performance, which is demonstrated in the ablation study (Sec.~\ref{subsec:ablation}).



\subsection{Comparisons on 3D Pose Estimation}

\begin{table}[h]
\begin{center}
\small
\begin{tabularx}{0.47\textwidth} { 
   >{\raggedright\arraybackslash}X 
   >{\centering\arraybackslash}X 
   >{\centering\arraybackslash}X  }
\hlineB{2.5}
Method & PA-MPJPE & BA-MPJPE \\
\hline
\multicolumn{2}{l}{\textbf{Wang \etal's test dataset}} \\
\hline
Wang \etal~\cite{wang2021estimating} & 83.40 & 63.88 \\
\hline
Rhodin \etal~\cite{rhodin2018learning} & 89.67 & 73.56 \\
Mo$^2$Cap$^2$ & 102.3 & 74.46 \\
$x$R-egopose & 112.0 & 87.20 \\
Ours &\textbf{82.61} & \textbf{65.18} \\
\hlineB{2.5}
\multicolumn{2}{l}{\textbf{Mo$^2$Cap$^2$ test dataset}} \\
\hline
Rhodin \etal~\cite{rhodin2018learning} & 97.69 & 76.92 \\
Mo$^2$Cap$^2$ & 91.16 & 70.75 \\
$x$R-egopose & 86.85 & 66.54 \\
Ours &  \textbf{81.68} & \textbf{63.01} \\
\hlineB{2.5}
\end{tabularx}
\end{center}
\caption{The experimental results on Wang~\etal's test dataset and Mo$^2$Cap$^2$ test dataset \cite{DBLP:journals/tvcg/XuCZRFST19}. Our method outperforms the state-of-the-art methods, i.e. Mo$^2$Cap$^2$ \cite{DBLP:journals/tvcg/XuCZRFST19} and $x$R-egopose \cite{DBLP:conf/iccv/TomePAB19} on both of the metrics. Our method also outperforms a video-based method~\cite{wang2021estimating} in terms of  PA-MPJPE.
% \vspace{-0.5em}
}
\label{table:main}
\end{table}


We compare our approach with previous state-of-the-art single-frame-based methods on the test dataset from~\cite{wang2021estimating} under the ``Wang \etal's test dataset'' in Table~\ref{table:main}. Since the code or the predictions of $x$R-egopose are not publicly available, we use our reimplementation of $x$R-egopose instead. On this dataset, our method outperforms Mo$^2$Cap$^2$ by 20.1\% and $x$R-egopose by 27.03\% respectively.
Our single-image based method performs even better than Wang~\etal~\cite{wang2021estimating} in terms of PA-MPJPE. 
% Note that Wang~\etal uses a temporal-based egocentric pose optimization method which requires a sequence as input and cannot ensure real-time performance, while our work predicts egocentric pose from a single image and runs in real time. 
Note that Wang~\etal uses a video-based optimization method, which requires a sequence as input (for computing SLAM and temporal optimization) and cannot achieve real-time performance. In contrast, we estimate 3D poses from a single egocentric image at inference which is a more difficult problem. As a result, our method can run in real time.
% \KS{What are the advantage of our method over Wang et al? Since the difference is not so much, we need to explicitly re-iterate our advantages over the previous method here.}

We also compared with previous methods on the Mo$^2$Cap$^2$ test dataset in Table~\ref{table:main}. Since the camera parameters used in Mo$^2$Cap$^2$ are different from those used in this work, we train our network on the unlabeled dataset from the Mo$^2$Cap$^2$ work. Since the external view is not available for the Mo$^2$Cap$^2$ test dataset, we generate the pseudo labels with the optimize equation~\ref{eq:optim} without $E_{R}^{ext}$, $E_{J}^{ext}$, $E_{C}$, and $E_{M}$. Next, we follow Sec.~\ref{subsec:train} to train the pose estimation network on the Mo$^2$Cap$^2$ test dataset and show the results under the ``Mo$^2$Cap$^2$ test dataset'' in Table~\ref{table:main}. Our method performs better than Mo$^2$Cap$^2$ and $x$R-egopose by 10.4\% and 6.0\% respectively on Mo$^2$Cap$^2$ test dataset.

From the results in Table~\ref{table:main}, we can see that our approach significantly outperforms all previous methods on the single-frame egocentric pose estimation task. More quantitative results on each type of motion have included in the supplementary materials. For the qualitative comparison, we show the results of our method on the studio dataset and in-the-wild dataset in Fig.~\ref{fig:results}. Our method performs much better comparing to Mo$^2$Cap$^2$ and $x$R-egopose, especially for the in-the-wild cases where the body parts are occluded. Please refer to the supplementary materials for more qualitative results.




\subsection{Ablation Study}\label{subsec:ablation}

\begin{table}[h]
\begin{center}
\small
\begin{tabular}{p{0.2\textwidth}
>{\centering}p{0.1\textwidth}
>{\centering\arraybackslash}p{0.1\textwidth}}
\hlineB{2.5}
Method & PA-MPJPE & BA-MPJPE \\ \hline
Mo$^2$Cap$^2$ & 102.3 & 74.46 \\
$x$R-egopose & 112.0 & 87.20 \\
\hline
w/o external view  & 86.72 & 67.11 \\
w/o domain discriminator  & 86.24 & 65.74 \\
w/o bootstrapping  & 91.01 & 67.93 \\
Unsupervised DA  & 91.56 & 69.17 \\
Only bootstrapping & 88.47 & 68.49 \\
\hline
Ours & \textbf{81.73} & \textbf{64.05}\\
\hlineB{2.5}
\end{tabular}
\end{center}
\caption{The quantitative results of ablation study.}
\label{table:ablation}
% \vspace{-1em}
\end{table}

% In this section, we conduct experiments to further evaluate the effects of individual components in our approach. 
\paragraph{Supervision from the external view.}
In our work, we introduce the external view as a supervision for training the network on the real EgoPW dataset. The external view enables the generating accurate pseudo labels, especially when the human body parts are occluded in the egocentric view but can be observed in the external view. Without the external view, the obtained pseudo labels is less accurate and will further affects the network performance. In order to demonstrate this, we first generate the pseudo labels without any external supervision, \ie run our optimizer without $E_{R}^{ext}$, $E_{J}^{ext}$, $E_{C}$, and $E_{M}$, and then train the pose estimation network on this new pseudo labels. The result is shown in the ``w/o external view'' row of Table~\ref{table:ablation}.
We also show the qualitative results in Figure~\ref{fig:wo_external} where we evaluate our method with and without external view supervision.
% We also show the qualitative results in Figure~\ref{fig:wo_external} which compares our method with the result without any external view supervision \LJ{where we evaluate our method with and without external view supervision}.
Both the qualitative and quantitative results demonstrate that by introducing the external supervision, the performance of our finetuned pose estimation network is significantly better especially on the occlusion cases.

\begin{figure}
\centering
\includegraphics[width=0.98\linewidth]{figures/wo_external/wo_external_crop.pdf}
\caption{The results of our method with (c) and without external view (b). The network cannot predict accurate poses for the occluded cases without the external view supervision. 
The external view is only for visualization and not used for predicting the pose.
}
\label{fig:wo_external}
\end{figure}

\paragraph{Adversarial domain adaptation strategy.}
In our work, we first train the pose estimation network on the synthetic images and in-the-wild images with the adversarial domain adaptation module (Sec.~\ref{subsubsec:da}). With a domain classifier, this module eliminates the domain gap and enables the full use of both the synthetic and real images.
In order to investigate the efficacy of this strategy, we removed the domain classifier in our training framework and train the network without $\mathcal{L}_{Dis}$. We evaluate this network on Wang~\etal's dataset and show the quantitative results in the row of ``w/o domain discriminator'' in Table~\ref{table:ablation}. After removing the domain classifier, our method suffers from performance drop, which demonstrates the necessity of this module.


\paragraph{Bootstrapping module.}
In order to alleviate the influence of inaccurate pseudo labels, we introduce the bootstrapping strategy (Sec.~\ref{subsubsec:bootstrapping}).
% by updating the pseudo labels and pose estimation network in a loop. 
To prove its importance, we removed this module from our pipeline and train the network only with the adversarial domain adaptation module. The experimental results are shown in the ``w/o bootstrapping'' of Table~\ref{table:ablation}. Without the bootstrapping module, the network performs worse since the network is trained on inaccurate pseudo labels.

\paragraph{}

\paragraph{Comparison with only using unsupervised domain adaptation.}
In this experiment, we compare our approach with the unsupervised adversarial domain adaptation method~\cite{tzeng2017adversarial} which is commonly used for transfer learning tasks. We first train the network only with the $\mathcal{L_S}$ and $\mathcal{L}_{Dis}$ in the adversarial domain adaptation module (Sec.~\ref{subsubsec:da}) and show the results in the ``Unsupervised DA'' of the Table~\ref{table:ablation}. Our approach significantly outperforms the unsupervised domain adaptation method due to our high-quality pseudo labels. 
Even though we train the network on pseudo labels without bootstrapping, the results are still better than the unsupervised domain adaptation results, which is demonstrated by the comparison between ``Unsupervised DA'' and ``w/o bootstrapping'' in Table~\ref{table:ablation}. This is because the pseudo labels encode information of the external view, which is more effective than the unsupervised domain adaptation method without any external supervision.

\paragraph{Comparison with only using bootstrapping.}
In this experiment, we compare the our method with the network only trained with the bootstrapping strategy. We directly update the network with bootstrapping (Sec.~\ref{subsubsec:bootstrapping}) without first training the network both on real and synthetic dataset in Sec.~\ref{subsubsec:da}, \ie we only use modules in the yellow dashed box in Figure~\ref{fig:framework}. The result is shown as ``only bootstrapping'' in Table~\ref{table:ablation}. We can see that training on both the synthetic and EgoPW dataset is crucial to our method, since the synthetic dataset covers a large number of egocentric training data with accurate ground truth, while our EgoPW dataset contains the images in the real-world domain. 
% It is very necessary to leverage a domain adaptation method to bridge the domain 

==> Estimating Egocentric 3D Human Pose in the Wild-CVPR2022/sections_old/intro_new_lingjie.tex <==
\section{Introduction}

Egocentric motion capture using head- or body-mounted cameras has become popular recently because traditional motion capture systems with outside-in cameras have strong limitations when the person is moving around in a large space and thus restrict the scope of applications. Different from traditional  systems, the egocentric motion capture system is mobile, flexible, and has no requirements on recording space, which enables capturing a wide range of human activities for many applications, such as wearable medical monitoring, sports analysis, and $x$R.  

\begin{figure}
\begin{center}
\includegraphics[width=0.97\linewidth]{figures/teaser/teaser_with_external_red_crop.pdf}
\end{center}
   \caption{Comparing with Mo$^2$Cap$^2$, our method gets a more accurate egocentric pose from a single in-the-wild image, especially when the body parts are occluded. Note that the external images are only used for visualization and the 3D poses in this figure are only generated from the egocentric images.}
\label{fig:teaser}
\end{figure}

In this work, we focus on estimating the full 3D body pose with a single head-mounted fisheye camera. The most related works to ours are Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} and $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19}. 
Despite these methods have produced compelling results, existing methods are only trained on the synthetic data as limited real data exist and therefore suffer from significant performance drop on real data due to the domain gap between synthetic and real images. 
Furthermore, these methods often struggle with the cases when the human body is occluded by or interacting with the surrounding scene (See the Mo$^2$Cap$^2$ results in Fig.~\ref{fig:teaser}), mainly because the training supervision is only from a single egocentric view. 

To address these issues, we propose a new method to estimate 3D body pose with a single egocentric camera, which is trained on a new in-the-wild dataset. Specifically, we firstly capture a large-scale in-the-wild egocentric dataset called \emph{Egocentric Poses in the Wild (EgoPW)} with a new device setup consisting of an egocentric camera and an auxiliary external camera. Note that this dataset is the largest egocentric in-the-wild dataset, containing more than 312k frames and covering 20 different daily activities in 8 everyday scenes. 

We also note that the new device setup used for data capture has several advantages over existing setups. Compared to a multi-view setup with dense cameras used in [citations?], this new device setup is lightweight, flexible and allows recording in an environment with limited space; compared to a single egocentric camera setup, the additional external view would provide the information of the occluded regions in the egocentric view, e.g. the lower body part. 

% To address these issues, we propose a new method to estimate 3D body pose with a single egocentric camera, which is trained on a new in-the-wild dataset. Specifically, we capture a large-scale in-the-wild egocentric dataset called \emph{Egocentric Poses in the Wild (EgoPW)} with a new device setup consisting of an egocentric camera and an auxiliary external camera; we then design a method for training on the new dataset in a weakly supervised manner based on the 2D supervision from the egocentric view and external view. Note that this dataset is the largest egocentric in-the-wild dataset, containing more than 312k frames and covering 20 different daily activities in 8 everyday scenes. We also note that the new device setup used for data capture has several advantages over existing setups.  Compared to a multi-view setup with dense cameras used in [citations?], this new device setup is lightweight, flexible and allows recording in an environment with limited space; compared to a single egocentric camera setup, the additional external view would provide the information of the occluded regions in the egocentric view, e.g. the lower body part. 

Next, we design a method for training on the new dataset in a weakly supervised manner based on the information from the egocentric view and external view. Firstly, we extend the spatio-temporal optimization method proposed by Wang~\etal~\cite{wang2021estimating} to the multi-view scenario and generate accurate 3D poses for each frame in EgoPW dataset. The generated poses are further used as pseudo labels for training the pose estimation network on the EgoPW dataset. Moreover, we introduce an adversarial training strategy to align the semantic representation of egocentric and external images, since both the views share the same identity and body pose. To further improve the accuracy of the estimated poses, the synthetic dataset is also used to train our network and a domain adaptation strategy is adopted to minimizes the domain gap between synthetic and real data. The network trained with our method gives accurate 3D pose even under serious occlusions (See our results in Figure~\ref{fig:teaser}).

% In order to leverage the supervision from both the external view and egocentric view, we generate pseudo labels by developing a new spatio-temporal optimization method that leverages the 2D and 3D keypoints detected from the two views. The pseudo labels are then used to train the pose estimation network. We note that the external view is only used for training, but not for testing. 
% \JW{To further improve the accuracy of the estimated poses, we introduce a new adversarial training strategy by aligning the semantic representation of egocentric and external images.
% We also use synthetic dataset to train our network and adopt a domain adaptation strategy that minimizes the domain gap. The network trained with our method gives accurate 3D pose even under serious occlusions (See our results in Figure~\ref{fig:teaser}).}

% \JW{Since the corresponding egocentric and external images share the same identity and body pose, the intermediate features of them should also share the same semantic representation. Aside from optimizing the pseudo labels, we introduce a new adversarial learning strategy to align the feature representation and supervise the training of egocentric pose estimation network.}

% \JW{To further improve the accuracy of the estimated poses, we also adopt a domain adaptation strategy that minimizes the domain gap between synthetic and real dataset, and a bootstrapping strategy that optimize pseudo labels and the pose estimation network in a loop. The network trained with our method gives accurate 3D pose even under serious occlusions (See our results in Figure~\ref{fig:teaser}). }

We evaluate our method on the test data provided by Wang~\etal~\cite{wang2021estimating} and Xu~\etal~\cite{DBLP:journals/tvcg/XuCZRFST19}. Our method significantly outperforms the state-of-the-art methods both quantitatively and qualitatively. We also show qualitative results on various in-the-wild images, demonstrating that our method can predict accurate 3D poses in the in-the-wild scenes, especially when the body joints are seriously occluded. To summarize, our contributions are:

\begin{itemize}
\itemsep -0.1em
    \item A new approach for estimating accurate 3D human poses from a single in-the-wild egocentric image;
    \item A new in-the-wild egocentric pose estimation dataset (EgoPW) captured with a head-mounted fisheye camera and an external normal camera. We will make this dataset publicly available;
    \item A novel optimization method to generating the pseudo labels for the in-the-wild dataset by incorporating the supervision from the external view;
    \item  An adversarial learning method for aligning the semantic features between egocentric and external view.
\end{itemize}


==> Estimating Egocentric 3D Human Pose in the Wild-CVPR2022/sections_old/introduction.tex <==
\section{Introduction}



Egocentric motion capture using head- or body-mounted cameras has become popular recently because traditional motion capture systems with outside-in cameras have strong limitations when the person is moving around in a large space and thus restrict the scope of applications. Different from traditional methods, the egocentric motion capture system is mobile, flexible, and has no requirements on recording space, which enables capturing a wide range of human activities for many applications, such as wearable medical monitoring, sports analysis, and $x$R.  

\begin{figure}
\begin{center}
\includegraphics[width=0.97\linewidth]{figures/teaser/teaser_with_external_red_crop.pdf}
\end{center}
   \caption{Comparing with Mo$^2$Cap$^2$, our method gets a more accurate egocentric pose from a single in-the-wild image, especially when the body parts are occluded. Note that the external images are only used for visualization and the 3D poses in this figure are only generated from the egocentric images.}
\label{fig:teaser}
\end{figure}

In this work, we focus on estimating the full 3D body pose with a single head-mounted fisheye camera. The most related works to ours are Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} and $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19}. 
Despite these methods have produced compelling results, existing methods are only trained on the synthetic data and therefore suffer from significant performance drop on real data due to the domain gap between synthetic and real images. 
Furthermore, due to the difficulty in creating challenging synthetic scenarios of occlusions and human-object interactions, these methods often struggle with the cases when the human body is occluded by or interacting with the surrounding scene (See the Mo$^2$Cap$^2$ results in Fig.~\ref{fig:teaser}).

\JW{To improve the pose estimation on real-world data and handle the issue caused by occlusions, we collected a new in-the-wild egocentric dataset called \emph{Egocentric Poses in the Wild (EgoPW)} for training the pose estimation network. 
This dataset is the first egocentric in-the-wild dataset, which contains more than 312k frames and covers 20 different daily activities in 8 everyday scenes.}

\JW{However, setting up multi-view system for capturing the ground truth is challenging for the in-the-wild dataset. To this end, we set up a single synchronized external normal camera and collect images from the external view when collecting the EgoPW dataset. The additional external view would provide the information of the occluded regions in the egocentric view, e.g. the lower body part.}

\JW{In order to leverage the supervision from the external view, we generate accurate pseudo labels by developing a new spatio-temporal optimization method that leverages the 2D and 3D keypoints from both the egocentric view and the external view. Afterwards, the pseudo labels are used for training the pose estimation network. We note that the external view is only used for training, but not for testing. 
Comparing with available single-view pose estimation methods with multi-view weak supervision~\cite{iqbal2020weakly,rhodin2018learning,wandt2021canonpose,kocabas2019self}, our spatio-temporal optimization method generates the pseudo labels under the guidance of learned motion prior. This makes it robust to noisy and inaccurate 2D pose estimations, which is common for the 2D pose estimation results from the egocentric view.}

\JW{Since the corresponding egocentric and external images share the same identity and body pose, the intermediate features of them should also share the same semantic representation. Aside from optimizing the pseudo labels, we introduce a new adversarial learning strategy to align the feature representation and supervise the training of egocentric pose estimation network.}

\JW{To further improve the accuracy of the estimated poses, we also adopt a domain adaptation strategy that minimizes the domain gap between synthetic and real dataset, and a bootstrapping strategy that optimize pseudo labels and the pose estimation network in a loop. The network trained with our method gives accurate 3D pose even under serious occlusions (See our results in Figure~\ref{fig:teaser}). }

% To improve the pose estimation on real-world data and handle the issue caused by occlusions, we collected a new in-the-wild egocentric dataset with a head-mounted fisheye camera and an external normal camera, called \emph{Egocentric Poses in the Wild (EgoPW)}, for training the pose estimation network. 
% This dataset is the first egocentric in-the-wild dataset, which contains more than 312k frames and covers 20 different daily activities in 8 everyday scenes.

% However, setting up multi-view system for capturing the ground truth is challenging for the in-the-wild dataset. In order to provie 
% Considering the challenges in obtaining ground truth in the real world, we resort to the 

% In order to generate accurate 3D poses as pseudo labels for the EgoPW dataset, we develop a new optimization method that leverages the 2D and 3D keypoints from both the egocentric view and the external view. 
% The additional external view would provide the information of the occluded regions in the egocentric view, e.g. the lower body part, and thus improves the quality of pseudo labels. 
% We note that the external view is only used for training, but not for testing. 
% Comparing with other motion capture approaches such as multi-view motion capture systems~\cite{elhayek2015efficient, pavlakos2017harvesting,liu2013markerless} and IMU-based motion capture systems~\cite{huang2018deep,von2017sparse,von2018recovering}, our approach is simple, flexible, and does not need fixed capture space or any special device.

% Considering that synthetic data has its advantages compared to real data, e.g. it is easily accessible and has large variations on poses and backgrounds, we use both synthetic data and real data for training. Due to the domain gap between the synthetic data and real data, using the mixed data for efficient training is a challenge. To address this issue, we introduce a new adversarial domain adaptation method. Specifically, we extract the features from the synthetic data and real data and use an adversarial discriminator to distinguish if the feature is from synthetic data or real data. Once trained, the feature extractor would learn to produce the features in the same feature space for synthetic data and real data to fool the discriminator. 
% In this way, our method is able to make full use of the synthetic data and real data, thus achieving better results. 
% To further improve the accuracy of the estimated poses, we propose a bootstrapping strategy, \ie the pseudo labels are optimized based on the updated egocentric network prediction, while the egocentric network is finetuned with the updated pseudo labels. The finetuned network gives accurate 3D pose even under serious occlusions (See our results in Figure~\ref{fig:teaser}). 

We evaluate our method on the test data provided by Wang~\etal~\cite{wang2021estimating} and Xu~\etal~\cite{DBLP:journals/tvcg/XuCZRFST19}. Our method significantly outperforms the state-of-the-art methods both quantitatively and qualitatively. We also show qualitative results on various in-the-wild images, demonstrating that our method can predict accurate 3D poses in the in-the-wild scenes, especially when the body joints are seriously occluded. To summarize, our contributions are:

\JW{\begin{itemize}
\itemsep -0.1em
    \item A new approach for estimating accurate 3D human poses from a single in-the-wild egocentric image;
    \item A new in-the-wild egocentric pose estimation dataset (EgoPW) captured with a head-mounted fisheye camera and an external normal camera. We will make this dataset publicly available;
    \item A novel optimization method to generating the pseudo labels for the in-the-wild dataset by incorporating the supervision from the external view;
    \item  An adversarial learning method for aligning the semantic features between egocentric and external view.
\end{itemize}}


==> Estimating Egocentric 3D Human Pose in the Wild-CVPR2022/sections_old/method.tex <==
\section{Method}

We propose a new approach to train an egocentric pose estimation network. This network is able to estimate an accurate 3D body pose from a single egocentric in-the-wild image. The overview of our approach is illustrated in Fig.~\ref{fig:framework}. We first capture a large egocentric in-the-wild dataset, called \emph{EgoPW}, which contains synchronized egocentric image sequences and external image sequences (Sec.~\ref{subsec:dataset}). Next, we generate the pseudo labels for the EgoPW dataset with an optimization-based framework. This framework takes a sequence in a time window with $B$ frames of egocentric images $\mathcal{I}^{ego}_{seq}=\{\mathcal{I}^{ego}_{1},\dots,\mathcal{I}^{ego}_{B}\}$ and external images $\mathcal{I}^{ext}_{seq}=\{\mathcal{I}^{ext}_{1},\dots,\mathcal{I}^{ext}_{B}\}$ as input and outputs egocentric 3D poses $\mathcal{P}^{ego}_{seq}=\{\mathcal{P}^{ego}_{1},\dots,\mathcal{P}^{ego}_{B}\}$ as the pseudo labels (Sec.~\ref{subsec:optimizer}). Then, we propose an adversarial domain adaptation strategy to train the egocentric pose estimation network on both the synthetic dataset and EgoPW dataset with the generated pseudo labels $\mathcal{P}^{ego}_{seq}$ (Sec.~\ref{subsubsec:da}). In order to alleviate the influence of inaccurate pseudo labels, we finally finetune the network on the EgoPW dataset and the pseudo labels with a bootstrapping strategy (Sec.~\ref{subsubsec:bootstrapping}).

\subsection{EgoPW Dataset}\label{subsec:dataset}

% We first present the EgoPW dataset which is the first large in-the-wild egocentric dataset. \LJ{-> We first describe the \emph{EgoPW} dataset we collected, which is the first large in-the-wild human performance dataset in egocentric and external visions}. 
We first describe the \emph{EgoPW} dataset we collected, which is the first large-scale in-the-wild human performance dataset captured by an egocentric camera and an external normal camera (Sony RX0) which are synchronized.
This dataset contains 97 sequences (318k frames in total) of 10 actors in 20 clothing styles performing 20 different actions
, including reading magazine/newspaper, playing board games, doing a presentation, walking, sitting down, using a computer, calling on the phone, drinking water, writing on the paper, writing on the whiteboard, making tea, cutting vegetables, stretching, running, playing table tennis, playing baseball, climbing floors, dancing, opening the door and waving hands. 
% These sequences are collected by an egocentric camera and an external normal camera (Sony RX0) which are synchronized. 
% When collecting the egocentric sequences, we place a normal camera (Sony RX0) looking at the whole human body and record the external images at the same time. This synchronized external view enables the generation of pseudo labels.
We generate 3D poses as pseudo labels using the egocentric and external images, which will be elaborated later. 
In terms of the dataset size, our EgoPW dataset is larger than existing in-the-wild 3D pose estimation datasets like 3DPW~\cite{von2018recovering} and has a similar scale as the existing synthetic egocentric datasets for training including the  Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} dataset and the  $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19} dataset. 

\subsection{Optimization for Generating Pseudo Labels}\label{subsec:optimizer}

In this section, we present an optimization method based on \cite{wang2021estimating} to generate pseudo labels for the EgoPW dataset. We split the whole sequence into segments containing $B$ consecutive frames. 
For the egocentric frames $I^{ego}_{seq}$, we estimate the 3D poses represented by 15 joint locations in the coordinate system of egocentric camera (called ``egocentric poses")  $\widetilde{\mathcal{P}}^{ego}_{seq}=\{\widetilde{\mathcal{P}}^{ego}_1,\dots,\widetilde{\mathcal{P}}^{ego}_B \}$, $\widetilde{\mathcal{P}}^{ego}_i \in \mathbb{R}^{15 \times 3}$, and 2D heatmaps $\mathcal{H}^{ego}_{seq}=\{\mathcal{H}^{ego}_1,\dots,\mathcal{H}^{ego}_B \}$ using the Mo$^2$Cap$^2$ method \cite{DBLP:journals/tvcg/XuCZRFST19}.
Aside from egocentric poses, we also estimate the transformation matrix between the egocentric camera poses of two adjacent frames $[R_{seq}^{SLAM} \mid t_{seq}^{SLAM}] = \{[R_1^2 \mid t_1^2], \dots, [R_{B-1}^{B} \mid t_{B-1}^B]\}$ using ORB-SLAM2~\cite{murTRO2015}.
For the external frames $I^{ext}_{seq}$, we estimate the 3D pose (called ``external poses") $\mathcal{P}^{ext}_{seq}=\{\mathcal{P}^{ext}_1,\dots,\mathcal{P}^{ext}_B \}$, $\mathcal{P}^{ext}_i \in \mathbb{R}^{15 \times 3}$ using VIBE~\cite{DBLP:conf/cvpr/KocabasAB20} and 2D joints $\mathcal{J}^{ext}_{seq}=\{\mathcal{J}^{ext}_1,\dots,\mathcal{J}^{ext}_B \}$, $\mathcal{J}^{ext}_i \in \mathbb{R}^{15 \times 2}$ using openpose~\cite{cao2017realtime}. 

% Next, we design an optimization framework which first captures the motion prior with a sequential VAE \cite{wang2021estimating} and then optimize the egocentric pose sequence $\mathcal{P}_{ego}^{seq}$ with the learned motion prior by minimizing the egocentric and external reprojection term.

Next, following \cite{wang2021estimating}, we learn a latent space to encode an egocentric motion prior with a sequential VAE which consists of a CNN-based encoder $f_{enc}$ and decoder $f_{dec}$. We then optimize the egocentric pose by finding a latent vector $z$ such that the corresponding pose sequence $P^{ego}_{seq} = f_{dec}(z)$ minimizes the objective function:

\begin{equation}
\begin{aligned}
	E (\mathcal{P}_{seq}^{ego}, R_{seq}, t_{seq}) &= \lambda_R^{ego} E_{R}^{ego} + \lambda_R^{ext} E_{R}^{ext} + \lambda_J^{ego} E_{J}^{ego} \\
	& +  \lambda_J^{ext} E_{J}^{ext} + \lambda_T E_{T} + \lambda_B E_{B}\\
	& + \lambda_C E_{C} + \lambda_M E_{M}
	\label{eq:optim}
\end{aligned}
\end{equation}
Note that since the relative pose between external camera and egocentric camera is unknown, we also need to optimize the relative egocentric camera pose with respect to the external camera pose for each frame, i.e. the rotations  $R_{seq} = {R_1,\dots,R_B}$ and translations $t_{seq} = {t_1,\dots,t_B}$.

In this objective function, $E_{R}^{ego}$, $E_{J}^{ego}$,$E_{T}$, and $E_{B}$ are egocentric reprojection term, egocentric pose regularization term, motion smoothness regularization term and bone length regularization term, which are the same as those defined in~\cite{wang2021estimating}. We will also include the detailed definitions in the supplemental materials. 
$E_{R}^{ext}$, $E_{J}^{ext}$, $E_{C}$, and $E_{M}$ are the external reprojection term, external 3D body pose regularization term, camera pose consistency term, and camera matrix regularization term, which will be described later. 



% \begin{equation}
% \begin{aligned}
% 	E (\mathcal{P}_{seq}^{ego}, R, t) &= \lambda_R^{ego} E_{R}^{ego}(\mathcal{P}_{seq}^{ego}) + \lambda_R^{ext} E_{R}^{ext}(\mathcal{P}_{seq}^{ext}, R, t)\\
% 	& + \lambda_J^{ego} E_{J}^{ego}(\mathcal{P}_{seq}^{ego}, \widetilde{\mathcal{P}}_{seq}^{ego}) \\
% 	& + \lambda_J^{ext} E_{J}^{ext}(\mathcal{P}_{seq}^{ego}, \mathcal{P}_{seq}^{ext}) \\
% 	& + \lambda_T E_{T}(\mathcal{P}_{seq}^{ego}) + \lambda_B E_{B}(\mathcal{P}_{seq}^{ego}) \\
% 	& + \lambda_C E_{C}(R, t, R^{ego}, t^{ego}) \\
% 	& + \lambda_M E_{M}(R)
% 	\label{eq:optim}
% \end{aligned}
% \end{equation}

\paragraph{External Reprojection Term}

We use the external 2D detection as a supervision in the optimization framework. The energy term is defined as:
\begin{equation}
    E_{R}^{ext}(\mathcal{P}_{seq}^{ego}, R_{seq}, t_{seq}) = \sum_{i=1}^{B}\left\Vert \mathcal{J}_{i}^{ext} - K\left[R_i\mid t_i\right]\mathcal{P}_{i}^{ego} \right\Vert_2^2 \label{eq:ext_reproj}
\end{equation}
where the $K$ is the intrinsic matrix of the external camera; $\left[R_{i} \mid t_{i} \right]$ is the pose of the egocentric camera of the $i$ th frame in the external camera space. 
In this term, we first project the egocentric body pose $\mathcal{P}_{i}^{ego}$ to the 2D body pose in the external view with the egocentric camera pose $\left[R_{i} \mid t_{i} \right]$ and the intrinsic matrix $K$, and then compare the projected body pose with the 2D joints estimated by the openpose~\cite{cao2017realtime}. Since the relative pose between the external camera and egocentric camera are unknown at the beginning of the optimization, we optimize the egocentric camera pose $\left[R_{i} \mid t_{i} \right]$ along with the egocentric body pose $\mathcal{P}_{seq}^{ego}$. 
In order to make the optimization process converge faster, we initialize the egocentric camera pose $\left[R_{i} \mid t_{i} \right]$ with the Perspective-n-Point algorithm~\cite{Gao2003CompleteSC}.
% However, because of the depth ambiguity, the accurate 3D pose cannot be obtained only with the external reprojection term.

\paragraph{Camera Pose Consistency}

% We cannot get the accurate 3D pose only with the external reprojection term because the egocentric camera pose and the optimized body pose can be arbitrarily changed without violating the external reprojection constraint \LJ{-> because there is an ambiguity in egocentric camera poses. }. 
We cannot get the accurate 3D body pose only with the external reprojection term because the egocentric camera pose and the optimized body pose can be changed in a coordinated manner without violating the constraint, as long as their relative position remains unchanged.
To alleviate this ambiguity, aside from the motion smoothness term $E_T$, we introduce the camera consistency term $E_C$. Specifically, this term enforces the egocentric camera pose at $(i + 1)$ th frame $[R_{i + 1} \mid t_{i + 1}]$ to be consistent with the pose obtained by transforming the egocentric camera pose at the $i$ th frame $[R_{i} \mid t_{i}]$ with the relative pose between the $i$ th and $(i + 1)$ th frame.

% This can be alleviated by applying the motion smoothness term to make the body pose consistent over the time. Aside from this, we also introduce the camera pose consistency term which keeps the camera pose $[R_i \mid t_i]$ and $[R_{i + 1} \mid t_{i + 1}]$ consistent by bridging them with the SLAM method which estimates the relative egocentric camera pose $[R_i^{i+1} \mid t_i^{i+1}]$ between $i$ th and $i + 1$ th frame 

% keeps the egocentric camera pose $[R_i \mid t_i]$ and $[R_{i + 1} \mid t_{i + 1}]$ consistent by bridging them with the relative egocentric camera pose $[R_i^{i+1} \mid t_i^{i+1}]$ between $i$ th and $i + 1$ th frame:

% % \begin{equation}
% % \begin{aligned}
% %     E_{C}(R_{seq}, t_{seq}) & = \sum_{i=1}^{B-1} \left (\left\Vert R_i R_i^{SLAM} - R_{i + 1} \right\Vert_2 \right.\\
% %     & + \left. \left\Vert R_i t_i^{SLAM} + t_i - t_{i + 1}\right\Vert_2 \right) \label{eq:consistency}
% % \end{aligned}
% % \end{equation}

\begin{equation}
\begin{aligned}
    E_{C}(R_{seq}, t_{seq}) & = \sum_{i=1}^{B-1}\left\Vert \begin{bmatrix} R_i  & t_i \\ 0 & 1 \end{bmatrix} \begin{bmatrix} R^{i+1}_i  & t^{i+1}_i \\ 0 & 1 \end{bmatrix} \right.\\
    & - \left. \begin{bmatrix} R_{i+1}  & t_{i+1} \\ 0 & 1 \end{bmatrix}\right\Vert_2 \label{eq:consistency}
\end{aligned}
\end{equation}

\paragraph{External 3D Body Pose Regularization}

Besides the external reprojection term, we also use the external 3D body poses to supervise the optimization of the egocentric 3D body pose. 
We define the external 3D pose term which measures the difference between the external body poses and the egocentric body poses after the rigid alignment:
% transformed from the egocentric camera space to the external camera space. 
% We make the optimized egocentric pose $\mathcal{P}_{i}^{ego}$ stay close to the external 3D pose estimation $\mathcal{P}_{i}^{ext}$ by defining the term as the difference between the 3D joint locations of egocentric and external view after the rigid alignment:

\begin{equation}
	E_{J}(\mathcal{P}_{seq}^{ego}, \mathcal{P}_{seq}^{ext}) = \sum_{i=1}^{B}\left\Vert \mathcal{P}_{i}^{ext} - \left[R_{i}^{pa}\mid t_{i}^{pa}\right]\mathcal{P}_{i}^{ego} \right\Vert_2^2 \label{eq:ext_3d_pose}
\end{equation}
where $\left[R_{i}^{pa} \mid t_{i}^{pa} \right]$ is the transformation matrix calculated with Procrustes analysis which rigidly aligns the external 3D pose estimation $\mathcal{P}_{i}^{ext}$ and the egocentric 3D pose $\mathcal{P}_{i}^{ego}$.

% With the external reprojection term and external 3D pose regularization term, we are able to generate accurate pseudo labels even though the human body in the egocentric view is seriously occluded, as illustrated in Fig.~\ref{fig:optimization_example}. With the external view, we are able to train the network with the accurate pseudo labels for the in-the-wild images, especially in the occluded cases. 

% We note that only by combining the egocentric view and external view, we can reconstruct accurate pseudo labels since the body parts can be either occluded in the egocentric or external view. 
By combining the body poses estimated from the egocentric view and external view, we can reconstruct more accurate pseudo labels.  
As shown in Fig.~\ref{fig:optimization_example}, the hands of the person are occluded in the external view, resulting in the tracking of the hands fails in the external view (Fig.~\ref{fig:optimization_example}, b), however, the hands can be clearly seen and tracked in the egocentric view (Fig.~\ref{fig:optimization_example}, d); 
on the other hand, the feet cannot be observed in the egocentric view and thus failed to be tracked in this view (Fig.~\ref{fig:optimization_example}, b), but can be easily viewed and tracked in the external view (Fig.~\ref{fig:optimization_example}, d). 
%Thus, either the optimizer with only the egocentric view (second image) or the external pose estimation method like VIBE~\cite{DBLP:conf/cvpr/KocabasAB20} (fourth image) cannot predict accurate pseudo labels. 
By joining the information from both views, we can successfully predict accurate 3D poses as the pseudo labels (Fig.~\ref{fig:optimization_example}, c).  
% combining the egocentric and external view in our optimization framework, we can predict accurate 3D poses as the pseudo labels, which is illustrated in the third image.
We note that the external camera is only used for generating the pseudo labels but at test time, only the egocentric camera is used. 

\begin{figure}
\centering
\includegraphics[width=0.98\linewidth]{figures/optimization_example/optimization_example_crop.pdf}
\caption{Our pseudo label generation method combines the information from both the egocentric view and external view, therefore leading to accurate pseudo labels (c). Only with the egocentric camera, the feet cannot be observed and well-tracked (b); Only with the external camera, the hands are occluded and result in the wrong result on the hand part (d).
% We note that the external camera is only used in the pseudo label generation for training, which is not used at test time.
}
% or external view is restrictive for predicting accurate 3D poses (the second and fourth image), while our optimization method gives reasonable result (the third image).
\label{fig:optimization_example}
\end{figure}



\paragraph{Camera Matrix Regularization}

We constrain the camera rotation matrix $R_{i}$ to be an orthogonal matrix:

\begin{equation}
	E_{J}(R_{seq}) = \sum_{i=1}^{B}\left\Vert R_{i}^TR_{i} - I \right\Vert_2^2 \label{eq:matrix}
\end{equation}
where $det(.)$ is the determinant of the matrix.

Through the optimization framework, we can get accurate 3D pose pseudo labels $\mathcal{P}_{seq}^{ego}$, which is further processed into the 2D heatmap $\mathcal{H_T}$ and the distance between joints and egocentric camera $\mathcal{D_T}$ with the fisheye camera model \cite{scaramuzza2014omnidirectional} described in supplementary materials. 

% for each batch and combine the batches to get the 3D labels for the whole EgoPW dataset $\mathcal{P_T}$ \LJ{I don't think we need to mention this, suggest removing the above sentence}

% , where the projection of a 3D point $[x, y, z]^T$ can be written as:

% \begin{equation}
% 	[u, v]^T = \frac{[x, y]^T}{\sqrt{x^2 + y^2}} \times f(\rho)
% \end{equation}
% where $\rho = \arctan(z / \sqrt{x^2 + y^2})$ and $f(\rho) = \alpha_0 + \alpha_1 \rho + \alpha_2 \rho^2 + \alpha_3 \rho^3 +\dots$ is a polynomial obtained from camera calibration.


\subsection{Domain Adaptation}\label{subsec:train}

After obtaining the pseudo labels for the EgoPW dataset, we introduce a domain adaptation approach for training a pose estimation network, which can be used for estimating the 3D pose from a single egocentric image. Our core idea is to use an adversarial discriminator to tackle the problem of the domain gap between the synthetic data and the real in-the-wild data. Here, we define the source domain $\mathcal{S} = \{\mathcal{I_{S}}, \mathcal{H_{S}}, \mathcal{D_{S}}\}$ which is composed of synthetic images $\mathcal{I_{S}}$ along with their corresponding heatmap $\mathcal{H_{S}}$ and distance $\mathcal{D_{S}}$ labels from Mo$^2$Cap$^2$ dataset, and the target domain $\mathcal{T}= \{\mathcal{I_{T}}, \mathcal{H_{T}}, \mathcal{D_{T}}\}$ which consists of in-the-wild egocentric images $\mathcal{I_T}$ with pseudo heatmaps $\mathcal{H_{T}}$ and distance labels $\mathcal{D_{T}}$ from EgoPW dataset. We first minimize the domain gap between the source and target domain using an adversarial domain adaptation network and then apply a bootstrapping strategy to finetune the network on the EgoPW dataset with pseudo labels. 

% In this section, we introduce our domain adaptation approach for training the egocentric pose estimation network on the EgoPW dataset. The source domain $\mathcal{S}$ consists of synthetic images $\mathcal{I_{S}}$ and the corresponding heatmap $\mathcal{H_{S}}$ and distance $\mathcal{D_{S}}$ labels from Mo$^2$Cap$^2$ dataset, and the target domain $\mathcal{T}$ consists of in-the-wild egocentric images $\mathcal{I_T}$ with pseudo heatmaps $\mathcal{H_{T}}$ and distance $\mathcal{D_{T}}$ labels \LJ{distance labels?} from EgoPW dataset. We firstly minimize the domain gap between the source and target domain using an adversarial domain adaptation network, and further apply a bootstrapping strategy to finetune the network on the EgoPW dataset with pseudo labels. 

\subsubsection{Adversarial Domain Adaptation Module}\label{subsubsec:da}

Our adversarial domain adaptation module consists of a Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} network for estimating the egocentric pose and an adversarial discriminator $\Gamma$. The Mo$^2$Cap$^2$ network has a feature extractor $\Theta$ which encodes an image into a feature vector and a pose estimator $\Psi$ which decodes the feature vector to a heatmap and a 3D pose. 
The adversarial discriminator takes as input the feature vectors extracted from a synthetic image and an in-the-wild image, and determines if the feature is extracted from an in-the-wild image. 
Note that the synthetic image does not have a corresponding in-the-wild image, so we refer to this data as \emph{unpaired}. 
We train the adversarial domain adaptation module with two reconstruction loss terms and a discriminator loss term.

The reconstruction loss is defined as the mean squared error (MSE) between the predicted heatmaps/distances and heatmaps/distances from pseudo labels.

% The reconstruction loss is defined as the sum of the mean squared error (MSE) between the predicted heatmaps and the ground truth heatmaps and that between the predicted distances and the ground truth distances. 

\begin{equation}
    \begin{aligned}
        \mathcal{L}_{S} &= \text{mse}(\mathcal{\hat{H}_{S}}, \mathcal{H_{S}}) + \text{mse}(\mathcal{\hat{D}_{S}}, \mathcal{D_{S}})\\
        \mathcal{L}_{T} &= \text{mse}(\mathcal{\hat{H}_{T}}, \mathcal{H_{T}}) + \text{mse}(\mathcal{\hat{D}_{T}}, \mathcal{D_{T}})
    \end{aligned}
\end{equation}
where 
% Given a pair of images $(\mathcal{I_{S}}, \mathcal{I_{T}}) \in \mathbb{R}^{H \times W \times 3}$ from the Mo$^2$Cap$^2$ and EgoPW dataset,  the intermediate features $(\mathcal{F_{S}}, \mathcal{F_{T}})$ is obtained by the extractor $\Theta$, which is subsequently put into the decoder $\Psi$ for generating 2D heatmap $(\mathcal{\hat{H}_{S}}, \mathcal{\hat{H}_{T}})$ and the distance $(\mathcal{\hat{D}_{S}}, \mathcal{\hat{D}_{T}})$ predictions:
\begin{equation}
    \begin{aligned}
        \mathcal{F_{S}} = \Theta(\mathcal{I_{S}});& \mathcal{F_{T}} = \Theta(\mathcal{I_{T}})\\
        \mathcal{\hat{H}_{S}}, \mathcal{\hat{D}_{S}} = \Psi(\mathcal{F_{S}});& \mathcal{\hat{H}_{T}}, \mathcal{\hat{D}_{T}} = \Psi(\mathcal{F_{T}})
    \end{aligned}
\end{equation}
% and the 3D poses $\mathcal{\hat{P}_S}$ and $\mathcal{\hat{P}_T}$ can be obtained with the fisheye camera model \cite{scaramuzza2014omnidirectional} described in supplementary materials. 

% We define the loss in the source and target domain as the mean square error (MSE) between the predictions and the labels:

% \begin{equation}
%     \begin{aligned}
%         \mathcal{L}_{S} &= mse(\mathcal{\hat{H}_{S}}, \mathcal{H_{S}}) + mse(\mathcal{\hat{D}_{S}}, \mathcal{D_{S}})\\
%         \mathcal{L}_{T} &=  mse(\mathcal{\hat{H}_{T}}, \mathcal{H_{T}}) + mse(\mathcal{\hat{D}_{T}}, \mathcal{D_{T}})
%     \end{aligned}
% \end{equation}

To bridge the domain gap between the source and target domains, we use an adversarial discriminator $\Gamma$ to distinguish the feature vectors from source or target data with a cross-entropy loss:

\begin{equation}
    \mathcal{L}_{Dis} = -E[\log(\Gamma(\mathcal{F_S}))] - E[\log(1 - \Gamma(\mathcal{F_T}))]
\end{equation}

Once the discriminator $\Gamma$ has been trained, the feature extractor $\Theta$ maps the images from different domains to the same feature space such that the classifier $\Gamma$ cannot tell if the features are extracted from synthetic images or real images. Therefore, the pose estimator $\Psi$ can predict more accurate poses for the in-the-wild data. 

\subsubsection{Bootstrapping}\label{subsubsec:bootstrapping}

\begin{figure}
\centering
\includegraphics[width=1\linewidth]{figures/optimization_iterations/optimization_iterations_wide_crop.pdf}
\caption{Results in the bootstrapping process. Given an inaccurate pose (initial network prediction) to initialize the optimization process, the pseudo label obtained with our optimization framework is inaccurate (initial optimization). However, given a good egocentric prediction from our finetuned network (final network prediction) for initialization, the optimization can converge to an accurate pose (final optimization).
% \LJ{Given the initial pseudo labels as supervision for the pose estimation network, the estimated pose from the network is inaccurate (initial network prediction). ...}
}
\label{fig:optimization_iterations}
\end{figure}

% In the Sec.~\ref{subsubsec:da}, we use the EgoPW dataset with the pseudo labels generated by the optimizer from the Mo2Cap2 predictions. 
While significant performance improvement has been made by the  adversarial domain adaptation, the accuracy of pose predictions is still limited due to the errors in the generated pseudo labels. These errors mostly stem from the noisy egocentric 3D poses and 2D heatmaps predicted by the Mo$^2$Cap$^2$ network. 
% Though significant performance improvement can be achieved by incorporating the adversarial domain adaptation in Sec.~\ref{subsubsec:da}, the accuracy of network predictions is still limited due to the significant errors in pseudo labels obtained by our optimization framework. These errors mostly stem from the noisy egocentric 3D poses and 2D heatmaps predicted by the Mo$^2$Cap$^2$ network. 

To circumvent this issue, inspired by SPIN~\cite{DBLP:conf/iccv/KolotourosPBD19}, we develop a bootstrapping algorithm. We first apply our adversarial domain-adaptation network (Sec.~\ref{subsubsec:da}) to get the initial egocentric 3D poses and use them for initializing the optimization framework. Next, we use the optimization framework (Sec.~\ref{subsec:optimizer}) to generate the pseudo labels and use the labels to finetune the pose estimation network. We execute this process iteratively, such that the finetuned network provides better initialization for the optimization framework and the optimization framework generates better pseudo labels to finetune the network:

\begin{algorithm}
\SetAlgoLined
\KwIn{$\Theta$, $\Psi$, $\mathcal{I_T}$, $\mathcal{H_T}$, $\mathcal{D_T}$, optimizer, max\_iter}
\KwOut{Finetuned network parameters $\Theta$}
 iter $\coloneqq$ 0\;
 \While{iter $<$ max\_iter}{
  $\mathcal{H}, \mathcal{D} \coloneqq \Psi(\Theta(\mathcal{I_T}))$\;
  $\mathcal{H_T}, \mathcal{D_T} \coloneqq$ optimizer$(\mathcal{H}, \mathcal{D})$\;
  update network parameter of $\Theta$ and $\Psi$ with $\mathcal{L}_{T}$\;
  iter $\coloneqq$ iter + 1\;
 }
 \caption{Bootstrapping Algorithm}
\end{algorithm}

We show the results before and after bootstrapping in Fig.~\ref{fig:optimization_iterations}. We can see that the pseudo labels have been improved significantly with bootstrapping, and the improved pseudo labels provide a better supervision for the pose estimation network, leading to better pose estimation for the in-the-wild data. 

% We show the initial optimized result and final optimized result in Fig.~\ref{fig:optimization_iterations}, which demonstrate that the pseudo labels are improved significantly along the training process. The improved pseudo labels provides a better supervision, enabling the better performance of the pose estimation network on the in-the-wild data.

% 






==> Estimating Egocentric 3D Human Pose in the Wild-CVPR2022/sections_old/method_cvpr.tex <==
\section{Method}
We propose a new approach to train a network with the weak supervision from egocentric and external views. This network is able to estimate an accurate 3D body pose from a single egocentric in-the-wild image. The overview of our approach is illustrated in Fig.~\ref{fig:framework}. We first capture a large egocentric in-the-wild dataset, called \emph{EgoPW}, which contains synchronized egocentric image sequences and external image sequences (Sec.~\ref{subsec:dataset}). Next, we generate the pseudo labels for the EgoPW dataset with an optimization-based framework. This framework takes a sequence in a time window with $B$ frames of egocentric images $\mathcal{I}^{ego}_{seq}=\{\mathcal{I}^{ego}_{1},\dots,\mathcal{I}^{ego}_{B}\}$ and external images $\mathcal{I}^{ext}_{seq}=\{\mathcal{I}^{ext}_{1},\dots,\mathcal{I}^{ext}_{B}\}$ as input and outputs egocentric 3D poses $\mathcal{P}^{ego}_{seq}=\{\mathcal{P}^{ego}_{1},\dots,\mathcal{P}^{ego}_{B}\}$ as the pseudo labels (Sec.~\ref{subsec:optimizer}). 

Next, we train the egocentric pose estimation network on the synthetic data and on the EgoPW dataset with pseudo labels $\mathcal{P}^{ego}_{seq}$. In the training process, we leverage the intermediate feature representation from the external pose estimation network~\cite{xiao2018simple} to supervise the training of egocentric pose estimation network in an adversarial way (Sec.~\ref{subsubsec:ext_adv}). We also introduce the adversarial domain adaptation strategy to eliminate the domain gap between synthetic and real dataset (Sec.~\ref{subsubsec:da}).


\subsection{EgoPW Dataset}\label{subsec:dataset}

We first describe the \emph{EgoPW} dataset we collected, which is the first large-scale in-the-wild human performance dataset captured by an egocentric camera and an external normal camera (Sony RX0) which are synchronized.
This dataset contains 97 sequences (318k frames in total) of 10 actors in 20 clothing styles performing 20 different actions
, including reading magazine/newspaper, playing board games, doing a presentation, walking, sitting down, using a computer, calling on the phone, drinking water, writing on the paper, writing on the whiteboard, making tea, cutting vegetables, stretching, running, playing table tennis, playing baseball, climbing floors, dancing, opening the door and waving hands. 
We generate 3D poses as pseudo labels using the egocentric and external images, which will be elaborated later. 
In terms of the dataset size, our EgoPW dataset is larger than existing in-the-wild 3D pose estimation datasets like 3DPW~\cite{von2018recovering} and has a similar scale as the existing synthetic egocentric datasets for training including the  Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} dataset and the  $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19} dataset. 

\subsection{Optimization for Generating Pseudo Labels}\label{subsec:optimizer}

In this section, we present an optimization method based on \cite{wang2021estimating} to generate pseudo labels for the EgoPW dataset. We split the whole sequence into segments containing $B$ consecutive frames. 
For the egocentric frames $I^{ego}_{seq}$, we estimate the 3D poses represented by 15 joint locations in the coordinate system of egocentric camera (called ``egocentric poses")  $\widetilde{\mathcal{P}}^{ego}_{seq}=\{\widetilde{\mathcal{P}}^{ego}_1,\dots,\widetilde{\mathcal{P}}^{ego}_B \}$, $\widetilde{\mathcal{P}}^{ego}_i \in \mathbb{R}^{15 \times 3}$, and 2D heatmaps $\mathcal{H}^{ego}_{seq}=\{\mathcal{H}^{ego}_1,\dots,\mathcal{H}^{ego}_B \}$ using the Mo$^2$Cap$^2$ method \cite{DBLP:journals/tvcg/XuCZRFST19}.
Aside from egocentric poses, we also estimate the transformation matrix between the egocentric camera poses of two adjacent frames $[R_{seq}^{SLAM} \mid t_{seq}^{SLAM}] = \{[R_1^2 \mid t_1^2], \dots, [R_{B-1}^{B} \mid t_{B-1}^B]\}$ using ORB-SLAM2~\cite{murTRO2015}.
For the external frames $I^{ext}_{seq}$, we estimate the 3D pose (called ``external poses") $\mathcal{P}^{ext}_{seq}=\{\mathcal{P}^{ext}_1,\dots,\mathcal{P}^{ext}_B \}$, $\mathcal{P}^{ext}_i \in \mathbb{R}^{15 \times 3}$ using VIBE~\cite{DBLP:conf/cvpr/KocabasAB20} and 2D joints $\mathcal{J}^{ext}_{seq}=\{\mathcal{J}^{ext}_1,\dots,\mathcal{J}^{ext}_B \}$, $\mathcal{J}^{ext}_i \in \mathbb{R}^{15 \times 2}$ using openpose~\cite{cao2017realtime}. 

Next, following \cite{wang2021estimating}, we learn a latent space to encode an egocentric motion prior with a sequential VAE which consists of a CNN-based encoder $f_{enc}$ and decoder $f_{dec}$. We then optimize the egocentric pose by finding a latent vector $z$ such that the corresponding pose sequence $P^{ego}_{seq} = f_{dec}(z)$ minimizes the objective function:

\begin{equation}
\begin{aligned}
	E (\mathcal{P}_{seq}^{ego}, R_{seq}, t_{seq}) &= \lambda_R^{ego} E_{R}^{ego} + \lambda_R^{ext} E_{R}^{ext} + \lambda_J^{ego} E_{J}^{ego} \\
	& +  \lambda_J^{ext} E_{J}^{ext} + \lambda_T E_{T} + \lambda_B E_{B}\\
	& + \lambda_C E_{C} + \lambda_M E_{M}
	\label{eq:optim}
\end{aligned}
\end{equation}
Note that since the relative pose between external camera and egocentric camera is unknown, we also need to optimize the relative egocentric camera pose with respect to the external camera pose for each frame, i.e. the rotations  $R_{seq} = {R_1,\dots,R_B}$ and translations $t_{seq} = {t_1,\dots,t_B}$.

In this objective function, $E_{R}^{ego}$, $E_{J}^{ego}$,$E_{T}$, and $E_{B}$ are egocentric reprojection term, egocentric pose regularization term, motion smoothness regularization term and bone length regularization term, which are the same as those defined in~\cite{wang2021estimating}. We will also include the detailed definitions in the supplemental materials. 
$E_{R}^{ext}$, $E_{J}^{ext}$, $E_{C}$, and $E_{M}$ are the external reprojection term, external 3D body pose regularization term, camera pose consistency term, and camera matrix regularization term, which will be described later. 



\paragraph{External Reprojection Term}

We use the external 2D detection as a supervision in the optimization framework. The energy term is defined as:
\begin{equation}
    E_{R}^{ext}(\mathcal{P}_{seq}^{ego}, R_{seq}, t_{seq}) = \sum_{i=1}^{B}\left\Vert \mathcal{J}_{i}^{ext} - K\left[R_i\mid t_i\right]\mathcal{P}_{i}^{ego} \right\Vert_2^2 \label{eq:ext_reproj}
\end{equation}
where the $K$ is the intrinsic matrix of the external camera; $\left[R_{i} \mid t_{i} \right]$ is the pose of the egocentric camera of the $i$ th frame in the external camera space. 
In this term, we first project the egocentric body pose $\mathcal{P}_{i}^{ego}$ to the 2D body pose in the external view with the egocentric camera pose $\left[R_{i} \mid t_{i} \right]$ and the intrinsic matrix $K$, and then compare the projected body pose with the 2D joints estimated by the openpose~\cite{cao2017realtime}. Since the relative pose between the external camera and egocentric camera are unknown at the beginning of the optimization, we optimize the egocentric camera pose $\left[R_{i} \mid t_{i} \right]$ along with the egocentric body pose $\mathcal{P}_{seq}^{ego}$. 
In order to make the optimization process converge faster, we initialize the egocentric camera pose $\left[R_{i} \mid t_{i} \right]$ with the Perspective-n-Point algorithm~\cite{Gao2003CompleteSC}.


\paragraph{Camera Pose Consistency}

We cannot get the accurate 3D body pose only with the external reprojection term because the egocentric camera pose and the optimized body pose can be changed in a coordinated manner without violating the constraint, as long as their relative position remains unchanged.
To alleviate this ambiguity, aside from the motion smoothness term $E_T$, we introduce the camera consistency term $E_C$. Specifically, this term enforces the egocentric camera pose at $(i + 1)$ th frame $[R_{i + 1} \mid t_{i + 1}]$ to be consistent with the pose obtained by transforming the egocentric camera pose at the $i$ th frame $[R_{i} \mid t_{i}]$ with the relative pose between the $i$ th and $(i + 1)$ th frame.

\begin{equation}
\begin{aligned}
    E_{C}(R_{seq}, t_{seq}) & = \sum_{i=1}^{B-1}\left\Vert \begin{bmatrix} R_i  & t_i \\ 0 & 1 \end{bmatrix} \begin{bmatrix} R^{i+1}_i  & t^{i+1}_i \\ 0 & 1 \end{bmatrix} \right.\\
    & - \left. \begin{bmatrix} R_{i+1}  & t_{i+1} \\ 0 & 1 \end{bmatrix}\right\Vert_2 \label{eq:consistency}
\end{aligned}
\end{equation}

\paragraph{External 3D Body Pose Regularization}

Besides the external reprojection term, we also use the external 3D body poses to supervise the optimization of the egocentric 3D body pose. 
We define the external 3D pose term which measures the difference between the external body poses and the egocentric body poses after the rigid alignment:
% transformed from the egocentric camera space to the external camera space. 
% We make the optimized egocentric pose $\mathcal{P}_{i}^{ego}$ stay close to the external 3D pose estimation $\mathcal{P}_{i}^{ext}$ by defining the term as the difference between the 3D joint locations of egocentric and external view after the rigid alignment:

\begin{equation}
	E_{J}(\mathcal{P}_{seq}^{ego}, \mathcal{P}_{seq}^{ext}) = \sum_{i=1}^{B}\left\Vert \mathcal{P}_{i}^{ext} - \left[R_{i}^{pa}\mid t_{i}^{pa}\right]\mathcal{P}_{i}^{ego} \right\Vert_2^2 \label{eq:ext_3d_pose}
\end{equation}
where $\left[R_{i}^{pa} \mid t_{i}^{pa} \right]$ is the transformation matrix calculated with Procrustes analysis which rigidly aligns the external 3D pose estimation $\mathcal{P}_{i}^{ext}$ and the egocentric 3D pose $\mathcal{P}_{i}^{ego}$.

% With the external reprojection term and external 3D pose regularization term, we are able to generate accurate pseudo labels even though the human body in the egocentric view is seriously occluded, as illustrated in Fig.~\ref{fig:optimization_example}. With the external view, we are able to train the network with the accurate pseudo labels for the in-the-wild images, especially in the occluded cases. 

% We note that only by combining the egocentric view and external view, we can reconstruct accurate pseudo labels since the body parts can be either occluded in the egocentric or external view. 
By combining the body poses estimated from the egocentric view and external view, we can reconstruct more accurate pseudo labels.  
As shown in Fig.~\ref{fig:optimization_example}, the hands of the person are occluded in the external view, resulting in the tracking of the hands fails in the external view (Fig.~\ref{fig:optimization_example}, b), however, the hands can be clearly seen and tracked in the egocentric view (Fig.~\ref{fig:optimization_example}, d); 
on the other hand, the feet cannot be observed in the egocentric view and thus failed to be tracked in this view (Fig.~\ref{fig:optimization_example}, b), but can be easily viewed and tracked in the external view (Fig.~\ref{fig:optimization_example}, d). 
%Thus, either the optimizer with only the egocentric view (second image) or the external pose estimation method like VIBE~\cite{DBLP:conf/cvpr/KocabasAB20} (fourth image) cannot predict accurate pseudo labels. 
By joining the information from both views, we can successfully predict accurate 3D poses as the pseudo labels (Fig.~\ref{fig:optimization_example}, c).  
% combining the egocentric and external view in our optimization framework, we can predict accurate 3D poses as the pseudo labels, which is illustrated in the third image.
We note that the external camera is only used for generating the pseudo labels but at test time, only the egocentric camera is used. 

\begin{figure}
\centering
\includegraphics[width=0.98\linewidth]{figures/optimization_example/optimization_example_crop.pdf}
\caption{Our pseudo label generation method combines the information from both the egocentric view and external view, therefore leading to accurate pseudo labels (c). Only with the egocentric camera, the feet cannot be observed and well-tracked (b); Only with the external camera, the hands are occluded and result in the wrong result on the hand part (d).
% We note that the external camera is only used in the pseudo label generation for training, which is not used at test time.
}
% or external view is restrictive for predicting accurate 3D poses (the second and fourth image), while our optimization method gives reasonable result (the third image).
\label{fig:optimization_example}
\end{figure}



\paragraph{Camera Matrix Regularization}

We constrain the camera rotation matrix $R_{i}$ to be an orthogonal matrix:

\begin{equation}
	E_{J}(R_{seq}) = \sum_{i=1}^{B}\left\Vert R_{i}^TR_{i} - I \right\Vert_2^2 \label{eq:matrix}
\end{equation}
where $det(.)$ is the determinant of the matrix.

Through the optimization framework, we can get accurate 3D pose pseudo labels $\mathcal{P}_{seq}^{ego}$ for each egocentric frame in EgoPW dataset, which is further processed into the 2D heatmap $\mathcal{H_E}$ and the distance between joints and egocentric camera $\mathcal{D_E}$ with the fisheye camera model \cite{scaramuzza2014omnidirectional} described in supplementary materials. 

Different from previous single-view pose estimation methods which leverages the weak supervision from multiple views~\cite{iqbal2020weakly,rhodin2018learning,wandt2021canonpose,kocabas2019self}, our spatio-temporal optimization method generates the pseudo labels under the guidance of learned motion prior, making it robust to noisy and inaccurate 2D pose estimations, which is common for the 2D pose estimation results from the egocentric view.


\subsection{Training Egocentric Pose Estimation Network}\label{subsec:train}

After obtaining the pseudo labels for the EgoPW dataset, we train a single-image based egocentric pose estimation network on both the synthetic dataset from Mo$^2$Cap$^2$ and the EgoPW dataset. The pose estimation network contains a feature extractor $\Theta$ which encodes an image into a feature vector and a pose estimator $\Psi$ which decodes the feature vector to a heatmap and a 3D pose. Here, we note the synthetic dataset $S = \{I_S, H_S, D_S\}$ which is composed of synthetic images $I_S$ along with their corresponding heatmap $H_S$ and distance labels $D_S$ from Mo$^2$Cap$^2$ dataset, and the EgoPW dataset $E = \{I_E^{ego}, H_E, D_E, I_E^{ext} \}$ which is composed of egocentric in-the-wild images $I_E^{ego}$ along with pseudo heatmaps $H_E$, distance labels $D_E$ and corresponding external images $I_E^{ext}$. 
During the training process, we train the egocentric pose estimation network with two reconstruction loss terms and two adversarial loss terms. The reconstruction loss is defined as the mean squared error (MSE) between the predicted heatmaps/distances and heatmaps/distances from labels.

% After obtaining the pseudo labels for the EgoPW dataset, we train a single-image based egocentric pose estimation network on both the synthetic dataset from Mo$^2$Cap$^2$ and the EgoPW dataset. The pose estimation network contains a feature extractor $\Theta$ which encodes an image into a feature vector and a pose estimator $\Psi$ which decodes the feature vector to a heatmap and a 3D pose. Here, we note the synthetic dataset $S = \{\mathcal{I_S}, \mathcal{H_S}, \mathcal{D_S}\}$ which is composed of synthetic images $\mathcal{I_S}$ along with their corresponding heatmap $\mathcal{H_S}$ and distance labels $\mathcal{D_S}$ from Mo$^2$Cap$^2$ dataset, and the EgoPW dataset $\mathcal{E} = \{ \mathcal{I_E}^{ego}, \mathcal{H_E}, \mathcal{D_E}, \mathcal{I_E}^{ext} \}$ which is composed of egocentric in-the-wild images $\mathcal{I_E}^{ego}$ along with pseudo heatmaps $\mathcal{H_E}$, distance labels $\mathcal{D_E}$ and corresponding external images $\mathcal{I_E}^{ext}$. 
% During the training process, we train the egocentric pose estimation network with two reconstruction loss terms and two adversarial loss terms. The reconstruction loss is defined as the mean squared error (MSE) between the predicted heatmaps/distances and heatmaps/distances from labels.

\begin{equation}
    \begin{aligned}
        \mathcal{L}_{S} &= \text{mse}(\mathcal{\hat{H}_{S}}, \mathcal{H_{S}}) + \text{mse}(\mathcal{\hat{D}_{S}}, \mathcal{D_{S}})\\
        \mathcal{L}_{E} &= \text{mse}(\mathcal{\hat{H}_{E}}, \mathcal{H_{E}}) + \text{mse}(\mathcal{\hat{D}_{E}}, \mathcal{D_{E}})
    \end{aligned}
\end{equation}
where 
\begin{equation}
    \begin{aligned}
        \mathcal{F_{S}} = \Theta(\mathcal{I_{S}});& \mathcal{F_{E}}^{ego} = \Theta(\mathcal{I_{E}}^{ego})\\
        \mathcal{\hat{H}_{S}}, \mathcal{\hat{D}_{S}} = \Psi(\mathcal{F_{S}});& \mathcal{\hat{H}_{E}}, \mathcal{\hat{D}_{E}} = \Psi(\mathcal{F_{E}}^{ego})
    \end{aligned}
\end{equation}

Two adversarial losses are separately designed for learning egocentric semantic representation and bridging the domain gap between synthetic and real dataset. These two loss functions will be described below. 


\subsubsection{Learning Egocentric Image Representation}\label{subsubsec:ext_adv}

Note that the identity and body pose are exactly the same in a pair of egocentric-external images $\{ \mathcal{I_E}^{ego}, \mathcal{I_E}^{ext} \}$. Thus, the intermediate feature from the egocentric pose estimation network $\mathcal{F_{E}}^{ego}$ and the external pose estimation network $\mathcal{F_{E}}^{ext}$ should share the same semantic representation. Based on this observation, we use the features from external pose estimation network to supervise the egocentric pose estimation network. However, directly minimizing the distance between egocentric features $\mathcal{F_{E}}^{ego}$ and external features $\mathcal{F_{E}}^{ext}$ will not enhance the performance since the intermediate features of the egocentric and external view should be very different from each other due to significant difference on the view direction and camera distortions. To tackle this issue, we introduce the adversarial training strategy to align the intermediate features from egocentric and external networks. Specifically, we use an adversarial discriminator $\Lambda$ which takes the feature vectors extracted from a egocentric image and the corresponding in-the-wild images and predicts if the feature is from egocentric or external images. The adversarial discriminator $\Lambda$ is trained with a cross-entropy loss:

\begin{equation}
    \mathcal{L}_{R} = -E[\log(\Lambda(\mathcal{F_E}^{ego}))] - E[\log(1 - \Lambda(\mathcal{F_E}^{ext}))]
\end{equation}

During the training process, the egocentric pose estimation network is trained to produce the features to fool the domain classifier $\Lambda$ such that $\Lambda$ cannot distinguish whether the feature is from an egocentric or external image. In order to achieve this, the pose estimation network is trained to generate features with semantic representation of human body, since the semantic representation of corresponding egocentric and external images should be the same. This is proved by Figure, where the features from egocentric network focus on the representation of human body after the adversarial training process.


\subsubsection{Adversarial Domain Adaptation}\label{subsubsec:da}
To bridge the domain gap between the synthetic and real data domains, following Tzeng~\etal~\cite{tzeng2017adversarial}, we introduce an adversarial discriminator $\Gamma$ which takes as input the feature vectors extracted from a synthetic image and an in-the-wild image, and determines if the feature is extracted from an in-the-wild image. 
The adversarial discriminator $\Gamma$ is trained with a cross-entropy loss:

\begin{equation}
    \mathcal{L}_{D} = -E[\log(\Gamma(\mathcal{F_S}))] - E[\log(1 - \Gamma(\mathcal{F_T}))]
\end{equation}

Once the discriminator $\Gamma$ has been trained, the feature extractor $\Theta$ maps the images from different domains to the same feature space such that the classifier $\Gamma$ cannot tell if the features are extracted from synthetic images or real images. Therefore, the pose estimator $\Psi$ can predict more accurate poses for the in-the-wild data. 

% Aside from training the network on the EgoPW dataset, we also train the pose estimation network simultaneously on the synthetic dataset considering that synthetic data has its advantages compared to real data, e.g. it is easily accessible and has large variations on poses and backgrounds. To address the domain gap between the synthetic data and real data, we introduce a new adversarial domain adaptation method. Specifically, we extract the features from the synthetic data and real data and use an adversarial discriminator to distinguish if the feature is from synthetic data or real data. Once trained, the feature extractor would learn to produce the features in the same feature space for synthetic data and real data. In this way, our method is able to make full use of the synthetic data and real data, thus achieving better results. 


==> sections/intro_new.tex <==
\section{Introduction}

% \ME{make sure that the '' semantic representation '' termonolgy is fixed during the paper. I think it is sometimes used interchangibly with '' features of extracted images ''. }

Egocentric motion capture using head- or body-mounted cameras has recently become popular, because traditional motion capture systems with outside-in cameras have limitations when the person is moving around in a large space and thus restrict the scope of applications. Different from traditional  systems, the egocentric motion capture system is mobile, flexible, and has no requirements on recording space, which enables capturing a wide range of human activities for many applications, such as wearable medical monitoring, sports analysis, and $x$R.  

\begin{figure}
\begin{center}
\includegraphics[width=0.97\linewidth]{figures/teaser/teaser_with_external_red_crop.pdf}
\end{center}
   \caption{Comparing with Mo$^2$Cap$^2$, our method gets a more accurate egocentric pose from a single in-the-wild image, especially when the body parts are occluded. Note that the external images are only used for visualization and the 3D poses in this figure are only generated from the egocentric images.}
\label{fig:teaser}
\end{figure}

In this work, we focus on estimating the full 3D body pose with a single head-mounted fisheye camera. The most related works to ours are Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} and $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19}. 
While these methods have produced compelling results they are only trained on the synthetic data as limited real data exists and therefore suffer from significant performance drop on real data due to the domain gap between synthetic and real images.
Furthermore, due to the similar reason, these methods often struggle with the cases when the human body is occluded by or interacting with the surrounding scene (See the Mo$^2$Cap$^2$ results in Fig.~\ref{fig:teaser}).
% mainly because the training supervision is only from a single egocentric view.

To address the limited data issue, we capture a large-scale in-the-wild egocentric dataset called \emph{Egocentric Poses in the Wild (EgoPW)}. This dataset is the largest egocentric in-the-wild dataset, containing more than 312k frames and covering 20 different daily activities in 8 everyday scenes. To improve the accuracy of the estimated poses from a single egocentric image, one possible way is to use a multi-view camera setup to capture training data to obtain a ground truth 3D body pose or apply multi-view weak supervision. However, this setup is impractical for recording in an environment with limited space (e.g. in the small kitchen shown in Fig.~\ref{fig:optimization_example}), which is a common recording scenario. Therefore, considering a balance between flexibility and data quality, we used a new device setup consisting of an egocentric camera and a single auxiliary external camera. The extra external view could provide additional supervision during training, especially on the occluded regions in the egocentric view (e.g. the lower body part). 

We then propose a new egocentric pose estimation method for training on the EgoPW dataset in a weakly supervised way. Specifically, we propose a spatio-temporal optimization method to generate accurate 3D poses for each frame in the EgoPW dataset. The generated poses are further used as pseudo labels for training an egocentric pose estimation network~\cite{DBLP:journals/tvcg/XuCZRFST19}. To improve the estimation accuracy, we propose an adversarial training strategy based on the observation that the feature representation of human body from the egocentric view and external view should contain similar parts. Specifically, we enforce the feature distribution extracted from these two views to be consistent by fooling a discriminator not being able to detect which views the features are from. 
To further improve the performance of pose estimation network, besides the EgoPW dataset, we also use a synthetic dataset~\cite{DBLP:journals/tvcg/XuCZRFST19} to train the egocentric pose estimation network and adopt a domain adaptation strategy to minimize the domain gap between synthetic and real data. 

% We then propose a new egocentric pose estimation method for training on the EgoPW dataset in a weakly supervised way. Specifically, we propose a spatio-temporal optimization method to generate accurate 3D poses for each frame in the EgoPW dataset. The generated poses are further used as pseudo labels for training an egocentric pose estimation network~\cite{DBLP:journals/tvcg/XuCZRFST19}. To improve the estimation accuracy, we propose an adversarial training strategy based on the observation that the feature representation of human body from the egocentric view and external view should be similar. Specifically, we enforce the features extracted from these two views to be consistent by fooling a discriminator not being able to detect which views the features are from. 
% To further improve the performance of pose estimation network, besides the EgoPW dataset, we also use a synthetic dataset~\cite{DBLP:journals/tvcg/XuCZRFST19} to train the egocentric pose estimation network and adopt a domain adaptation strategy to minimize the domain gap between synthetic and real data. 

% In order to leverage the supervision from both the external view and egocentric view, we generate pseudo labels by developing a new spatio-temporal optimization method that leverages the 2D and 3D keypoints detected from the two views. The pseudo labels are then used to train the pose estimation network. We note that the external view is only used for training, but not for testing. 
% \JW{To further improve the accuracy of the estimated poses, we introduce a new adversarial training strategy by aligning the semantic representation of egocentric and external images.
% We also use synthetic dataset to train our network and adopt a domain adaptation strategy that minimizes the domain gap. The network trained with our method gives accurate 3D pose even under serious occlusions (See our results in Figure~\ref{fig:teaser}).}

% \JW{Since the corresponding egocentric and external images share the same identity and body pose, the intermediate features of them should also share the same semantic representation. Aside from optimizing the pseudo labels, we introduce a new adversarial learning strategy to align the feature representation and supervise the training of egocentric pose estimation network.}

% \JW{To further improve the accuracy of the estimated poses, we also adopt a domain adaptation strategy that minimizes the domain gap between synthetic and real dataset, and a bootstrapping strategy that optimize pseudo labels and the pose estimation network in a loop. The network trained with our method gives accurate 3D pose even under serious occlusions (See our results in Figure~\ref{fig:teaser}). }

We evaluate our method on the test data provided by Wang~\etal~\cite{wang2021estimating} and Xu~\etal~\cite{DBLP:journals/tvcg/XuCZRFST19}. Our method significantly outperforms the state-of-the-art methods both quantitatively and qualitatively. We also show qualitative results on various in-the-wild images, demonstrating that our method can predict accurate 3D poses in the in-the-wild scenes, especially when the body joints are seriously occluded (See our results in Figure~\ref{fig:teaser}). To summarize, our contributions are:

\begin{itemize}
\itemsep -0.1em
    % \item A new approach to estimating accurate 3D human poses from a single in-the-wild egocentric image;
    \item A new learning approach for egocentric human pose estimation by leveraging supervision from an external view;
    % \item \DL{The first contribution is very important and it should be more specific. A new method that does X is a quite general statement. I believe we should state here that we propose a new learning method/framework for egocentric human pose estimation that leverages information from external views for improving the feature representation.}
    \item A large-scale in-the-wild egocentric dataset (EgoPW) captured with a head-mounted fisheye camera and an external normal camera. We will make this dataset publicly available;
    \item A new optimization method to generating the pseudo labels for the in-the-wild dataset by incorporating the supervision from the external view;
    \item  An adversarial method for training the network by learning the feature representation of egocentric images with external feature representation. 
    \LJ{A new efficient strategy for learning egocentric feature representation with the supervision from the high-quality features extracted by a pretrained model trained on a large amount of external-view data. }
    % \item  An adversarial learning method to enforcing the features of body parts from the egocentric view and external view to be consistent. \DL{this contribution is somehow in the first, so it could be emphasized there and removed from here. Instead, you could claim SotA results on two datasets}
\end{itemize}


==> sections_old/experiments.tex <==
\section{Experiments}

\subsection{Datasets}

% Our network is trained on the synthetic dataset from Mo$^2$Cap$^2$ \cite{DBLP:journals/tvcg/XuCZRFST19} and the training split of EgoPW dataset. The Mo$^2$Cap$^2$ training dataset contains 530k images under 700 body textures.
We quantitatively evaluate our finetuned network on the real-world dataset from Mo$^2$Cap$^2$ \cite{DBLP:journals/tvcg/XuCZRFST19} and Wang \etal~\cite{wang2021estimating}. The real-world dataset in Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} contains 2.7k frames of two people captured in indoor and outdoor scenes, and that in Wang \etal~\cite{wang2021estimating} contains 12k frames of two people captured in the studio. To measure the accuracy of our pseudo labels, we evaluate our optimization method (Sec~\ref{subsec:optimizer}) only on the dataset from Wang \etal~\cite{wang2021estimating} since the Mo$^2$Cap$^2$ dataset does not include the external view.

% These datasets have the ground truth 3D poses from a multi-view motion capture system while they are mostly captured in the studio. \LJ{suggest removing the above sentence} 
To evaluate our method on the in-the-wild data, we also conduct a qualitative evaluation on the test set of EgoPW dataset. The EgoPW dataset will be made publicly available, and more details and comparisons to other datasets are included in the supplementary materials.

\subsection{Evaluation Metrics}
We measure the results of our method as well as other baseline methods with two metrics, PA-MPJPE and BA-MPJPE, which estimate the accuracy of a single body pose. For \textbf{PA-MPJPE}, we rigidly align the estimated pose $\mathcal{\hat{P}}$ of each frame to the ground truth pose $\mathcal{P}$ using Procrustes analysis \cite{kendall1989survey}. In order to eliminate the influence of body scale, we also report the \textbf{BA-MPJPE} scores. We first resize the bone length of each predicted body pose $\mathcal{\hat{P}}$ and ground truth body pose $\mathcal{P}$ to the bone length of a standard skeleton. Then, we calculate the PA-MPJPE between the two resulting poses. 

\begin{figure*}
\centering
\includegraphics[width=0.975\linewidth]{figures/results/results_wide_crop.pdf}
\caption{Qualitative comparison between our method and the state-of-the-art methods. From left to right: input image, Mo$^2$Cap$^2$ result, $x$R-egopose result, our result and external image. The ground truth pose is shown in red. Note that the external images is only for visualization and they are not used for predicting the pose.}
\label{fig:results}
\end{figure*}

\subsection{Accuracy of Pseudo Labels}\label{subsec:pseudo_labels}

\begin{table}[h]
\begin{center}
\small
\begin{tabular}{p{0.19\textwidth}
>{\centering}p{0.1\textwidth}
>{\centering\arraybackslash}p{0.1\textwidth}}
\hlineB{2.5}
Method & PA-MPJPE & BA-MPJPE \\ \hline
Mo$^2$Cap$^2$ & 102.3 & 74.46 \\
$x$R-egopose & 112.0 & 87.20 \\
Wang \etal~\cite{wang2021estimating} & 83.40 & 63.88 \\
VIBE~\cite{DBLP:conf/cvpr/KocabasAB20} & 68.13 & 52.99 \\
\hline
Our Optimizer & \textbf{57.19} & \textbf{46.14}\\
\hlineB{2.5}
\end{tabular}
\end{center}
\caption{The performance of our optimization framework on  Wang \etal's dataset. Our optimization method outperforms all previous egocentric pose estimation methods and the state-of-the-art pose estimation method of the external view.}
\label{table:pseudo_labels}
% \vspace{-1em}
\end{table}

In this paper, we first generate the pseudo labels with the optimization framework (Sec.~\ref{subsec:optimizer}) and use them to train the network. Thus, the accuracy of pseudo labels are critical. In this experiment, we evaluate the accuracy of pseudo labels on the Wang~\etal's dataset and show the results in Table~\ref{table:pseudo_labels}. 
This table shows that our method outperforms all the baseline methods by leveraging both the egocentric view and external view during optimization. Note that though compared in Table~\ref{table:pseudo_labels}, we cannot use any external-view based pose estimation method, \eg VIBE~\cite{DBLP:conf/cvpr/KocabasAB20} and 3DPW~\cite{von2018recovering}, for training the egocentric pose estimation network. This is because the relative pose between the external and egocentric camera is unknown, making it impossible to obtain the egocentric body pose only from the external view. Comparing with our optimization approach, the method in~\cite{wang2021estimating} performs worse due to the lack of external-view supervision. It is still possible to use this method to generate pseudo labels for training the network yet resulting in worse performance, which is demonstrated in the ablation study (Sec.~\ref{subsec:ablation}).



\subsection{Comparisons on 3D Pose Estimation}

\begin{table}[h]
\begin{center}
\small
\begin{tabularx}{0.47\textwidth} { 
   >{\raggedright\arraybackslash}X 
   >{\centering\arraybackslash}X 
   >{\centering\arraybackslash}X  }
\hlineB{2.5}
Method & PA-MPJPE & BA-MPJPE \\
\hline
\multicolumn{2}{l}{\textbf{Wang \etal's test dataset}} \\
\hline
Wang \etal~\cite{wang2021estimating} & 83.40 & 63.88 \\
\hline
Rhodin \etal~\cite{rhodin2018learning} & 89.67 & 73.56 \\
Mo$^2$Cap$^2$ & 102.3 & 74.46 \\
$x$R-egopose & 112.0 & 87.20 \\
Ours &\textbf{82.61} & \textbf{65.18} \\
\hlineB{2.5}
\multicolumn{2}{l}{\textbf{Mo$^2$Cap$^2$ test dataset}} \\
\hline
Rhodin \etal~\cite{rhodin2018learning} & 97.69 & 76.92 \\
Mo$^2$Cap$^2$ & 91.16 & 70.75 \\
$x$R-egopose & 86.85 & 66.54 \\
Ours &  \textbf{81.68} & \textbf{63.01} \\
\hlineB{2.5}
\end{tabularx}
\end{center}
\caption{The experimental results on Wang~\etal's test dataset and Mo$^2$Cap$^2$ test dataset \cite{DBLP:journals/tvcg/XuCZRFST19}. Our method outperforms the state-of-the-art methods, i.e. Mo$^2$Cap$^2$ \cite{DBLP:journals/tvcg/XuCZRFST19} and $x$R-egopose \cite{DBLP:conf/iccv/TomePAB19} on both of the metrics. Our method also outperforms a video-based method~\cite{wang2021estimating} in terms of  PA-MPJPE.
% \vspace{-0.5em}
}
\label{table:main}
\end{table}


We compare our approach with previous state-of-the-art single-frame-based methods on the test dataset from~\cite{wang2021estimating} under the ``Wang \etal's test dataset'' in Table~\ref{table:main}. Since the code or the predictions of $x$R-egopose are not publicly available, we use our reimplementation of $x$R-egopose instead. On this dataset, our method outperforms Mo$^2$Cap$^2$ by 20.1\% and $x$R-egopose by 27.03\% respectively.
Our single-image based method performs even better than Wang~\etal~\cite{wang2021estimating} in terms of PA-MPJPE. 
% Note that Wang~\etal uses a temporal-based egocentric pose optimization method which requires a sequence as input and cannot ensure real-time performance, while our work predicts egocentric pose from a single image and runs in real time. 
Note that Wang~\etal uses a video-based optimization method, which requires a sequence as input (for computing SLAM and temporal optimization) and cannot achieve real-time performance. In contrast, we estimate 3D poses from a single egocentric image at inference which is a more difficult problem. As a result, our method can run in real time.
% \KS{What are the advantage of our method over Wang et al? Since the difference is not so much, we need to explicitly re-iterate our advantages over the previous method here.}

We also compared with previous methods on the Mo$^2$Cap$^2$ test dataset in Table~\ref{table:main}. Since the camera parameters used in Mo$^2$Cap$^2$ are different from those used in this work, we train our network on the unlabeled dataset from the Mo$^2$Cap$^2$ work. Since the external view is not available for the Mo$^2$Cap$^2$ test dataset, we generate the pseudo labels with the optimize equation~\ref{eq:optim} without $E_{R}^{ext}$, $E_{J}^{ext}$, $E_{C}$, and $E_{M}$. Next, we follow Sec.~\ref{subsec:train} to train the pose estimation network on the Mo$^2$Cap$^2$ test dataset and show the results under the ``Mo$^2$Cap$^2$ test dataset'' in Table~\ref{table:main}. Our method performs better than Mo$^2$Cap$^2$ and $x$R-egopose by 10.4\% and 6.0\% respectively on Mo$^2$Cap$^2$ test dataset.

From the results in Table~\ref{table:main}, we can see that our approach significantly outperforms all previous methods on the single-frame egocentric pose estimation task. More quantitative results on each type of motion have included in the supplementary materials. For the qualitative comparison, we show the results of our method on the studio dataset and in-the-wild dataset in Fig.~\ref{fig:results}. Our method performs much better comparing to Mo$^2$Cap$^2$ and $x$R-egopose, especially for the in-the-wild cases where the body parts are occluded. Please refer to the supplementary materials for more qualitative results.




\subsection{Ablation Study}\label{subsec:ablation}

\begin{table}[h]
\begin{center}
\small
\begin{tabular}{p{0.2\textwidth}
>{\centering}p{0.1\textwidth}
>{\centering\arraybackslash}p{0.1\textwidth}}
\hlineB{2.5}
Method & PA-MPJPE & BA-MPJPE \\ \hline
Mo$^2$Cap$^2$ & 102.3 & 74.46 \\
$x$R-egopose & 112.0 & 87.20 \\
\hline
w/o external view  & 86.72 & 67.11 \\
w/o domain discriminator  & 86.24 & 65.74 \\
w/o bootstrapping  & 91.01 & 67.93 \\
Unsupervised DA  & 91.56 & 69.17 \\
Only bootstrapping & 88.47 & 68.49 \\
\hline
Ours & \textbf{81.73} & \textbf{64.05}\\
\hlineB{2.5}
\end{tabular}
\end{center}
\caption{The quantitative results of ablation study.}
\label{table:ablation}
% \vspace{-1em}
\end{table}

% In this section, we conduct experiments to further evaluate the effects of individual components in our approach. 
\paragraph{Supervision from the external view.}
In our work, we introduce the external view as a supervision for training the network on the real EgoPW dataset. The external view enables the generating accurate pseudo labels, especially when the human body parts are occluded in the egocentric view but can be observed in the external view. Without the external view, the obtained pseudo labels is less accurate and will further affects the network performance. In order to demonstrate this, we first generate the pseudo labels without any external supervision, \ie run our optimizer without $E_{R}^{ext}$, $E_{J}^{ext}$, $E_{C}$, and $E_{M}$, and then train the pose estimation network on this new pseudo labels. The result is shown in the ``w/o external view'' row of Table~\ref{table:ablation}.
We also show the qualitative results in Figure~\ref{fig:wo_external} where we evaluate our method with and without external view supervision.
% We also show the qualitative results in Figure~\ref{fig:wo_external} which compares our method with the result without any external view supervision \LJ{where we evaluate our method with and without external view supervision}.
Both the qualitative and quantitative results demonstrate that by introducing the external supervision, the performance of our finetuned pose estimation network is significantly better especially on the occlusion cases.

\begin{figure}
\centering
\includegraphics[width=0.98\linewidth]{figures/wo_external/wo_external_crop.pdf}
\caption{The results of our method with (c) and without external view (b). The network cannot predict accurate poses for the occluded cases without the external view supervision. 
The external view is only for visualization and not used for predicting the pose.
}
\label{fig:wo_external}
\end{figure}

\paragraph{Adversarial domain adaptation strategy.}
In our work, we first train the pose estimation network on the synthetic images and in-the-wild images with the adversarial domain adaptation module (Sec.~\ref{subsubsec:da}). With a domain classifier, this module eliminates the domain gap and enables the full use of both the synthetic and real images.
In order to investigate the efficacy of this strategy, we removed the domain classifier in our training framework and train the network without $\mathcal{L}_{Dis}$. We evaluate this network on Wang~\etal's dataset and show the quantitative results in the row of ``w/o domain discriminator'' in Table~\ref{table:ablation}. After removing the domain classifier, our method suffers from performance drop, which demonstrates the necessity of this module.


\paragraph{Bootstrapping module.}
In order to alleviate the influence of inaccurate pseudo labels, we introduce the bootstrapping strategy (Sec.~\ref{subsubsec:bootstrapping}).
% by updating the pseudo labels and pose estimation network in a loop. 
To prove its importance, we removed this module from our pipeline and train the network only with the adversarial domain adaptation module. The experimental results are shown in the ``w/o bootstrapping'' of Table~\ref{table:ablation}. Without the bootstrapping module, the network performs worse since the network is trained on inaccurate pseudo labels.

\paragraph{}

\paragraph{Comparison with only using unsupervised domain adaptation.}
In this experiment, we compare our approach with the unsupervised adversarial domain adaptation method~\cite{tzeng2017adversarial} which is commonly used for transfer learning tasks. We first train the network only with the $\mathcal{L_S}$ and $\mathcal{L}_{Dis}$ in the adversarial domain adaptation module (Sec.~\ref{subsubsec:da}) and show the results in the ``Unsupervised DA'' of the Table~\ref{table:ablation}. Our approach significantly outperforms the unsupervised domain adaptation method due to our high-quality pseudo labels. 
Even though we train the network on pseudo labels without bootstrapping, the results are still better than the unsupervised domain adaptation results, which is demonstrated by the comparison between ``Unsupervised DA'' and ``w/o bootstrapping'' in Table~\ref{table:ablation}. This is because the pseudo labels encode information of the external view, which is more effective than the unsupervised domain adaptation method without any external supervision.

\paragraph{Comparison with only using bootstrapping.}
In this experiment, we compare the our method with the network only trained with the bootstrapping strategy. We directly update the network with bootstrapping (Sec.~\ref{subsubsec:bootstrapping}) without first training the network both on real and synthetic dataset in Sec.~\ref{subsubsec:da}, \ie we only use modules in the yellow dashed box in Figure~\ref{fig:framework}. The result is shown as ``only bootstrapping'' in Table~\ref{table:ablation}. We can see that training on both the synthetic and EgoPW dataset is crucial to our method, since the synthetic dataset covers a large number of egocentric training data with accurate ground truth, while our EgoPW dataset contains the images in the real-world domain. 
% It is very necessary to leverage a domain adaptation method to bridge the domain 

==> sections_old/intro_new_lingjie.tex <==
\section{Introduction}

Egocentric motion capture using head- or body-mounted cameras has become popular recently because traditional motion capture systems with outside-in cameras have strong limitations when the person is moving around in a large space and thus restrict the scope of applications. Different from traditional  systems, the egocentric motion capture system is mobile, flexible, and has no requirements on recording space, which enables capturing a wide range of human activities for many applications, such as wearable medical monitoring, sports analysis, and $x$R.  

\begin{figure}
\begin{center}
\includegraphics[width=0.97\linewidth]{figures/teaser/teaser_with_external_red_crop.pdf}
\end{center}
   \caption{Comparing with Mo$^2$Cap$^2$, our method gets a more accurate egocentric pose from a single in-the-wild image, especially when the body parts are occluded. Note that the external images are only used for visualization and the 3D poses in this figure are only generated from the egocentric images.}
\label{fig:teaser}
\end{figure}

In this work, we focus on estimating the full 3D body pose with a single head-mounted fisheye camera. The most related works to ours are Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} and $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19}. 
Despite these methods have produced compelling results, existing methods are only trained on the synthetic data as limited real data exist and therefore suffer from significant performance drop on real data due to the domain gap between synthetic and real images. 
Furthermore, these methods often struggle with the cases when the human body is occluded by or interacting with the surrounding scene (See the Mo$^2$Cap$^2$ results in Fig.~\ref{fig:teaser}), mainly because the training supervision is only from a single egocentric view. 

To address these issues, we propose a new method to estimate 3D body pose with a single egocentric camera, which is trained on a new in-the-wild dataset. Specifically, we firstly capture a large-scale in-the-wild egocentric dataset called \emph{Egocentric Poses in the Wild (EgoPW)} with a new device setup consisting of an egocentric camera and an auxiliary external camera. Note that this dataset is the largest egocentric in-the-wild dataset, containing more than 312k frames and covering 20 different daily activities in 8 everyday scenes. 

We also note that the new device setup used for data capture has several advantages over existing setups. Compared to a multi-view setup with dense cameras used in [citations?], this new device setup is lightweight, flexible and allows recording in an environment with limited space; compared to a single egocentric camera setup, the additional external view would provide the information of the occluded regions in the egocentric view, e.g. the lower body part. 

% To address these issues, we propose a new method to estimate 3D body pose with a single egocentric camera, which is trained on a new in-the-wild dataset. Specifically, we capture a large-scale in-the-wild egocentric dataset called \emph{Egocentric Poses in the Wild (EgoPW)} with a new device setup consisting of an egocentric camera and an auxiliary external camera; we then design a method for training on the new dataset in a weakly supervised manner based on the 2D supervision from the egocentric view and external view. Note that this dataset is the largest egocentric in-the-wild dataset, containing more than 312k frames and covering 20 different daily activities in 8 everyday scenes. We also note that the new device setup used for data capture has several advantages over existing setups.  Compared to a multi-view setup with dense cameras used in [citations?], this new device setup is lightweight, flexible and allows recording in an environment with limited space; compared to a single egocentric camera setup, the additional external view would provide the information of the occluded regions in the egocentric view, e.g. the lower body part. 

Next, we design a method for training on the new dataset in a weakly supervised manner based on the information from the egocentric view and external view. Firstly, we extend the spatio-temporal optimization method proposed by Wang~\etal~\cite{wang2021estimating} to the multi-view scenario and generate accurate 3D poses for each frame in EgoPW dataset. The generated poses are further used as pseudo labels for training the pose estimation network on the EgoPW dataset. Moreover, we introduce an adversarial training strategy to align the semantic representation of egocentric and external images, since both the views share the same identity and body pose. To further improve the accuracy of the estimated poses, the synthetic dataset is also used to train our network and a domain adaptation strategy is adopted to minimizes the domain gap between synthetic and real data. The network trained with our method gives accurate 3D pose even under serious occlusions (See our results in Figure~\ref{fig:teaser}).

% In order to leverage the supervision from both the external view and egocentric view, we generate pseudo labels by developing a new spatio-temporal optimization method that leverages the 2D and 3D keypoints detected from the two views. The pseudo labels are then used to train the pose estimation network. We note that the external view is only used for training, but not for testing. 
% \JW{To further improve the accuracy of the estimated poses, we introduce a new adversarial training strategy by aligning the semantic representation of egocentric and external images.
% We also use synthetic dataset to train our network and adopt a domain adaptation strategy that minimizes the domain gap. The network trained with our method gives accurate 3D pose even under serious occlusions (See our results in Figure~\ref{fig:teaser}).}

% \JW{Since the corresponding egocentric and external images share the same identity and body pose, the intermediate features of them should also share the same semantic representation. Aside from optimizing the pseudo labels, we introduce a new adversarial learning strategy to align the feature representation and supervise the training of egocentric pose estimation network.}

% \JW{To further improve the accuracy of the estimated poses, we also adopt a domain adaptation strategy that minimizes the domain gap between synthetic and real dataset, and a bootstrapping strategy that optimize pseudo labels and the pose estimation network in a loop. The network trained with our method gives accurate 3D pose even under serious occlusions (See our results in Figure~\ref{fig:teaser}). }

We evaluate our method on the test data provided by Wang~\etal~\cite{wang2021estimating} and Xu~\etal~\cite{DBLP:journals/tvcg/XuCZRFST19}. Our method significantly outperforms the state-of-the-art methods both quantitatively and qualitatively. We also show qualitative results on various in-the-wild images, demonstrating that our method can predict accurate 3D poses in the in-the-wild scenes, especially when the body joints are seriously occluded. To summarize, our contributions are:

\begin{itemize}
\itemsep -0.1em
    \item A new approach for estimating accurate 3D human poses from a single in-the-wild egocentric image;
    \item A new in-the-wild egocentric pose estimation dataset (EgoPW) captured with a head-mounted fisheye camera and an external normal camera. We will make this dataset publicly available;
    \item A novel optimization method to generating the pseudo labels for the in-the-wild dataset by incorporating the supervision from the external view;
    \item  An adversarial learning method for aligning the semantic features between egocentric and external view.
\end{itemize}


==> sections_old/introduction.tex <==
\section{Introduction}



Egocentric motion capture using head- or body-mounted cameras has become popular recently because traditional motion capture systems with outside-in cameras have strong limitations when the person is moving around in a large space and thus restrict the scope of applications. Different from traditional methods, the egocentric motion capture system is mobile, flexible, and has no requirements on recording space, which enables capturing a wide range of human activities for many applications, such as wearable medical monitoring, sports analysis, and $x$R.  

\begin{figure}
\begin{center}
\includegraphics[width=0.97\linewidth]{figures/teaser/teaser_with_external_red_crop.pdf}
\end{center}
   \caption{Comparing with Mo$^2$Cap$^2$, our method gets a more accurate egocentric pose from a single in-the-wild image, especially when the body parts are occluded. Note that the external images are only used for visualization and the 3D poses in this figure are only generated from the egocentric images.}
\label{fig:teaser}
\end{figure}

In this work, we focus on estimating the full 3D body pose with a single head-mounted fisheye camera. The most related works to ours are Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} and $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19}. 
Despite these methods have produced compelling results, existing methods are only trained on the synthetic data and therefore suffer from significant performance drop on real data due to the domain gap between synthetic and real images. 
Furthermore, due to the difficulty in creating challenging synthetic scenarios of occlusions and human-object interactions, these methods often struggle with the cases when the human body is occluded by or interacting with the surrounding scene (See the Mo$^2$Cap$^2$ results in Fig.~\ref{fig:teaser}).

\JW{To improve the pose estimation on real-world data and handle the issue caused by occlusions, we collected a new in-the-wild egocentric dataset called \emph{Egocentric Poses in the Wild (EgoPW)} for training the pose estimation network. 
This dataset is the first egocentric in-the-wild dataset, which contains more than 312k frames and covers 20 different daily activities in 8 everyday scenes.}

\JW{However, setting up multi-view system for capturing the ground truth is challenging for the in-the-wild dataset. To this end, we set up a single synchronized external normal camera and collect images from the external view when collecting the EgoPW dataset. The additional external view would provide the information of the occluded regions in the egocentric view, e.g. the lower body part.}

\JW{In order to leverage the supervision from the external view, we generate accurate pseudo labels by developing a new spatio-temporal optimization method that leverages the 2D and 3D keypoints from both the egocentric view and the external view. Afterwards, the pseudo labels are used for training the pose estimation network. We note that the external view is only used for training, but not for testing. 
Comparing with available single-view pose estimation methods with multi-view weak supervision~\cite{iqbal2020weakly,rhodin2018learning,wandt2021canonpose,kocabas2019self}, our spatio-temporal optimization method generates the pseudo labels under the guidance of learned motion prior. This makes it robust to noisy and inaccurate 2D pose estimations, which is common for the 2D pose estimation results from the egocentric view.}

\JW{Since the corresponding egocentric and external images share the same identity and body pose, the intermediate features of them should also share the same semantic representation. Aside from optimizing the pseudo labels, we introduce a new adversarial learning strategy to align the feature representation and supervise the training of egocentric pose estimation network.}

\JW{To further improve the accuracy of the estimated poses, we also adopt a domain adaptation strategy that minimizes the domain gap between synthetic and real dataset, and a bootstrapping strategy that optimize pseudo labels and the pose estimation network in a loop. The network trained with our method gives accurate 3D pose even under serious occlusions (See our results in Figure~\ref{fig:teaser}). }

% To improve the pose estimation on real-world data and handle the issue caused by occlusions, we collected a new in-the-wild egocentric dataset with a head-mounted fisheye camera and an external normal camera, called \emph{Egocentric Poses in the Wild (EgoPW)}, for training the pose estimation network. 
% This dataset is the first egocentric in-the-wild dataset, which contains more than 312k frames and covers 20 different daily activities in 8 everyday scenes.

% However, setting up multi-view system for capturing the ground truth is challenging for the in-the-wild dataset. In order to provie 
% Considering the challenges in obtaining ground truth in the real world, we resort to the 

% In order to generate accurate 3D poses as pseudo labels for the EgoPW dataset, we develop a new optimization method that leverages the 2D and 3D keypoints from both the egocentric view and the external view. 
% The additional external view would provide the information of the occluded regions in the egocentric view, e.g. the lower body part, and thus improves the quality of pseudo labels. 
% We note that the external view is only used for training, but not for testing. 
% Comparing with other motion capture approaches such as multi-view motion capture systems~\cite{elhayek2015efficient, pavlakos2017harvesting,liu2013markerless} and IMU-based motion capture systems~\cite{huang2018deep,von2017sparse,von2018recovering}, our approach is simple, flexible, and does not need fixed capture space or any special device.

% Considering that synthetic data has its advantages compared to real data, e.g. it is easily accessible and has large variations on poses and backgrounds, we use both synthetic data and real data for training. Due to the domain gap between the synthetic data and real data, using the mixed data for efficient training is a challenge. To address this issue, we introduce a new adversarial domain adaptation method. Specifically, we extract the features from the synthetic data and real data and use an adversarial discriminator to distinguish if the feature is from synthetic data or real data. Once trained, the feature extractor would learn to produce the features in the same feature space for synthetic data and real data to fool the discriminator. 
% In this way, our method is able to make full use of the synthetic data and real data, thus achieving better results. 
% To further improve the accuracy of the estimated poses, we propose a bootstrapping strategy, \ie the pseudo labels are optimized based on the updated egocentric network prediction, while the egocentric network is finetuned with the updated pseudo labels. The finetuned network gives accurate 3D pose even under serious occlusions (See our results in Figure~\ref{fig:teaser}). 

We evaluate our method on the test data provided by Wang~\etal~\cite{wang2021estimating} and Xu~\etal~\cite{DBLP:journals/tvcg/XuCZRFST19}. Our method significantly outperforms the state-of-the-art methods both quantitatively and qualitatively. We also show qualitative results on various in-the-wild images, demonstrating that our method can predict accurate 3D poses in the in-the-wild scenes, especially when the body joints are seriously occluded. To summarize, our contributions are:

\JW{\begin{itemize}
\itemsep -0.1em
    \item A new approach for estimating accurate 3D human poses from a single in-the-wild egocentric image;
    \item A new in-the-wild egocentric pose estimation dataset (EgoPW) captured with a head-mounted fisheye camera and an external normal camera. We will make this dataset publicly available;
    \item A novel optimization method to generating the pseudo labels for the in-the-wild dataset by incorporating the supervision from the external view;
    \item  An adversarial learning method for aligning the semantic features between egocentric and external view.
\end{itemize}}


==> sections_old/method.tex <==
\section{Method}

We propose a new approach to train an egocentric pose estimation network. This network is able to estimate an accurate 3D body pose from a single egocentric in-the-wild image. The overview of our approach is illustrated in Fig.~\ref{fig:framework}. We first capture a large egocentric in-the-wild dataset, called \emph{EgoPW}, which contains synchronized egocentric image sequences and external image sequences (Sec.~\ref{subsec:dataset}). Next, we generate the pseudo labels for the EgoPW dataset with an optimization-based framework. This framework takes a sequence in a time window with $B$ frames of egocentric images $\mathcal{I}^{ego}_{seq}=\{\mathcal{I}^{ego}_{1},\dots,\mathcal{I}^{ego}_{B}\}$ and external images $\mathcal{I}^{ext}_{seq}=\{\mathcal{I}^{ext}_{1},\dots,\mathcal{I}^{ext}_{B}\}$ as input and outputs egocentric 3D poses $\mathcal{P}^{ego}_{seq}=\{\mathcal{P}^{ego}_{1},\dots,\mathcal{P}^{ego}_{B}\}$ as the pseudo labels (Sec.~\ref{subsec:optimizer}). Then, we propose an adversarial domain adaptation strategy to train the egocentric pose estimation network on both the synthetic dataset and EgoPW dataset with the generated pseudo labels $\mathcal{P}^{ego}_{seq}$ (Sec.~\ref{subsubsec:da}). In order to alleviate the influence of inaccurate pseudo labels, we finally finetune the network on the EgoPW dataset and the pseudo labels with a bootstrapping strategy (Sec.~\ref{subsubsec:bootstrapping}).

\subsection{EgoPW Dataset}\label{subsec:dataset}

% We first present the EgoPW dataset which is the first large in-the-wild egocentric dataset. \LJ{-> We first describe the \emph{EgoPW} dataset we collected, which is the first large in-the-wild human performance dataset in egocentric and external visions}. 
We first describe the \emph{EgoPW} dataset we collected, which is the first large-scale in-the-wild human performance dataset captured by an egocentric camera and an external normal camera (Sony RX0) which are synchronized.
This dataset contains 97 sequences (318k frames in total) of 10 actors in 20 clothing styles performing 20 different actions
, including reading magazine/newspaper, playing board games, doing a presentation, walking, sitting down, using a computer, calling on the phone, drinking water, writing on the paper, writing on the whiteboard, making tea, cutting vegetables, stretching, running, playing table tennis, playing baseball, climbing floors, dancing, opening the door and waving hands. 
% These sequences are collected by an egocentric camera and an external normal camera (Sony RX0) which are synchronized. 
% When collecting the egocentric sequences, we place a normal camera (Sony RX0) looking at the whole human body and record the external images at the same time. This synchronized external view enables the generation of pseudo labels.
We generate 3D poses as pseudo labels using the egocentric and external images, which will be elaborated later. 
In terms of the dataset size, our EgoPW dataset is larger than existing in-the-wild 3D pose estimation datasets like 3DPW~\cite{von2018recovering} and has a similar scale as the existing synthetic egocentric datasets for training including the  Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} dataset and the  $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19} dataset. 

\subsection{Optimization for Generating Pseudo Labels}\label{subsec:optimizer}

In this section, we present an optimization method based on \cite{wang2021estimating} to generate pseudo labels for the EgoPW dataset. We split the whole sequence into segments containing $B$ consecutive frames. 
For the egocentric frames $I^{ego}_{seq}$, we estimate the 3D poses represented by 15 joint locations in the coordinate system of egocentric camera (called ``egocentric poses")  $\widetilde{\mathcal{P}}^{ego}_{seq}=\{\widetilde{\mathcal{P}}^{ego}_1,\dots,\widetilde{\mathcal{P}}^{ego}_B \}$, $\widetilde{\mathcal{P}}^{ego}_i \in \mathbb{R}^{15 \times 3}$, and 2D heatmaps $\mathcal{H}^{ego}_{seq}=\{\mathcal{H}^{ego}_1,\dots,\mathcal{H}^{ego}_B \}$ using the Mo$^2$Cap$^2$ method \cite{DBLP:journals/tvcg/XuCZRFST19}.
Aside from egocentric poses, we also estimate the transformation matrix between the egocentric camera poses of two adjacent frames $[R_{seq}^{SLAM} \mid t_{seq}^{SLAM}] = \{[R_1^2 \mid t_1^2], \dots, [R_{B-1}^{B} \mid t_{B-1}^B]\}$ using ORB-SLAM2~\cite{murTRO2015}.
For the external frames $I^{ext}_{seq}$, we estimate the 3D pose (called ``external poses") $\mathcal{P}^{ext}_{seq}=\{\mathcal{P}^{ext}_1,\dots,\mathcal{P}^{ext}_B \}$, $\mathcal{P}^{ext}_i \in \mathbb{R}^{15 \times 3}$ using VIBE~\cite{DBLP:conf/cvpr/KocabasAB20} and 2D joints $\mathcal{J}^{ext}_{seq}=\{\mathcal{J}^{ext}_1,\dots,\mathcal{J}^{ext}_B \}$, $\mathcal{J}^{ext}_i \in \mathbb{R}^{15 \times 2}$ using openpose~\cite{cao2017realtime}. 

% Next, we design an optimization framework which first captures the motion prior with a sequential VAE \cite{wang2021estimating} and then optimize the egocentric pose sequence $\mathcal{P}_{ego}^{seq}$ with the learned motion prior by minimizing the egocentric and external reprojection term.

Next, following \cite{wang2021estimating}, we learn a latent space to encode an egocentric motion prior with a sequential VAE which consists of a CNN-based encoder $f_{enc}$ and decoder $f_{dec}$. We then optimize the egocentric pose by finding a latent vector $z$ such that the corresponding pose sequence $P^{ego}_{seq} = f_{dec}(z)$ minimizes the objective function:

\begin{equation}
\begin{aligned}
	E (\mathcal{P}_{seq}^{ego}, R_{seq}, t_{seq}) &= \lambda_R^{ego} E_{R}^{ego} + \lambda_R^{ext} E_{R}^{ext} + \lambda_J^{ego} E_{J}^{ego} \\
	& +  \lambda_J^{ext} E_{J}^{ext} + \lambda_T E_{T} + \lambda_B E_{B}\\
	& + \lambda_C E_{C} + \lambda_M E_{M}
	\label{eq:optim}
\end{aligned}
\end{equation}
Note that since the relative pose between external camera and egocentric camera is unknown, we also need to optimize the relative egocentric camera pose with respect to the external camera pose for each frame, i.e. the rotations  $R_{seq} = {R_1,\dots,R_B}$ and translations $t_{seq} = {t_1,\dots,t_B}$.

In this objective function, $E_{R}^{ego}$, $E_{J}^{ego}$,$E_{T}$, and $E_{B}$ are egocentric reprojection term, egocentric pose regularization term, motion smoothness regularization term and bone length regularization term, which are the same as those defined in~\cite{wang2021estimating}. We will also include the detailed definitions in the supplemental materials. 
$E_{R}^{ext}$, $E_{J}^{ext}$, $E_{C}$, and $E_{M}$ are the external reprojection term, external 3D body pose regularization term, camera pose consistency term, and camera matrix regularization term, which will be described later. 



% \begin{equation}
% \begin{aligned}
% 	E (\mathcal{P}_{seq}^{ego}, R, t) &= \lambda_R^{ego} E_{R}^{ego}(\mathcal{P}_{seq}^{ego}) + \lambda_R^{ext} E_{R}^{ext}(\mathcal{P}_{seq}^{ext}, R, t)\\
% 	& + \lambda_J^{ego} E_{J}^{ego}(\mathcal{P}_{seq}^{ego}, \widetilde{\mathcal{P}}_{seq}^{ego}) \\
% 	& + \lambda_J^{ext} E_{J}^{ext}(\mathcal{P}_{seq}^{ego}, \mathcal{P}_{seq}^{ext}) \\
% 	& + \lambda_T E_{T}(\mathcal{P}_{seq}^{ego}) + \lambda_B E_{B}(\mathcal{P}_{seq}^{ego}) \\
% 	& + \lambda_C E_{C}(R, t, R^{ego}, t^{ego}) \\
% 	& + \lambda_M E_{M}(R)
% 	\label{eq:optim}
% \end{aligned}
% \end{equation}

\paragraph{External Reprojection Term}

We use the external 2D detection as a supervision in the optimization framework. The energy term is defined as:
\begin{equation}
    E_{R}^{ext}(\mathcal{P}_{seq}^{ego}, R_{seq}, t_{seq}) = \sum_{i=1}^{B}\left\Vert \mathcal{J}_{i}^{ext} - K\left[R_i\mid t_i\right]\mathcal{P}_{i}^{ego} \right\Vert_2^2 \label{eq:ext_reproj}
\end{equation}
where the $K$ is the intrinsic matrix of the external camera; $\left[R_{i} \mid t_{i} \right]$ is the pose of the egocentric camera of the $i$ th frame in the external camera space. 
In this term, we first project the egocentric body pose $\mathcal{P}_{i}^{ego}$ to the 2D body pose in the external view with the egocentric camera pose $\left[R_{i} \mid t_{i} \right]$ and the intrinsic matrix $K$, and then compare the projected body pose with the 2D joints estimated by the openpose~\cite{cao2017realtime}. Since the relative pose between the external camera and egocentric camera are unknown at the beginning of the optimization, we optimize the egocentric camera pose $\left[R_{i} \mid t_{i} \right]$ along with the egocentric body pose $\mathcal{P}_{seq}^{ego}$. 
In order to make the optimization process converge faster, we initialize the egocentric camera pose $\left[R_{i} \mid t_{i} \right]$ with the Perspective-n-Point algorithm~\cite{Gao2003CompleteSC}.
% However, because of the depth ambiguity, the accurate 3D pose cannot be obtained only with the external reprojection term.

\paragraph{Camera Pose Consistency}

% We cannot get the accurate 3D pose only with the external reprojection term because the egocentric camera pose and the optimized body pose can be arbitrarily changed without violating the external reprojection constraint \LJ{-> because there is an ambiguity in egocentric camera poses. }. 
We cannot get the accurate 3D body pose only with the external reprojection term because the egocentric camera pose and the optimized body pose can be changed in a coordinated manner without violating the constraint, as long as their relative position remains unchanged.
To alleviate this ambiguity, aside from the motion smoothness term $E_T$, we introduce the camera consistency term $E_C$. Specifically, this term enforces the egocentric camera pose at $(i + 1)$ th frame $[R_{i + 1} \mid t_{i + 1}]$ to be consistent with the pose obtained by transforming the egocentric camera pose at the $i$ th frame $[R_{i} \mid t_{i}]$ with the relative pose between the $i$ th and $(i + 1)$ th frame.

% This can be alleviated by applying the motion smoothness term to make the body pose consistent over the time. Aside from this, we also introduce the camera pose consistency term which keeps the camera pose $[R_i \mid t_i]$ and $[R_{i + 1} \mid t_{i + 1}]$ consistent by bridging them with the SLAM method which estimates the relative egocentric camera pose $[R_i^{i+1} \mid t_i^{i+1}]$ between $i$ th and $i + 1$ th frame 

% keeps the egocentric camera pose $[R_i \mid t_i]$ and $[R_{i + 1} \mid t_{i + 1}]$ consistent by bridging them with the relative egocentric camera pose $[R_i^{i+1} \mid t_i^{i+1}]$ between $i$ th and $i + 1$ th frame:

% % \begin{equation}
% % \begin{aligned}
% %     E_{C}(R_{seq}, t_{seq}) & = \sum_{i=1}^{B-1} \left (\left\Vert R_i R_i^{SLAM} - R_{i + 1} \right\Vert_2 \right.\\
% %     & + \left. \left\Vert R_i t_i^{SLAM} + t_i - t_{i + 1}\right\Vert_2 \right) \label{eq:consistency}
% % \end{aligned}
% % \end{equation}

\begin{equation}
\begin{aligned}
    E_{C}(R_{seq}, t_{seq}) & = \sum_{i=1}^{B-1}\left\Vert \begin{bmatrix} R_i  & t_i \\ 0 & 1 \end{bmatrix} \begin{bmatrix} R^{i+1}_i  & t^{i+1}_i \\ 0 & 1 \end{bmatrix} \right.\\
    & - \left. \begin{bmatrix} R_{i+1}  & t_{i+1} \\ 0 & 1 \end{bmatrix}\right\Vert_2 \label{eq:consistency}
\end{aligned}
\end{equation}

\paragraph{External 3D Body Pose Regularization}

Besides the external reprojection term, we also use the external 3D body poses to supervise the optimization of the egocentric 3D body pose. 
We define the external 3D pose term which measures the difference between the external body poses and the egocentric body poses after the rigid alignment:
% transformed from the egocentric camera space to the external camera space. 
% We make the optimized egocentric pose $\mathcal{P}_{i}^{ego}$ stay close to the external 3D pose estimation $\mathcal{P}_{i}^{ext}$ by defining the term as the difference between the 3D joint locations of egocentric and external view after the rigid alignment:

\begin{equation}
	E_{J}(\mathcal{P}_{seq}^{ego}, \mathcal{P}_{seq}^{ext}) = \sum_{i=1}^{B}\left\Vert \mathcal{P}_{i}^{ext} - \left[R_{i}^{pa}\mid t_{i}^{pa}\right]\mathcal{P}_{i}^{ego} \right\Vert_2^2 \label{eq:ext_3d_pose}
\end{equation}
where $\left[R_{i}^{pa} \mid t_{i}^{pa} \right]$ is the transformation matrix calculated with Procrustes analysis which rigidly aligns the external 3D pose estimation $\mathcal{P}_{i}^{ext}$ and the egocentric 3D pose $\mathcal{P}_{i}^{ego}$.

% With the external reprojection term and external 3D pose regularization term, we are able to generate accurate pseudo labels even though the human body in the egocentric view is seriously occluded, as illustrated in Fig.~\ref{fig:optimization_example}. With the external view, we are able to train the network with the accurate pseudo labels for the in-the-wild images, especially in the occluded cases. 

% We note that only by combining the egocentric view and external view, we can reconstruct accurate pseudo labels since the body parts can be either occluded in the egocentric or external view. 
By combining the body poses estimated from the egocentric view and external view, we can reconstruct more accurate pseudo labels.  
As shown in Fig.~\ref{fig:optimization_example}, the hands of the person are occluded in the external view, resulting in the tracking of the hands fails in the external view (Fig.~\ref{fig:optimization_example}, b), however, the hands can be clearly seen and tracked in the egocentric view (Fig.~\ref{fig:optimization_example}, d); 
on the other hand, the feet cannot be observed in the egocentric view and thus failed to be tracked in this view (Fig.~\ref{fig:optimization_example}, b), but can be easily viewed and tracked in the external view (Fig.~\ref{fig:optimization_example}, d). 
%Thus, either the optimizer with only the egocentric view (second image) or the external pose estimation method like VIBE~\cite{DBLP:conf/cvpr/KocabasAB20} (fourth image) cannot predict accurate pseudo labels. 
By joining the information from both views, we can successfully predict accurate 3D poses as the pseudo labels (Fig.~\ref{fig:optimization_example}, c).  
% combining the egocentric and external view in our optimization framework, we can predict accurate 3D poses as the pseudo labels, which is illustrated in the third image.
We note that the external camera is only used for generating the pseudo labels but at test time, only the egocentric camera is used. 

\begin{figure}
\centering
\includegraphics[width=0.98\linewidth]{figures/optimization_example/optimization_example_crop.pdf}
\caption{Our pseudo label generation method combines the information from both the egocentric view and external view, therefore leading to accurate pseudo labels (c). Only with the egocentric camera, the feet cannot be observed and well-tracked (b); Only with the external camera, the hands are occluded and result in the wrong result on the hand part (d).
% We note that the external camera is only used in the pseudo label generation for training, which is not used at test time.
}
% or external view is restrictive for predicting accurate 3D poses (the second and fourth image), while our optimization method gives reasonable result (the third image).
\label{fig:optimization_example}
\end{figure}



\paragraph{Camera Matrix Regularization}

We constrain the camera rotation matrix $R_{i}$ to be an orthogonal matrix:

\begin{equation}
	E_{J}(R_{seq}) = \sum_{i=1}^{B}\left\Vert R_{i}^TR_{i} - I \right\Vert_2^2 \label{eq:matrix}
\end{equation}
where $det(.)$ is the determinant of the matrix.

Through the optimization framework, we can get accurate 3D pose pseudo labels $\mathcal{P}_{seq}^{ego}$, which is further processed into the 2D heatmap $\mathcal{H_T}$ and the distance between joints and egocentric camera $\mathcal{D_T}$ with the fisheye camera model \cite{scaramuzza2014omnidirectional} described in supplementary materials. 

% for each batch and combine the batches to get the 3D labels for the whole EgoPW dataset $\mathcal{P_T}$ \LJ{I don't think we need to mention this, suggest removing the above sentence}

% , where the projection of a 3D point $[x, y, z]^T$ can be written as:

% \begin{equation}
% 	[u, v]^T = \frac{[x, y]^T}{\sqrt{x^2 + y^2}} \times f(\rho)
% \end{equation}
% where $\rho = \arctan(z / \sqrt{x^2 + y^2})$ and $f(\rho) = \alpha_0 + \alpha_1 \rho + \alpha_2 \rho^2 + \alpha_3 \rho^3 +\dots$ is a polynomial obtained from camera calibration.


\subsection{Domain Adaptation}\label{subsec:train}

After obtaining the pseudo labels for the EgoPW dataset, we introduce a domain adaptation approach for training a pose estimation network, which can be used for estimating the 3D pose from a single egocentric image. Our core idea is to use an adversarial discriminator to tackle the problem of the domain gap between the synthetic data and the real in-the-wild data. Here, we define the source domain $\mathcal{S} = \{\mathcal{I_{S}}, \mathcal{H_{S}}, \mathcal{D_{S}}\}$ which is composed of synthetic images $\mathcal{I_{S}}$ along with their corresponding heatmap $\mathcal{H_{S}}$ and distance $\mathcal{D_{S}}$ labels from Mo$^2$Cap$^2$ dataset, and the target domain $\mathcal{T}= \{\mathcal{I_{T}}, \mathcal{H_{T}}, \mathcal{D_{T}}\}$ which consists of in-the-wild egocentric images $\mathcal{I_T}$ with pseudo heatmaps $\mathcal{H_{T}}$ and distance labels $\mathcal{D_{T}}$ from EgoPW dataset. We first minimize the domain gap between the source and target domain using an adversarial domain adaptation network and then apply a bootstrapping strategy to finetune the network on the EgoPW dataset with pseudo labels. 

% In this section, we introduce our domain adaptation approach for training the egocentric pose estimation network on the EgoPW dataset. The source domain $\mathcal{S}$ consists of synthetic images $\mathcal{I_{S}}$ and the corresponding heatmap $\mathcal{H_{S}}$ and distance $\mathcal{D_{S}}$ labels from Mo$^2$Cap$^2$ dataset, and the target domain $\mathcal{T}$ consists of in-the-wild egocentric images $\mathcal{I_T}$ with pseudo heatmaps $\mathcal{H_{T}}$ and distance $\mathcal{D_{T}}$ labels \LJ{distance labels?} from EgoPW dataset. We firstly minimize the domain gap between the source and target domain using an adversarial domain adaptation network, and further apply a bootstrapping strategy to finetune the network on the EgoPW dataset with pseudo labels. 

\subsubsection{Adversarial Domain Adaptation Module}\label{subsubsec:da}

Our adversarial domain adaptation module consists of a Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} network for estimating the egocentric pose and an adversarial discriminator $\Gamma$. The Mo$^2$Cap$^2$ network has a feature extractor $\Theta$ which encodes an image into a feature vector and a pose estimator $\Psi$ which decodes the feature vector to a heatmap and a 3D pose. 
The adversarial discriminator takes as input the feature vectors extracted from a synthetic image and an in-the-wild image, and determines if the feature is extracted from an in-the-wild image. 
Note that the synthetic image does not have a corresponding in-the-wild image, so we refer to this data as \emph{unpaired}. 
We train the adversarial domain adaptation module with two reconstruction loss terms and a discriminator loss term.

The reconstruction loss is defined as the mean squared error (MSE) between the predicted heatmaps/distances and heatmaps/distances from pseudo labels.

% The reconstruction loss is defined as the sum of the mean squared error (MSE) between the predicted heatmaps and the ground truth heatmaps and that between the predicted distances and the ground truth distances. 

\begin{equation}
    \begin{aligned}
        \mathcal{L}_{S} &= \text{mse}(\mathcal{\hat{H}_{S}}, \mathcal{H_{S}}) + \text{mse}(\mathcal{\hat{D}_{S}}, \mathcal{D_{S}})\\
        \mathcal{L}_{T} &= \text{mse}(\mathcal{\hat{H}_{T}}, \mathcal{H_{T}}) + \text{mse}(\mathcal{\hat{D}_{T}}, \mathcal{D_{T}})
    \end{aligned}
\end{equation}
where 
% Given a pair of images $(\mathcal{I_{S}}, \mathcal{I_{T}}) \in \mathbb{R}^{H \times W \times 3}$ from the Mo$^2$Cap$^2$ and EgoPW dataset,  the intermediate features $(\mathcal{F_{S}}, \mathcal{F_{T}})$ is obtained by the extractor $\Theta$, which is subsequently put into the decoder $\Psi$ for generating 2D heatmap $(\mathcal{\hat{H}_{S}}, \mathcal{\hat{H}_{T}})$ and the distance $(\mathcal{\hat{D}_{S}}, \mathcal{\hat{D}_{T}})$ predictions:
\begin{equation}
    \begin{aligned}
        \mathcal{F_{S}} = \Theta(\mathcal{I_{S}});& \mathcal{F_{T}} = \Theta(\mathcal{I_{T}})\\
        \mathcal{\hat{H}_{S}}, \mathcal{\hat{D}_{S}} = \Psi(\mathcal{F_{S}});& \mathcal{\hat{H}_{T}}, \mathcal{\hat{D}_{T}} = \Psi(\mathcal{F_{T}})
    \end{aligned}
\end{equation}
% and the 3D poses $\mathcal{\hat{P}_S}$ and $\mathcal{\hat{P}_T}$ can be obtained with the fisheye camera model \cite{scaramuzza2014omnidirectional} described in supplementary materials. 

% We define the loss in the source and target domain as the mean square error (MSE) between the predictions and the labels:

% \begin{equation}
%     \begin{aligned}
%         \mathcal{L}_{S} &= mse(\mathcal{\hat{H}_{S}}, \mathcal{H_{S}}) + mse(\mathcal{\hat{D}_{S}}, \mathcal{D_{S}})\\
%         \mathcal{L}_{T} &=  mse(\mathcal{\hat{H}_{T}}, \mathcal{H_{T}}) + mse(\mathcal{\hat{D}_{T}}, \mathcal{D_{T}})
%     \end{aligned}
% \end{equation}

To bridge the domain gap between the source and target domains, we use an adversarial discriminator $\Gamma$ to distinguish the feature vectors from source or target data with a cross-entropy loss:

\begin{equation}
    \mathcal{L}_{Dis} = -E[\log(\Gamma(\mathcal{F_S}))] - E[\log(1 - \Gamma(\mathcal{F_T}))]
\end{equation}

Once the discriminator $\Gamma$ has been trained, the feature extractor $\Theta$ maps the images from different domains to the same feature space such that the classifier $\Gamma$ cannot tell if the features are extracted from synthetic images or real images. Therefore, the pose estimator $\Psi$ can predict more accurate poses for the in-the-wild data. 

\subsubsection{Bootstrapping}\label{subsubsec:bootstrapping}

\begin{figure}
\centering
\includegraphics[width=1\linewidth]{figures/optimization_iterations/optimization_iterations_wide_crop.pdf}
\caption{Results in the bootstrapping process. Given an inaccurate pose (initial network prediction) to initialize the optimization process, the pseudo label obtained with our optimization framework is inaccurate (initial optimization). However, given a good egocentric prediction from our finetuned network (final network prediction) for initialization, the optimization can converge to an accurate pose (final optimization).
% \LJ{Given the initial pseudo labels as supervision for the pose estimation network, the estimated pose from the network is inaccurate (initial network prediction). ...}
}
\label{fig:optimization_iterations}
\end{figure}

% In the Sec.~\ref{subsubsec:da}, we use the EgoPW dataset with the pseudo labels generated by the optimizer from the Mo2Cap2 predictions. 
While significant performance improvement has been made by the  adversarial domain adaptation, the accuracy of pose predictions is still limited due to the errors in the generated pseudo labels. These errors mostly stem from the noisy egocentric 3D poses and 2D heatmaps predicted by the Mo$^2$Cap$^2$ network. 
% Though significant performance improvement can be achieved by incorporating the adversarial domain adaptation in Sec.~\ref{subsubsec:da}, the accuracy of network predictions is still limited due to the significant errors in pseudo labels obtained by our optimization framework. These errors mostly stem from the noisy egocentric 3D poses and 2D heatmaps predicted by the Mo$^2$Cap$^2$ network. 

To circumvent this issue, inspired by SPIN~\cite{DBLP:conf/iccv/KolotourosPBD19}, we develop a bootstrapping algorithm. We first apply our adversarial domain-adaptation network (Sec.~\ref{subsubsec:da}) to get the initial egocentric 3D poses and use them for initializing the optimization framework. Next, we use the optimization framework (Sec.~\ref{subsec:optimizer}) to generate the pseudo labels and use the labels to finetune the pose estimation network. We execute this process iteratively, such that the finetuned network provides better initialization for the optimization framework and the optimization framework generates better pseudo labels to finetune the network:

\begin{algorithm}
\SetAlgoLined
\KwIn{$\Theta$, $\Psi$, $\mathcal{I_T}$, $\mathcal{H_T}$, $\mathcal{D_T}$, optimizer, max\_iter}
\KwOut{Finetuned network parameters $\Theta$}
 iter $\coloneqq$ 0\;
 \While{iter $<$ max\_iter}{
  $\mathcal{H}, \mathcal{D} \coloneqq \Psi(\Theta(\mathcal{I_T}))$\;
  $\mathcal{H_T}, \mathcal{D_T} \coloneqq$ optimizer$(\mathcal{H}, \mathcal{D})$\;
  update network parameter of $\Theta$ and $\Psi$ with $\mathcal{L}_{T}$\;
  iter $\coloneqq$ iter + 1\;
 }
 \caption{Bootstrapping Algorithm}
\end{algorithm}

We show the results before and after bootstrapping in Fig.~\ref{fig:optimization_iterations}. We can see that the pseudo labels have been improved significantly with bootstrapping, and the improved pseudo labels provide a better supervision for the pose estimation network, leading to better pose estimation for the in-the-wild data. 

% We show the initial optimized result and final optimized result in Fig.~\ref{fig:optimization_iterations}, which demonstrate that the pseudo labels are improved significantly along the training process. The improved pseudo labels provides a better supervision, enabling the better performance of the pose estimation network on the in-the-wild data.

% 






==> sections_old/method_cvpr.tex <==
\section{Method}
We propose a new approach to train a network with the weak supervision from egocentric and external views. This network is able to estimate an accurate 3D body pose from a single egocentric in-the-wild image. The overview of our approach is illustrated in Fig.~\ref{fig:framework}. We first capture a large egocentric in-the-wild dataset, called \emph{EgoPW}, which contains synchronized egocentric image sequences and external image sequences (Sec.~\ref{subsec:dataset}). Next, we generate the pseudo labels for the EgoPW dataset with an optimization-based framework. This framework takes a sequence in a time window with $B$ frames of egocentric images $\mathcal{I}^{ego}_{seq}=\{\mathcal{I}^{ego}_{1},\dots,\mathcal{I}^{ego}_{B}\}$ and external images $\mathcal{I}^{ext}_{seq}=\{\mathcal{I}^{ext}_{1},\dots,\mathcal{I}^{ext}_{B}\}$ as input and outputs egocentric 3D poses $\mathcal{P}^{ego}_{seq}=\{\mathcal{P}^{ego}_{1},\dots,\mathcal{P}^{ego}_{B}\}$ as the pseudo labels (Sec.~\ref{subsec:optimizer}). 

Next, we train the egocentric pose estimation network on the synthetic data and on the EgoPW dataset with pseudo labels $\mathcal{P}^{ego}_{seq}$. In the training process, we leverage the intermediate feature representation from the external pose estimation network~\cite{xiao2018simple} to supervise the training of egocentric pose estimation network in an adversarial way (Sec.~\ref{subsubsec:ext_adv}). We also introduce the adversarial domain adaptation strategy to eliminate the domain gap between synthetic and real dataset (Sec.~\ref{subsubsec:da}).


\subsection{EgoPW Dataset}\label{subsec:dataset}

We first describe the \emph{EgoPW} dataset we collected, which is the first large-scale in-the-wild human performance dataset captured by an egocentric camera and an external normal camera (Sony RX0) which are synchronized.
This dataset contains 97 sequences (318k frames in total) of 10 actors in 20 clothing styles performing 20 different actions
, including reading magazine/newspaper, playing board games, doing a presentation, walking, sitting down, using a computer, calling on the phone, drinking water, writing on the paper, writing on the whiteboard, making tea, cutting vegetables, stretching, running, playing table tennis, playing baseball, climbing floors, dancing, opening the door and waving hands. 
We generate 3D poses as pseudo labels using the egocentric and external images, which will be elaborated later. 
In terms of the dataset size, our EgoPW dataset is larger than existing in-the-wild 3D pose estimation datasets like 3DPW~\cite{von2018recovering} and has a similar scale as the existing synthetic egocentric datasets for training including the  Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} dataset and the  $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19} dataset. 

\subsection{Optimization for Generating Pseudo Labels}\label{subsec:optimizer}

In this section, we present an optimization method based on \cite{wang2021estimating} to generate pseudo labels for the EgoPW dataset. We split the whole sequence into segments containing $B$ consecutive frames. 
For the egocentric frames $I^{ego}_{seq}$, we estimate the 3D poses represented by 15 joint locations in the coordinate system of egocentric camera (called ``egocentric poses")  $\widetilde{\mathcal{P}}^{ego}_{seq}=\{\widetilde{\mathcal{P}}^{ego}_1,\dots,\widetilde{\mathcal{P}}^{ego}_B \}$, $\widetilde{\mathcal{P}}^{ego}_i \in \mathbb{R}^{15 \times 3}$, and 2D heatmaps $\mathcal{H}^{ego}_{seq}=\{\mathcal{H}^{ego}_1,\dots,\mathcal{H}^{ego}_B \}$ using the Mo$^2$Cap$^2$ method \cite{DBLP:journals/tvcg/XuCZRFST19}.
Aside from egocentric poses, we also estimate the transformation matrix between the egocentric camera poses of two adjacent frames $[R_{seq}^{SLAM} \mid t_{seq}^{SLAM}] = \{[R_1^2 \mid t_1^2], \dots, [R_{B-1}^{B} \mid t_{B-1}^B]\}$ using ORB-SLAM2~\cite{murTRO2015}.
For the external frames $I^{ext}_{seq}$, we estimate the 3D pose (called ``external poses") $\mathcal{P}^{ext}_{seq}=\{\mathcal{P}^{ext}_1,\dots,\mathcal{P}^{ext}_B \}$, $\mathcal{P}^{ext}_i \in \mathbb{R}^{15 \times 3}$ using VIBE~\cite{DBLP:conf/cvpr/KocabasAB20} and 2D joints $\mathcal{J}^{ext}_{seq}=\{\mathcal{J}^{ext}_1,\dots,\mathcal{J}^{ext}_B \}$, $\mathcal{J}^{ext}_i \in \mathbb{R}^{15 \times 2}$ using openpose~\cite{cao2017realtime}. 

Next, following \cite{wang2021estimating}, we learn a latent space to encode an egocentric motion prior with a sequential VAE which consists of a CNN-based encoder $f_{enc}$ and decoder $f_{dec}$. We then optimize the egocentric pose by finding a latent vector $z$ such that the corresponding pose sequence $P^{ego}_{seq} = f_{dec}(z)$ minimizes the objective function:

\begin{equation}
\begin{aligned}
	E (\mathcal{P}_{seq}^{ego}, R_{seq}, t_{seq}) &= \lambda_R^{ego} E_{R}^{ego} + \lambda_R^{ext} E_{R}^{ext} + \lambda_J^{ego} E_{J}^{ego} \\
	& +  \lambda_J^{ext} E_{J}^{ext} + \lambda_T E_{T} + \lambda_B E_{B}\\
	& + \lambda_C E_{C} + \lambda_M E_{M}
	\label{eq:optim}
\end{aligned}
\end{equation}
Note that since the relative pose between external camera and egocentric camera is unknown, we also need to optimize the relative egocentric camera pose with respect to the external camera pose for each frame, i.e. the rotations  $R_{seq} = {R_1,\dots,R_B}$ and translations $t_{seq} = {t_1,\dots,t_B}$.

In this objective function, $E_{R}^{ego}$, $E_{J}^{ego}$,$E_{T}$, and $E_{B}$ are egocentric reprojection term, egocentric pose regularization term, motion smoothness regularization term and bone length regularization term, which are the same as those defined in~\cite{wang2021estimating}. We will also include the detailed definitions in the supplemental materials. 
$E_{R}^{ext}$, $E_{J}^{ext}$, $E_{C}$, and $E_{M}$ are the external reprojection term, external 3D body pose regularization term, camera pose consistency term, and camera matrix regularization term, which will be described later. 



\paragraph{External Reprojection Term}

We use the external 2D detection as a supervision in the optimization framework. The energy term is defined as:
\begin{equation}
    E_{R}^{ext}(\mathcal{P}_{seq}^{ego}, R_{seq}, t_{seq}) = \sum_{i=1}^{B}\left\Vert \mathcal{J}_{i}^{ext} - K\left[R_i\mid t_i\right]\mathcal{P}_{i}^{ego} \right\Vert_2^2 \label{eq:ext_reproj}
\end{equation}
where the $K$ is the intrinsic matrix of the external camera; $\left[R_{i} \mid t_{i} \right]$ is the pose of the egocentric camera of the $i$ th frame in the external camera space. 
In this term, we first project the egocentric body pose $\mathcal{P}_{i}^{ego}$ to the 2D body pose in the external view with the egocentric camera pose $\left[R_{i} \mid t_{i} \right]$ and the intrinsic matrix $K$, and then compare the projected body pose with the 2D joints estimated by the openpose~\cite{cao2017realtime}. Since the relative pose between the external camera and egocentric camera are unknown at the beginning of the optimization, we optimize the egocentric camera pose $\left[R_{i} \mid t_{i} \right]$ along with the egocentric body pose $\mathcal{P}_{seq}^{ego}$. 
In order to make the optimization process converge faster, we initialize the egocentric camera pose $\left[R_{i} \mid t_{i} \right]$ with the Perspective-n-Point algorithm~\cite{Gao2003CompleteSC}.


\paragraph{Camera Pose Consistency}

We cannot get the accurate 3D body pose only with the external reprojection term because the egocentric camera pose and the optimized body pose can be changed in a coordinated manner without violating the constraint, as long as their relative position remains unchanged.
To alleviate this ambiguity, aside from the motion smoothness term $E_T$, we introduce the camera consistency term $E_C$. Specifically, this term enforces the egocentric camera pose at $(i + 1)$ th frame $[R_{i + 1} \mid t_{i + 1}]$ to be consistent with the pose obtained by transforming the egocentric camera pose at the $i$ th frame $[R_{i} \mid t_{i}]$ with the relative pose between the $i$ th and $(i + 1)$ th frame.

\begin{equation}
\begin{aligned}
    E_{C}(R_{seq}, t_{seq}) & = \sum_{i=1}^{B-1}\left\Vert \begin{bmatrix} R_i  & t_i \\ 0 & 1 \end{bmatrix} \begin{bmatrix} R^{i+1}_i  & t^{i+1}_i \\ 0 & 1 \end{bmatrix} \right.\\
    & - \left. \begin{bmatrix} R_{i+1}  & t_{i+1} \\ 0 & 1 \end{bmatrix}\right\Vert_2 \label{eq:consistency}
\end{aligned}
\end{equation}

\paragraph{External 3D Body Pose Regularization}

Besides the external reprojection term, we also use the external 3D body poses to supervise the optimization of the egocentric 3D body pose. 
We define the external 3D pose term which measures the difference between the external body poses and the egocentric body poses after the rigid alignment:
% transformed from the egocentric camera space to the external camera space. 
% We make the optimized egocentric pose $\mathcal{P}_{i}^{ego}$ stay close to the external 3D pose estimation $\mathcal{P}_{i}^{ext}$ by defining the term as the difference between the 3D joint locations of egocentric and external view after the rigid alignment:

\begin{equation}
	E_{J}(\mathcal{P}_{seq}^{ego}, \mathcal{P}_{seq}^{ext}) = \sum_{i=1}^{B}\left\Vert \mathcal{P}_{i}^{ext} - \left[R_{i}^{pa}\mid t_{i}^{pa}\right]\mathcal{P}_{i}^{ego} \right\Vert_2^2 \label{eq:ext_3d_pose}
\end{equation}
where $\left[R_{i}^{pa} \mid t_{i}^{pa} \right]$ is the transformation matrix calculated with Procrustes analysis which rigidly aligns the external 3D pose estimation $\mathcal{P}_{i}^{ext}$ and the egocentric 3D pose $\mathcal{P}_{i}^{ego}$.

% With the external reprojection term and external 3D pose regularization term, we are able to generate accurate pseudo labels even though the human body in the egocentric view is seriously occluded, as illustrated in Fig.~\ref{fig:optimization_example}. With the external view, we are able to train the network with the accurate pseudo labels for the in-the-wild images, especially in the occluded cases. 

% We note that only by combining the egocentric view and external view, we can reconstruct accurate pseudo labels since the body parts can be either occluded in the egocentric or external view. 
By combining the body poses estimated from the egocentric view and external view, we can reconstruct more accurate pseudo labels.  
As shown in Fig.~\ref{fig:optimization_example}, the hands of the person are occluded in the external view, resulting in the tracking of the hands fails in the external view (Fig.~\ref{fig:optimization_example}, b), however, the hands can be clearly seen and tracked in the egocentric view (Fig.~\ref{fig:optimization_example}, d); 
on the other hand, the feet cannot be observed in the egocentric view and thus failed to be tracked in this view (Fig.~\ref{fig:optimization_example}, b), but can be easily viewed and tracked in the external view (Fig.~\ref{fig:optimization_example}, d). 
%Thus, either the optimizer with only the egocentric view (second image) or the external pose estimation method like VIBE~\cite{DBLP:conf/cvpr/KocabasAB20} (fourth image) cannot predict accurate pseudo labels. 
By joining the information from both views, we can successfully predict accurate 3D poses as the pseudo labels (Fig.~\ref{fig:optimization_example}, c).  
% combining the egocentric and external view in our optimization framework, we can predict accurate 3D poses as the pseudo labels, which is illustrated in the third image.
We note that the external camera is only used for generating the pseudo labels but at test time, only the egocentric camera is used. 

\begin{figure}
\centering
\includegraphics[width=0.98\linewidth]{figures/optimization_example/optimization_example_crop.pdf}
\caption{Our pseudo label generation method combines the information from both the egocentric view and external view, therefore leading to accurate pseudo labels (c). Only with the egocentric camera, the feet cannot be observed and well-tracked (b); Only with the external camera, the hands are occluded and result in the wrong result on the hand part (d).
% We note that the external camera is only used in the pseudo label generation for training, which is not used at test time.
}
% or external view is restrictive for predicting accurate 3D poses (the second and fourth image), while our optimization method gives reasonable result (the third image).
\label{fig:optimization_example}
\end{figure}



\paragraph{Camera Matrix Regularization}

We constrain the camera rotation matrix $R_{i}$ to be an orthogonal matrix:

\begin{equation}
	E_{J}(R_{seq}) = \sum_{i=1}^{B}\left\Vert R_{i}^TR_{i} - I \right\Vert_2^2 \label{eq:matrix}
\end{equation}
where $det(.)$ is the determinant of the matrix.

Through the optimization framework, we can get accurate 3D pose pseudo labels $\mathcal{P}_{seq}^{ego}$ for each egocentric frame in EgoPW dataset, which is further processed into the 2D heatmap $\mathcal{H_E}$ and the distance between joints and egocentric camera $\mathcal{D_E}$ with the fisheye camera model \cite{scaramuzza2014omnidirectional} described in supplementary materials. 

Different from previous single-view pose estimation methods which leverages the weak supervision from multiple views~\cite{iqbal2020weakly,rhodin2018learning,wandt2021canonpose,kocabas2019self}, our spatio-temporal optimization method generates the pseudo labels under the guidance of learned motion prior, making it robust to noisy and inaccurate 2D pose estimations, which is common for the 2D pose estimation results from the egocentric view.


\subsection{Training Egocentric Pose Estimation Network}\label{subsec:train}

After obtaining the pseudo labels for the EgoPW dataset, we train a single-image based egocentric pose estimation network on both the synthetic dataset from Mo$^2$Cap$^2$ and the EgoPW dataset. The pose estimation network contains a feature extractor $\Theta$ which encodes an image into a feature vector and a pose estimator $\Psi$ which decodes the feature vector to a heatmap and a 3D pose. Here, we note the synthetic dataset $S = \{I_S, H_S, D_S\}$ which is composed of synthetic images $I_S$ along with their corresponding heatmap $H_S$ and distance labels $D_S$ from Mo$^2$Cap$^2$ dataset, and the EgoPW dataset $E = \{I_E^{ego}, H_E, D_E, I_E^{ext} \}$ which is composed of egocentric in-the-wild images $I_E^{ego}$ along with pseudo heatmaps $H_E$, distance labels $D_E$ and corresponding external images $I_E^{ext}$. 
During the training process, we train the egocentric pose estimation network with two reconstruction loss terms and two adversarial loss terms. The reconstruction loss is defined as the mean squared error (MSE) between the predicted heatmaps/distances and heatmaps/distances from labels.

% After obtaining the pseudo labels for the EgoPW dataset, we train a single-image based egocentric pose estimation network on both the synthetic dataset from Mo$^2$Cap$^2$ and the EgoPW dataset. The pose estimation network contains a feature extractor $\Theta$ which encodes an image into a feature vector and a pose estimator $\Psi$ which decodes the feature vector to a heatmap and a 3D pose. Here, we note the synthetic dataset $S = \{\mathcal{I_S}, \mathcal{H_S}, \mathcal{D_S}\}$ which is composed of synthetic images $\mathcal{I_S}$ along with their corresponding heatmap $\mathcal{H_S}$ and distance labels $\mathcal{D_S}$ from Mo$^2$Cap$^2$ dataset, and the EgoPW dataset $\mathcal{E} = \{ \mathcal{I_E}^{ego}, \mathcal{H_E}, \mathcal{D_E}, \mathcal{I_E}^{ext} \}$ which is composed of egocentric in-the-wild images $\mathcal{I_E}^{ego}$ along with pseudo heatmaps $\mathcal{H_E}$, distance labels $\mathcal{D_E}$ and corresponding external images $\mathcal{I_E}^{ext}$. 
% During the training process, we train the egocentric pose estimation network with two reconstruction loss terms and two adversarial loss terms. The reconstruction loss is defined as the mean squared error (MSE) between the predicted heatmaps/distances and heatmaps/distances from labels.

\begin{equation}
    \begin{aligned}
        \mathcal{L}_{S} &= \text{mse}(\mathcal{\hat{H}_{S}}, \mathcal{H_{S}}) + \text{mse}(\mathcal{\hat{D}_{S}}, \mathcal{D_{S}})\\
        \mathcal{L}_{E} &= \text{mse}(\mathcal{\hat{H}_{E}}, \mathcal{H_{E}}) + \text{mse}(\mathcal{\hat{D}_{E}}, \mathcal{D_{E}})
    \end{aligned}
\end{equation}
where 
\begin{equation}
    \begin{aligned}
        \mathcal{F_{S}} = \Theta(\mathcal{I_{S}});& \mathcal{F_{E}}^{ego} = \Theta(\mathcal{I_{E}}^{ego})\\
        \mathcal{\hat{H}_{S}}, \mathcal{\hat{D}_{S}} = \Psi(\mathcal{F_{S}});& \mathcal{\hat{H}_{E}}, \mathcal{\hat{D}_{E}} = \Psi(\mathcal{F_{E}}^{ego})
    \end{aligned}
\end{equation}

Two adversarial losses are separately designed for learning egocentric semantic representation and bridging the domain gap between synthetic and real dataset. These two loss functions will be described below. 


\subsubsection{Learning Egocentric Image Representation}\label{subsubsec:ext_adv}

Note that the identity and body pose are exactly the same in a pair of egocentric-external images $\{ \mathcal{I_E}^{ego}, \mathcal{I_E}^{ext} \}$. Thus, the intermediate feature from the egocentric pose estimation network $\mathcal{F_{E}}^{ego}$ and the external pose estimation network $\mathcal{F_{E}}^{ext}$ should share the same semantic representation. Based on this observation, we use the features from external pose estimation network to supervise the egocentric pose estimation network. However, directly minimizing the distance between egocentric features $\mathcal{F_{E}}^{ego}$ and external features $\mathcal{F_{E}}^{ext}$ will not enhance the performance since the intermediate features of the egocentric and external view should be very different from each other due to significant difference on the view direction and camera distortions. To tackle this issue, we introduce the adversarial training strategy to align the intermediate features from egocentric and external networks. Specifically, we use an adversarial discriminator $\Lambda$ which takes the feature vectors extracted from a egocentric image and the corresponding in-the-wild images and predicts if the feature is from egocentric or external images. The adversarial discriminator $\Lambda$ is trained with a cross-entropy loss:

\begin{equation}
    \mathcal{L}_{R} = -E[\log(\Lambda(\mathcal{F_E}^{ego}))] - E[\log(1 - \Lambda(\mathcal{F_E}^{ext}))]
\end{equation}

During the training process, the egocentric pose estimation network is trained to produce the features to fool the domain classifier $\Lambda$ such that $\Lambda$ cannot distinguish whether the feature is from an egocentric or external image. In order to achieve this, the pose estimation network is trained to generate features with semantic representation of human body, since the semantic representation of corresponding egocentric and external images should be the same. This is proved by Figure, where the features from egocentric network focus on the representation of human body after the adversarial training process.


\subsubsection{Adversarial Domain Adaptation}\label{subsubsec:da}
To bridge the domain gap between the synthetic and real data domains, following Tzeng~\etal~\cite{tzeng2017adversarial}, we introduce an adversarial discriminator $\Gamma$ which takes as input the feature vectors extracted from a synthetic image and an in-the-wild image, and determines if the feature is extracted from an in-the-wild image. 
The adversarial discriminator $\Gamma$ is trained with a cross-entropy loss:

\begin{equation}
    \mathcal{L}_{D} = -E[\log(\Gamma(\mathcal{F_S}))] - E[\log(1 - \Gamma(\mathcal{F_T}))]
\end{equation}

Once the discriminator $\Gamma$ has been trained, the feature extractor $\Theta$ maps the images from different domains to the same feature space such that the classifier $\Gamma$ cannot tell if the features are extracted from synthetic images or real images. Therefore, the pose estimator $\Psi$ can predict more accurate poses for the in-the-wild data. 

% Aside from training the network on the EgoPW dataset, we also train the pose estimation network simultaneously on the synthetic dataset considering that synthetic data has its advantages compared to real data, e.g. it is easily accessible and has large variations on poses and backgrounds. To address the domain gap between the synthetic data and real data, we introduce a new adversarial domain adaptation method. Specifically, we extract the features from the synthetic data and real data and use an adversarial discriminator to distinguish if the feature is from synthetic data or real data. Once trained, the feature extractor would learn to produce the features in the same feature space for synthetic data and real data. In this way, our method is able to make full use of the synthetic data and real data, thus achieving better results. 

